A study of events with photoelectric emission in the DarkSide-50 liquid argon Time Projection Chamber

Finding unequivocal evidence of dark matter interactions in a particle detector is a major objective of physics research. Liquid argon time projection chambers offer a path to probe Weakly Interacting Massive Particles scattering cross sections on nucleus down to the so-called neutrino floor, in a mass range from few GeV's to hundredths of TeV's. Based on the successful operation of the DarkSide-50 detector at LNGS, a new and more sensitive experiment, DarkSide-20k, has been designed and is now under construction. A thorough understanding of the DarkSide-50 detector response and, therefore, of all kind of observed events, is essential for an optimal design of the new experiment. In this paper, we report on a particular set of events, which were not used for dark matter searches. Namely, standard two-pulse scintillation-ionization signals accompanied by a small amplitude third pulse, originating from single or few electrons, in a time window of less than a maximum drift time. We compare our findings to those of a recent paper of the LUX Collaboration (D.S.Akerib et al. Phys.Rev.D 102, 092004). Indeed, both experiments observe events related to photoionization of the cathode. From the measured rate of these events, we estimate for the first time the quantum efficiency of the tetraphenyl butadiene deposited on the DarkSide-50 cathode at wavelengths around 128 nm, in liquid argon. Also, both experiments observe events likely related to photoionization of impurities in the liquid. The probability of photoelectron emission per unit length turns out to be one order of magnitude smaller in DarkSide-50 than in LUX. This result, together with the much larger measured electron lifetime, coherently hints toward a lower concentration of contaminants in DarkSide-50 than in LUX.

==> AU-50-2021.tex <==
\author{P.~Agnes}\affiliation{\Houston}
\author{I.F.M.~Albuquerque}\affiliation{\USP}
\author{T.~Alexander}\affiliation{\PNNL}
\author{A.K.~Alton}\affiliation{\Augustana}
\author{M.~Ave}\affiliation{\USP}
\author{H.O.~Back}\affiliation{\PNNL}
\author{G.~Batignani}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{K.~Biery}\affiliation{\FNAL}
\author{V.~Bocci}\affiliation{\RMUnoINFN}
%\author{G.~Bonfini}\affiliation{\AQLNGS}
\author{W.M.~Bonivento}\affiliation{\CAINFN}
\author{B.~Bottino}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{S.~Bussino}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{M.~Cadeddu}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{M.~Cadoni}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{F.~Calaprice}\affiliation{\Princeton}
\author{A.~Caminata}\affiliation{\GEINFN}
\author{N.~Canci}\affiliation{\Houston}\affiliation{\AQLNGS}
%\author{A.~Candela}\affiliation{\AQLNGS}
\author{M.~Caravati}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{M.~Cariello}\affiliation{\GEINFN}
\author{M.~Carlini}\affiliation{\AQLNGS}\affiliation{\AQGSSI}
\author{M.~Carpinelli}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{S.~Catalanotti}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{V.~Cataudella}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{P.~Cavalcante}\affiliation{\VTech}\affiliation{\AQLNGS}
\author{S.~Cavuoti}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{A.~Chepurnov}\affiliation{\MSU}
\author{C.~Cical\`o}\affiliation{\CAINFN}
\author{A.G.~Cocco}\affiliation{\NAINFN}
\author{G.~Covone}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{D.~D'Angelo}\affiliation{\MIUni}\affiliation{\MIINFN}
\author{S.~Davini}\affiliation{\GEINFN}
\author{A.~De~Candia}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{S.~De~Cecco}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
%\author{M.~De~Deo}\affiliation{\AQLNGS}
\author{G.~De~Filippis}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{G.~De~Rosa}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{A.V.~Derbin}\affiliation{\Petersburg}
\author{A.~Devoto}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
%\author{F.~Di~Eusanio}\affiliation{\Princeton}\affiliation{\VTech}
\author{M.~D'Incecco}\affiliation{\AQLNGS}
%\author{G.~Di~Pietro}\affiliation{\AQLNGS}\affiliation{\MIINFN}
\author{C.~Dionisi}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{M.~Downing}\affiliation{\UMass}
\author{D.~D'Urso}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
%\author{E.~Edkins}\affiliation{\Hawaii}
%\author{A.~Empl}\affiliation{\Houston}
\author{G.~Fiorillo}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
%\author{K.~Fomenko}\affiliation{\JINR}
\author{D.~Franco}\affiliation{\APC}
\author{F.~Gabriele}\affiliation{\AQLNGS}
\author{C.~Galbiati}\affiliation{\Princeton}\affiliation{\AQGSSI}\affiliation{\AQLNGS}\affiliation{\CentroFermi}
\author{C.~Ghiano}\affiliation{\AQLNGS}
%\author{S.~Giagu}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{C.~Giganti}\affiliation{\LPNHE}
\author{G.K.~Giovanetti}\affiliation{\Princeton}
\author{O.~Gorchakov}\altaffiliation{Deceased.}\affiliation{\JINR}
\author{A.M.~Goretti}\affiliation{\AQLNGS}
%\author{F.~Granato}\affiliation{\Temple}
\author{A.~Grobov}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{M.~Gromov}\affiliation{\MSU}\affiliation{\JINR}
\author{M.~Guan}\affiliation{\IHEP}
%\author{Y.~Guardincerri}\altaffiliation{Deceased.}\affiliation{\FNAL}
\author{M.~Gulino}\affiliation{\ENUniCEE}\affiliation{\CTLNS}
\author{B.R.~Hackett}\affiliation{\Hawaii}
\author{K.~Herner}\affiliation{\FNAL}
\author{B.~Hosseini}\affiliation{\CAINFN}
%\author{D.~Hughes}\affiliation{\Princeton}
%\author{P.~Humble}\affiliation{\PNNL}
\author{E.V.~Hungerford}\affiliation{\Houston}
%\author{Al.~Ianni}\affiliation{\AQLNGS}
\author{An.~Ianni}\affiliation{\Princeton}\affiliation{\AQLNGS}
\author{V.~Ippolito}\affiliation{\RMUnoINFN}
%\author{T.N.~Johnson}\affiliation{\UCDavis}
\author{K.~Keeter}\affiliation{\BHSU}
\author{C.L.~Kendziora}\affiliation{\FNAL}
\author{I.~Kochanek}\affiliation{\AQLNGS}
%\author{G.~Koh}\affiliation{\Princeton}
\author{D.~Korablev}\affiliation{\JINR}
\author{G.~Korga}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{A.~Kubankin}\affiliation{\Belgorod}
\author{M.~Kuss}\affiliation{\PIINFN}
\author{M.~La~Commara}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{M.~Lai}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{X.~Li}\affiliation{\Princeton}
\author{M.~Lissia}\affiliation{\CAINFN}
\author{G.~Longo}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
%\author{A.A.~Machado}\affiliation{\Campinas}
\author{I.N.~Machulin}\affiliation{\Kurchatov}\affiliation{\MEPhI}
%\author{A.~Mandarano}\affiliation{\AQGSSI}\affiliation{\AQLNGS}
\author{L.~Mapelli}\affiliation{\Princeton}\affiliation{\CAINFN}
\author{S.M.~Mari}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{J.~Maricic}\affiliation{\Hawaii}
\author{C.J.~Martoff}\affiliation{\Temple}
\author{A.~Messina}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{P.D.~Meyers}\affiliation{\Princeton}
\author{R.~Milincic}\affiliation{\Hawaii}
%\author{A.~Monte}\affiliation{\FNAL}\affiliation{\UMass}
\author{M.~Morrocchi}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{V.N.~Muratova}\affiliation{\Petersburg}
\author{P.~Musico}\affiliation{\GEINFN}
\author{A.~Navrer~Agasson}\affiliation{\LPNHE}
\author{A.O.~Nozdrina}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{A.~Oleinik}\affiliation{\Belgorod}
%\author{M.~Orsini}\affiliation{\AQLNGS}
\author{F.~Ortica}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{L.~Pagani}\affiliation{\UCDavis}
\author{M.~Pallavicini}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{L.~Pandola}\affiliation{\CTLNS}
\author{E.~Pantic}\affiliation{\UCDavis}
\author{E.~Paoloni}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{K.~Pelczar}\affiliation{\AQLNGS}\affiliation{\Krakow}
\author{N.~Pelliccia}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{E.~Picciau}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{A.~Pocar}\affiliation{\UMass}
\author{S.~Pordes}\affiliation{\FNAL}
\author{S.S.~Poudel}\affiliation{\Houston}
%\author{H.~Qian}\affiliation{\Princeton}
\author{F.~Ragusa}\affiliation{\MIUni}\affiliation{\MIINFN}
\author{M.~Razeti}\affiliation{\CAINFN}
\author{A.~Razeto}\affiliation{\AQLNGS}
\author{A.L.~Renshaw}\affiliation{\Houston}
\author{M.~Rescigno}\affiliation{\RMUnoINFN}
%\author{Q.~Riffard}\affiliation{\APC}
\author{A.~Romani}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
%\author{B.~Rossi}\affiliation{\NAINFN}
%\author{N.~Rossi}\affiliation{\RMUnoINFN}
\author{D.~Sablone}\affiliation{\Princeton}\affiliation{\AQLNGS}
\author{O.~Samoylov}\affiliation{\JINR}
\author{W.~Sands}\affiliation{\Princeton}
\author{S.~Sanfilippo}\affiliation{\RMTreUni}\affiliation{\RMTreINFN}
\author{C.~Savarese}\affiliation{\AQGSSI}\affiliation{\AQLNGS}\affiliation{\Princeton}
\author{B.~Schlitzer}\affiliation{\UCDavis}
%\author{E.~Segreto}\affiliation{\Campinas}
\author{D.A.~Semenov}\affiliation{\Petersburg}
\author{A.~Shchagin}\affiliation{\Belgorod}
\author{A.~Sheshukov}\affiliation{\JINR}
%\author{P.N.~Singh}\affiliation{\Houston}
\author{M.D.~Skorokhvatov}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{O.~Smirnov}\affiliation{\JINR}
\author{A.~Sotnikov}\affiliation{\JINR}
%\author{C.~Stanford}\affiliation{\Princeton}
\author{S.~Stracka}\affiliation{\PIINFN}
\author{Y.~Suvorov}\affiliation{\NAUniPHY}\affiliation{\NAINFN}\affiliation{\Kurchatov}
\author{R.~Tartaglia}\affiliation{\AQLNGS}
\author{G.~Testera}\affiliation{\GEINFN}
\author{A.~Tonazzo}\affiliation{\APC}
%\author{P.~Trinchese}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{E.V.~Unzhakov}\affiliation{\Petersburg}
%\author{M.~Verducci}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{A.~Vishneva}\affiliation{\JINR}
\author{R.B.~Vogelaar}\affiliation{\VTech}
\author{M.~Wada}\affiliation{\Princeton}\affiliation{\CAINFN}
%\author{T.J.~Waldrop}\affiliation{\Augustana}
\author{H.~Wang}\affiliation{\UCLA}
\author{Y.~Wang}\affiliation{\UCLA}
%\author{A.W.~Watson}\affiliation{\Temple}
\author{S.~Westerdale}\affiliation{\Princeton}
\author{M.M.~Wojcik}\affiliation{\Krakow}
%\author{X.~Xiang}\affiliation{\Princeton}
\author{X.~Xiao}\affiliation{\UCLA}
\author{C.~Yang}\affiliation{\IHEP}
%\author{Z.~Ye}\affiliation{\Houston}
%\author{C.~Zhu}\affiliation{\Princeton}
\author{G.~Zuzel}\affiliation{\Krakow}


==> Bibliography/AU-20k.tex <==
\author{C.~E.~Aalseth}\affiliation{\PNNLaddress}
\author{S.~Abdelhakim}\affiliation{\IPNO}
\author{F.~Acerbi}\affiliation{\TNFBK}\affiliation{\TNTIFPA}
\author{P.~Agnes}\affiliation{\Houston}
\author{I.~F.~M.~Albuquerque}\affiliation{\USP}
\author{T.~Alexander}\affiliation{\PNNLaddress}
\author{A.~Alici}\affiliation{\BOUniPHY}\affiliation{\BOINFN}
\author{A.~K.~Alton}\affiliation{\Augustana}
\author{P.~Amaudruz}\affiliation{\TRIUMFaddress}
\author{F.~Ameli}\affiliation{\RMUnoINFN}
\author{P.~Antonioli}\affiliation{\BOINFN}
\author{S.~Arcelli}\affiliation{\BOUniPHY}\affiliation{\BOINFN}
\author{R.~Ardito}\affiliation{\MIPoliICA}\affiliation{\MIINFN}
\author{I.~J.~Arnquist}\affiliation{\PNNLaddress}
\author{P.~Arpaia}\affiliation{\NAUniEEIT}\affiliation{\NAINFN}
\author{D.~M.~Asner}\affiliation{\BNLaddress}
\author{A.~Asunskis}\affiliation{\BHSU}
\author{M.~Ave}\affiliation{\USP}
\author{H.~O.~Back}\affiliation{\PNNLaddress}
\author{A.~Barrado~Olmedo}\affiliation{\CIEMAT}
\author{G.~Batignani}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{M.~G.~Bisogni}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{V.~Bocci}\affiliation{\RMUnoINFN}
\author{A.~Bondar}\affiliation{\BINP}\affiliation{\NSU}
\author{G.~Bonfini}\affiliation{\AQLNGS}
\author{W.~Bonivento}\affiliation{\CAINFN}
\author{B.~Bottino}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{M.~G.~Boulay}\affiliation{\Carleton}
\author{R.~Bunker}\affiliation{\PNNLaddress}
\author{S.~Bussino}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{A.~Buzulutskov}\affiliation{\BINP}\affiliation{\NSU}
\author{M.~Cadeddu}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{M.~Cadoni}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{A.~Caminata}\affiliation{\GEINFN}
\author{N.~Canci}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{A.~Candela}\affiliation{\AQLNGS}
\author{C.~Cantini}\affiliation{\ETHZ}
\author{M.~Caravati}\affiliation{\CAINFN}
\author{M.~Cariello}\affiliation{\GEINFN}
\author{M.~Carpinelli}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{A.~Castellani}\affiliation{\MIPoliICA}\affiliation{\MIINFN}
\author{P.~Castello}\affiliation{\CAUniELE}\affiliation{\CAINFN}
\author{S.~Catalanotti}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{V.~Cataudella}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{P.~Cavalcante}\affiliation{\VTech}\affiliation{\AQLNGS}
\author{S.~Cavuoti}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{S.~Cebrian}\affiliation{\Zaragoza}
\author{B.~Celano}\affiliation{\NAINFN}
\author{R.~Cereseto}\affiliation{\GEINFN}
\author{W.~Cheng}\affiliation{\TOINFN}\affiliation{\TOPoli}
\author{A.~Chepurnov}\affiliation{\MSU}
\author{C.~Cical\`o}\affiliation{\CAINFN}
\author{L.~Cifarelli}\affiliation{\BOUniPHY}\affiliation{\BOINFN}
\author{M.~Citterio}\affiliation{\MIINFN}
\author{A.~G.~Cocco}\affiliation{\NAINFN}
\author{M.~Colocci}\affiliation{\BOUniPHY}\affiliation{\BOINFN}
\author{L.~Consiglio}\affiliation{\AQGSSI}
\author{F.~Cossio}\affiliation{\TOINFN}\affiliation{\TOPoli}
\author{G.~Covone}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{P.~Crivelli}\affiliation{\ETHZ}
\author{I.~D'Antone}\affiliation{\BOINFN}
\author{M.~D'Incecco}\affiliation{\AQLNGS}
\author{D.~D'Urso}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{M.~D.~Da~Rocha~Rolo}\affiliation{\TOINFN}
\author{M.~Daniel}\affiliation{\CIEMAT}
\author{S.~Davini}\affiliation{\GEINFN}
\author{A.~De~Candia}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{S.~De~Cecco}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{M.~De~Deo}\affiliation{\AQLNGS}
\author{A.~De~Falco}\affiliation{\CAINFN}\affiliation{\CAUniPHY}
\author{G.~De~Filippis}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{D.~De~Gruttola}\affiliation{\SAINFN}
\author{G.~De~Guido}\affiliation{\MIPoliCHE}\affiliation{\MIINFN}
\author{G.~De~Rosa}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{G.~Dellacasa}\affiliation{\TOINFN}
\author{P.~Demontis}\affiliation{\SSUniCHP}\affiliation{\CTLNS}\affiliation{\INSTM}
\author{S.~DePaquale}\affiliation{\SAINFN}
\author{A.~V.~Derbin}\affiliation{\Petersburg}
\author{A.~Devoto}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{F.~Di~Eusanio}\affiliation{\Princeton}\affiliation{\AQLNGS}
\author{G.~Di~Pietro}\affiliation{\AQLNGS}\affiliation{\MIINFN}
\author{P.~Di~Stefano}\affiliation{\Queens}
\author{C.~Dionisi}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{F.~Dordei}\affiliation{\CAINFN}
\author{M.~Downing}\affiliation{\UMass}
\author{F.~Edalatfar}\affiliation{\TRIUMFaddress}
\author{A.~Empl}\affiliation{\Houston}
\author{M.~Fernandez~Diaz}\affiliation{\CIEMAT}
\author{A.~Ferri}\affiliation{\TNFBK}\affiliation{\TNTIFPA}
\author{C.~Filip}\affiliation{\Cluj}
\author{G.~Fiorillo}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{K.~Fomenko}\affiliation{\JINR}
\author{A.~Franceschi}\affiliation{\LNFINFN}
\author{D.~Franco}\affiliation{\APC}
\author{G.~E.~Froudakis}\affiliation{\UOC}
\author{F.~Gabriele}\affiliation{\AQLNGS}
\author{A.~Gabrieli}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{C.~Galbiati}\affiliation{\Princeton}\affiliation{\AQGSSI}
\author{P.~Garcia~Abia}\affiliation{\CIEMAT}
\author{D.~Gasc\'on~Fora}\affiliation{\UB}
\author{A.~Gendotti}\affiliation{\ETHZ}
\author{C.~Ghiano}\affiliation{\AQLNGS}
\author{A.~Ghisi}\affiliation{\MIPoliICA}\affiliation{\MIINFN}
\author{S.~Giagu}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{P.~Giampa}\affiliation{\TRIUMFaddress}
\author{R.~A.~Giampaolo}\affiliation{\TOINFN}
\author{C.~Giganti}\affiliation{\LPNHE}
\author{M.~A.~Giorgi}\affiliation{\PIUniPHY}\affiliation{\PIINFN}
\author{G.~K.~Giovanetti}\affiliation{\Princeton}
\author{M.~L.~Gligan}\affiliation{\Cluj}
\author{A.~Gola}\affiliation{\TNFBK}\affiliation{\TNTIFPA}
\author{O.~Gorchakov}\affiliation{\JINR}
\author{M.~Grab}\affiliation{\Krakow}
\author{R.~Graciani~Diaz}\affiliation{\UB}
\author{F.~Granato}\affiliation{\Temple}
\author{M.~Grassi}\affiliation{\PIINFN}
\author{J.~W.~Grate}\affiliation{\PNNLaddress}
\author{G.~Y.~Grigoriev}\affiliation{\Kurchatov}
\author{M.~Gromov}\affiliation{\MSU}
\author{M.~Guan}\affiliation{\IHEP}
\author{M.~B.~B.~Guerra}\affiliation{\BHSU}
\author{M.~Guerzoni}\affiliation{\BOINFN}
\author{M.~Gulino}\affiliation{\ENUniCEE}\affiliation{\CTLNS}
\author{R.~K.~Haaland}\affiliation{\FortLewis}
\author{B.~R.~Hackett}\affiliation{\Hawaii}
\author{A.~Hallin}\affiliation{\Alberta}
\author{B.~Harrop}\affiliation{\Princeton}
\author{E.~W.~Hoppe}\affiliation{\PNNLaddress}
\author{S.~Horikawa}\affiliation{\AQGSSI}\affiliation{\AQLNGS}
\author{B.~Hosseini}\affiliation{\CAINFN}
\author{F.~Hubaut}\affiliation{\CPPM}
\author{P.~Humble}\affiliation{\PNNLaddress}
\author{E.~V.~Hungerford}\affiliation{\Houston}
\author{An.~Ianni}\affiliation{\Princeton}\affiliation{\AQLNGS}
\author{V.~Ippolito}\affiliation{\RMUnoINFN}
\author{C.~Jillings}\affiliation{\Laurentian}\affiliation{\SNOLABaddress}
\author{S.~Jimenez~Cabre}\affiliation{\CIEMAT}
\author{K.~Keeter}\affiliation{\BHSU}
\author{C.~L.~Kendziora}\affiliation{\FNALaddress}
\author{S.~Kim}\affiliation{\Temple}
\author{I.~Kochanek}\affiliation{\AQLNGS}
\author{K.~Kondo}\affiliation{\AQGSSI}
\author{G.~Kopp}\affiliation{\Princeton}
\author{D.~Korablev}\affiliation{\JINR}
\author{G.~Korga}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{A.~Kubankin}\affiliation{\Belgorod}
\author{R.~Kugathasan}\affiliation{\TOINFN}\affiliation{\TOPoli}
\author{M.~Kuss}\affiliation{\PIINFN}
\author{M.~Kuzniak}\affiliation{\Carleton}
\author{M.~La~Commara}\affiliation{\NAUniPHARM}\affiliation{\NAINFN}
\author{M.~Lai}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{S.~Langrock}\affiliation{\Laurentian}\affiliation{\SNOLABaddress}
\author{M.~Lebois}\affiliation{\IPNO}
\author{B.~Lehnert}\affiliation{\Alberta}
\author{X.~Li}\affiliation{\Princeton}
\author{Q.~Liqiang}\affiliation{\IPNO}
\author{M.~Lissia}\affiliation{\CAINFN}
\author{G.~U.~Lodi}\affiliation{\MIPoliCHE}\affiliation{\MIINFN}
\author{G.~Longo}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{R.~Lussana}\affiliation{\MIPoliEIB}\affiliation{\MIINFN}
\author{L.~Luzzi}\affiliation{\MIPoliENE}\affiliation{\MIINFN}
\author{A.~A.~Machado}\affiliation{\Campinas}
\author{I.~N.~Machulin}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{A.~Mandarano}\affiliation{\AQGSSI}\affiliation{\AQLNGS}
\author{L.~Mapelli}\affiliation{\Princeton}
\author{M.~Marcante}\affiliation{\TNUni}\affiliation{\TNTIFPA}\affiliation{\TNFBK}
\author{A.~Margotti}\affiliation{\BOINFN}
\author{S.~M.~Mari}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{M.~Mariani}\affiliation{\MIPoliENE}\affiliation{\MIINFN}
\author{J.~Maricic}\affiliation{\Hawaii}
\author{M.~Marinelli}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{D.~Marras}\affiliation{\CAINFN}
\author{A.~D.~Martinez~Rojas}\affiliation{\TOINFN}\affiliation{\TOPoli}
\author{C.~J.~Martoff}\affiliation{\Temple}
\author{M.~Mascia}\affiliation{\CAUniCHE}\affiliation{\CAINFN}
\author{A.~Masoni}\affiliation{\CAINFN}
\author{A.~Mazzi}\affiliation{\TNFBK}\affiliation{\TNTIFPA}
\author{A.~B.~McDonald}\affiliation{\Queens}
\author{A.~Messina}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{P.~D.~Meyers}\affiliation{\Princeton}
\author{T.~Miletic}\affiliation{\Hawaii}
\author{R.~Milincic}\affiliation{\Hawaii}
\author{A.~Moggi}\affiliation{\PIINFN}
\author{S.~Moioli}\affiliation{\MIPoliCHE}\affiliation{\MIINFN}
\author{J.~Monroe}\affiliation{\RHUL}
\author{M.~Morrocchi}\affiliation{\PIINFN}
\author{T.~Mroz}\affiliation{\Krakow}
\author{W.~Mu}\affiliation{\ETHZ}
\author{V.~N.~Muratova}\affiliation{\Petersburg}
\author{S.~Murphy}\affiliation{\ETHZ}
\author{C.~Muscas}\affiliation{\CAUniELE}\affiliation{\CAINFN}
\author{P.~Musico}\affiliation{\GEINFN}
\author{R.~Nania}\affiliation{\BOINFN}
\author{T.~Napolitano}\affiliation{\LNFINFN}
\author{A.~Navrer~Agasson}\affiliation{\LPNHE}
\author{M.~Nessi}\affiliation{\CERNaddress}
\author{I.~Nikulin}\affiliation{\Belgorod}
\author{A.~O.~Nozdrina}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{N.~N.~Nurakhov}\affiliation{\Kurchatov}
\author{A.~Oleinik}\affiliation{\Belgorod}
\author{V.~Oleynikov}\affiliation{\BINP}\affiliation{\NSU}
\author{M.~Orsini}\affiliation{\AQLNGS}
\author{F.~Ortica}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{L.~Pagani}\affiliation{\UCDavis}
\author{M.~Pallavicini}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{S.~Palmas}\affiliation{\CAUniCHE}\affiliation{\CAINFN}
\author{L.~Pandola}\affiliation{\CTLNS}
\author{E.~Pantic}\affiliation{\UCDavis}
\author{E.~Paoloni}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{G.~Paternoster}\affiliation{\TNFBK}\affiliation{\TNTIFPA}
\author{V.~Pavletcov}\affiliation{\MSU}
\author{F.~Pazzona}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{S.~Peeters}\affiliation{\Sussex}
\author{P.~A.~Pegoraro}\affiliation{\CAUniELE}\affiliation{\CAINFN}
\author{K.~Pelczar}\affiliation{\AQLNGS}
\author{L.~A.~Pellegrini}\affiliation{\MIPoliCHE}\affiliation{\MIINFN}
\author{N.~Pelliccia}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{F.~Perotti}\affiliation{\MIPoliICA}\affiliation{\MIINFN}
\author{V.~Pesudo}\affiliation{\CIEMAT}
\author{E.~Picciau}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{C.~Piemonte}\affiliation{\TNFBK}\affiliation{\TNTIFPA}
\author{F.~Pietropaolo}\affiliation{\CERNaddress}
\author{A.~Pocar}\affiliation{\UMass}
\author{T.~Pollman}\affiliation{\TUM}
\author{D.~Portaluppi}\affiliation{\MIPoliEIB}\affiliation{\MIINFN}
\author{S.~S.~Poudel}\affiliation{\Houston}
\author{P.~Pralavorio}\affiliation{\CPPM}
\author{D.~Price}\affiliation{\Manchester}
\author{D.~A.~Pugachev}\affiliation{\Kurchatov}
\author{B.~Radics}\affiliation{\ETHZ}
\author{F.~Raffaelli}\affiliation{\PIINFN}
\author{F.~Ragusa}\affiliation{\MIUni}\affiliation{\MIINFN}
\author{M.~Razeti}\affiliation{\CAINFN}
\author{A.~Razeto}\affiliation{\AQLNGS}
\author{V.~Regazzoni}\affiliation{\TNUni}\affiliation{\TNTIFPA}\affiliation{\TNFBK}
\author{C.~Regenfus}\affiliation{\ETHZ}
\author{A.~L.~Renshaw}\affiliation{\Houston}
\author{S.~Rescia}\affiliation{\BNLaddress}
\author{M.~Rescigno}\affiliation{\RMUnoINFN}
\author{F.~Retiere}\affiliation{\TRIUMFaddress}
\author{Q.~Riffard}\affiliation{\APC}
\author{A.~Rivetti}\affiliation{\TOINFN}
\author{A.~Romani}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{L.~Romero}\affiliation{\CIEMAT}
\author{N.~Rossi}\affiliation{\RMUnoINFN}\affiliation{\AQLNGS}
\author{A.~Rubbia}\affiliation{\ETHZ}
\author{D.~Sablone}\affiliation{\Temple}\affiliation{\AQLNGS}
\author{P.~Sala}\affiliation{\CERNaddress}
\author{P.~Salatino}\affiliation{\NAUniCHE}\affiliation{\NAINFN}
\author{O.~Samoylov}\affiliation{\JINR}
\author{E.~S\`anchez~Garc\`ia}\affiliation{\CIEMAT}
\author{S.~Sanfilippo}\affiliation{\RMTreUni}\affiliation{\RMTreINFN}
\author{M.~Sant}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{D.~Santone}\affiliation{\RHUL}
\author{R.~Santorelli}\affiliation{\CIEMAT}
\author{C.~Savarese}\affiliation{\Princeton}
\author{E.~Scapparone}\affiliation{\BOINFN}
\author{B.~Schlitzer}\affiliation{\UCDavis}
\author{G.~Scioli}\affiliation{\BOUniPHY}\affiliation{\BOINFN}
\author{E.~Segreto}\affiliation{\Campinas}
\author{A.~Seifert}\affiliation{\PNNLaddress}
\author{D.~A.~Semenov}\affiliation{\Petersburg}
\author{A.~Shchagin}\affiliation{\Belgorod}
\author{E.~Shemyakina}\affiliation{\BINP}\affiliation{\NSU}
\author{A.~Sheshukov}\affiliation{\JINR}
\author{S.~Siddhanta}\affiliation{\CAINFN}
\author{M.~Simeone}\affiliation{\NAUniCHE}\affiliation{\NAINFN}
\author{P.~N.~Singh}\affiliation{\Houston}
\author{P.~Skensved}\affiliation{\Queens}
\author{M.~D.~Skorokhvatov}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{O.~Smirnov}\affiliation{\JINR}
\author{G.~Sobrero}\affiliation{\GEINFN}
\author{A.~Sokolov}\affiliation{\BINP}\affiliation{\NSU}
\author{A.~Sotnikov}\affiliation{\JINR}
\author{R.~Stainforth}\affiliation{\Carleton}
\author{S.~Stracka}\affiliation{\PIINFN}
\author{G.~B.~Suffritti}\affiliation{\SSUniCHP}\affiliation{\CTLNS}\affiliation{\INSTM}
\author{S.~Sulis}\affiliation{\CAUniELE}\affiliation{\CAINFN}
\author{Y.~Suvorov}\affiliation{\NAUniPHY}\affiliation{\NAINFN}\affiliation{\Kurchatov}
\author{A.M.~Szelc}\affiliation{\Manchester}
\author{R.~Tartaglia}\affiliation{\AQLNGS}
\author{G.~Testera}\affiliation{\GEINFN}
\author{T.~Thorpe}\affiliation{\AQGSSI}\affiliation{\AQLNGS}
\author{A.~Tonazzo}\affiliation{\APC}
\author{A.~Tosi}\affiliation{\MIPoliEIB}\affiliation{\MIINFN}
\author{E.~V.~Unzhakov}\affiliation{\Petersburg}
\author{G.~Usai}\affiliation{\CAINFN}\affiliation{\CAUniPHY}
\author{A.~Vacca}\affiliation{\CAUniCHE}\affiliation{\CAINFN}
\author{E.~V\'azquez-J\'auregui}\affiliation{\UNAM}
\author{M.~Verducci}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{T.~Viant}\affiliation{\ETHZ}
\author{S.~Viel}\affiliation{\Carleton}
\author{F.~Villa}\affiliation{\MIPoliEIB}\affiliation{\MIINFN}
\author{A.~Vishneva}\affiliation{\JINR}
\author{B.~Vogelaar}\affiliation{\VTech}
\author{M.~Wada}\affiliation{\CAINFN}
\author{J.~Wahl}\affiliation{\PNNLaddress}
\author{J.~J.~Walding}\affiliation{\RHUL}
\author{H.~Wang}\affiliation{\UCLA}
\author{Y.~Wang}\affiliation{\UCLA}
\author{S.~Westerdale}\affiliation{\Carleton}
\author{R.~J.~Wheadon}\affiliation{\TOINFN}
\author{R.~Williams}\affiliation{\PNNLaddress}
\author{J.~Wilson}\affiliation{\IPNO}
\author{Marcin~Wojcik}\affiliation{\Krakow}
\author{Mariusz~Wojcik}\affiliation{\Lodz}
\author{S.~Wu}\affiliation{\ETHZ}
\author{X.~Xiao}\affiliation{\UCLA}
\author{C.~Yang}\affiliation{\IHEP}
\author{Z.~Ye}\affiliation{\Houston}
\author{G.~Zuzel}\affiliation{\Krakow}

==> Bibliography/AU-50-Low-MassPaper.tex <==
\author{P.~Agnes}\affiliation{\Houston}
\author{I.~F.~M.~Albuquerque}\affiliation{\USP}
\author{T.~Alexander}\affiliation{\PNNL}
\author{A.~K.~Alton}\affiliation{\Augustana}
\author{G.~R.~Araujo}\affiliation{\USP}
\author{D.~M.~Asner}\affiliation{\Bnl}
\author{M.~Ave}\affiliation{\USP}
\author{H.~O.~Back}\affiliation{\PNNL}
\author{B.~Baldin}\altaffiliation{Current address: Raleigh, NC 27613-3133, USA}\affiliation{\Fnal}
\author{G.~Batignani}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{K.~Biery}\affiliation{\Fnal}
\author{V.~Bocci}\affiliation{\RMUnoINFN}
\author{G.~Bonfini}\affiliation{\AQLNGS}
\author{W.~Bonivento}\affiliation{\CAINFN}
\author{B.~Bottino}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{F.~Budano}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{S.~Bussino}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{M.~Cadeddu}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{M.~Cadoni}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{F.~Calaprice}\affiliation{\Princeton}
\author{A.~Caminata}\affiliation{\GEINFN}
\author{N.~Canci}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{A.~Candela}\affiliation{\AQLNGS}
\author{M.~Caravati}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{M.~Cariello}\affiliation{\GEINFN}
\author{M.~Carlini}\affiliation{\AQLNGS}
\author{M.~Carpinelli}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{S.~Catalanotti}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{V.~Cataudella}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{P.~Cavalcante}\affiliation{\VTech}\affiliation{\AQLNGS}
\author{S.~Cavuoti}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{R.~Cereseto}\affiliation{\GEINFN}
\author{A.~Chepurnov}\affiliation{\MSU}
\author{C.~Cical\`o}\affiliation{\CAINFN}
\author{L.~Cifarelli}\affiliation{\BOUniPHY}\affiliation{\BOINFN}
\author{A.~G.~Cocco}\affiliation{\NAINFN}
\author{G.~Covone}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{D.~D'Angelo}\affiliation{\MIUni}\affiliation{\MIINFN}
\author{M.~D'Incecco}\affiliation{\AQLNGS}
\author{D.~D'Urso}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{S.~Davini}\affiliation{\GEINFN}
\author{A.~De~Candia}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{S.~De~Cecco}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{M.~De~Deo}\affiliation{\AQLNGS}
\author{G.~De~Filippis}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{G.~De~Rosa}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{M.~De~Vincenzi}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{P.~Demontis}\affiliation{\SSUniCHP}\affiliation{\CTLNS}\affiliation{\INSTM}
\author{A.~V.~Derbin}\affiliation{\Petersburg}
\author{A.~Devoto}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{F.~Di~Eusanio}\affiliation{\Princeton}
\author{G.~Di~Pietro}\affiliation{\AQLNGS}\affiliation{\MIINFN}
\author{C.~Dionisi}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{M.~Downing}\affiliation{\UMass}
\author{E.~Edkins}\affiliation{\Hawaii}
\author{A.~Empl}\affiliation{\Houston}
\author{A.~Fan}\affiliation{\UCLA}
\author{G.~Fiorillo}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{K.~Fomenko}\affiliation{\JINR}
\author{D.~Franco}\affiliation{\APC}
\author{F.~Gabriele}\affiliation{\AQLNGS}
\author{A.~Gabrieli}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{C.~Galbiati}\affiliation{\Princeton}\affiliation{\AQGSSI}
\author{P.~Garcia~Abia}\affiliation{\CIEMAT}
\author{C.~Ghiano}\affiliation{\AQLNGS}
\author{S.~Giagu}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{C.~Giganti}\affiliation{\LPNHE}
\author{G.~K.~Giovanetti}\affiliation{\Princeton}
\author{O.~Gorchakov}\affiliation{\JINR}
\author{A.~M.~Goretti}\affiliation{\AQLNGS}
\author{F.~Granato}\affiliation{\Temple}
\author{M.~Gromov}\affiliation{\MSU}
\author{M.~Guan}\affiliation{\IHEP}
\author{Y.~Guardincerri}\altaffiliation{Deceased.}\affiliation{\Fnal}
\author{M.~Gulino}\affiliation{\ENUniCEE}\affiliation{\CTLNS}
\author{B.~R.~Hackett}\affiliation{\Hawaii}
\author{M.~H.~Hassanshahi}\affiliation{\AQLNGS}
\author{K.~Herner}\affiliation{\Fnal}
\author{B.~Hosseini}\affiliation{\CAINFN}
\author{D.~Hughes}\affiliation{\Princeton}
\author{P.~Humble}\affiliation{\PNNL}
\author{E.~V.~Hungerford}\affiliation{\Houston}
\author{Al.~Ianni}\affiliation{\AQLNGS}
\author{An.~Ianni}\affiliation{\Princeton}\affiliation{\AQLNGS}
\author{V.~Ippolito}\affiliation{\RMUnoINFN}
\author{I.~James}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{T.~N.~Johnson}\affiliation{\UCDavis}
\author{Y.~Kahn}\affiliation{\Princeton}
\author{K.~Keeter}\affiliation{\BHSU}
\author{C.~L.~Kendziora}\affiliation{\Fnal}
\author{I.~Kochanek}\affiliation{\AQLNGS}
\author{G.~Koh}\affiliation{\Princeton}
\author{D.~Korablev}\affiliation{\JINR}
\author{G.~Korga}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{A.~Kubankin}\affiliation{\Belgorod}
\author{M.~Kuss}\affiliation{\PIINFN}
\author{M.~La~Commara}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{M.~Lai}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{X.~Li}\affiliation{\Princeton}
\author{M.~Lisanti}\affiliation{\Princeton}
\author{M.~Lissia}\affiliation{\CAINFN}
\author{B.~Loer}\affiliation{\PNNL}
\author{G.~Longo}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{Y.~Ma}\affiliation{\IHEP}
\author{A.~A.~Machado}\affiliation{\Campinas}
\author{I.~N.~Machulin}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{A.~Mandarano}\affiliation{\AQGSSI}\affiliation{\AQLNGS}
\author{L.~Mapelli}\affiliation{\Princeton}
\author{S.~M.~Mari}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{J.~Maricic}\affiliation{\Hawaii}
\author{C.~J.~Martoff}\affiliation{\Temple}
\author{A.~Messina}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{P.~D.~Meyers}\affiliation{\Princeton}
\author{R.~Milincic}\affiliation{\Hawaii}
\author{S.~Mishra-Sharma}\affiliation{\Princeton}
\author{A.~Monte}\affiliation{\UMass}
\author{M.~Morrocchi}\affiliation{\PIINFN}
\author{B.~J.~Mount}\affiliation{\BHSU}
\author{V.~N.~Muratova}\affiliation{\Petersburg}
\author{P.~Musico}\affiliation{\GEINFN}
\author{R.~Nania}\affiliation{\BOINFN}
\author{A.~Navrer~Agasson}\affiliation{\LPNHE}
\author{A.~O.~Nozdrina}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{A.~Oleinik}\affiliation{\Belgorod}
\author{M.~Orsini}\affiliation{\AQLNGS}
\author{F.~Ortica}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{L.~Pagani}\affiliation{\UCDavis}
\author{M.~Pallavicini}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{L.~Pandola}\affiliation{\CTLNS}
\author{E.~Pantic}\affiliation{\UCDavis}
\author{E.~Paoloni}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{F.~Pazzona}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{K.~Pelczar}\affiliation{\AQLNGS}
\author{N.~Pelliccia}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{V.~Pesudo}\affiliation{\CIEMAT}
\author{A.~Pocar}\affiliation{\UMass}
\author{S.~Pordes}\affiliation{\Fnal}
\author{S.~S.~Poudel}\affiliation{\Houston}
\author{D.~A.~Pugachev}\affiliation{\Kurchatov}
\author{H.~Qian}\affiliation{\Princeton}
\author{F.~Ragusa}\affiliation{\MIUni}\affiliation{\MIINFN}
\author{M.~Razeti}\affiliation{\CAINFN}
\author{A.~Razeto}\affiliation{\AQLNGS}
\author{B.~Reinhold}\affiliation{\Hawaii}
\author{A.~L.~Renshaw}\affiliation{\Houston}
\author{M.~Rescigno}\affiliation{\RMUnoINFN}
\author{Q.~Riffard}\affiliation{\APC}
\author{A.~Romani}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{B.~Rossi}\affiliation{\NAINFN}
\author{N.~Rossi}\affiliation{\RMUnoINFN}
\author{D.~Sablone}\affiliation{\Princeton}\affiliation{\AQLNGS}
\author{O.~Samoylov}\affiliation{\JINR}
\author{W.~Sands}\affiliation{\Princeton}
\author{S.~Sanfilippo}\affiliation{\RMTreUni}\affiliation{\RMTreINFN}
\author{M.~Sant}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{R.~Santorelli}\affiliation{\CIEMAT}
\author{C.~Savarese}\affiliation{\AQGSSI}\affiliation{\AQLNGS}
\author{E.~Scapparone}\affiliation{\BOINFN}
\author{B.~Schlitzer}\affiliation{\UCDavis}
\author{E.~Segreto}\affiliation{\Campinas}
\author{D.~A.~Semenov}\affiliation{\Petersburg}
\author{A.~Shchagin}\affiliation{\Belgorod}
\author{A.~Sheshukov}\affiliation{\JINR}
\author{P.~N.~Singh}\affiliation{\Houston}
\author{M.~D.~Skorokhvatov}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{O.~Smirnov}\affiliation{\JINR}
\author{A.~Sotnikov}\affiliation{\JINR}
\author{C.~Stanford}\affiliation{\Princeton}
\author{S.~Stracka}\affiliation{\PIINFN}
\author{G.~B.~Suffritti}\affiliation{\SSUniCHP}\affiliation{\CTLNS}\affiliation{\INSTM}
\author{Y.~Suvorov}\affiliation{\NAUniPHY}\affiliation{\NAINFN}\affiliation{\UCLA}\affiliation{\Kurchatov}
\author{R.~Tartaglia}\affiliation{\AQLNGS}
\author{G.~Testera}\affiliation{\GEINFN}
\author{A.~Tonazzo}\affiliation{\APC}
\author{P.~Trinchese}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{E.~V.~Unzhakov}\affiliation{\Petersburg}
\author{M.~Verducci}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{A.~Vishneva}\affiliation{\JINR}
\author{B.~Vogelaar}\affiliation{\VTech}
\author{M.~Wada}\affiliation{\Princeton}
\author{T.~J.~Waldrop}\affiliation{\Augustana}
\author{H.~Wang}\affiliation{\UCLA}
\author{Y.~Wang}\affiliation{\UCLA}
\author{A.~W.~Watson}\affiliation{\Temple}
\author{S.~Westerdale}\altaffiliation{Currently at Carleton University, Ottawa, Canada.}\affiliation{\Princeton}
\author{M.~M.~Wojcik}\affiliation{\Krakow}
\author{M.~Wojcik}\affiliation{\Lodz}
\author{X.~Xiang}\affiliation{\Princeton}
\author{X.~Xiao}\affiliation{\UCLA}
\author{C.~Yang}\affiliation{\IHEP}
\author{Z.~Ye}\affiliation{\Houston}
\author{C.~Zhu}\affiliation{\Princeton}
\author{A.~Zichichi}\affiliation{\BOUniPHY}\affiliation{\BOINFN}
\author{G.~Zuzel}\affiliation{\Krakow}


==> Bibliography/AU-50.tex <==
\author{P.~Agnes}\affiliation{\Houston}
\author{I.~F.~M.~Albuquerque}\affiliation{\USP}
\author{T.~Alexander}\affiliation{\PNNL}
\author{A.~K.~Alton}\affiliation{\Augustana}
\author{G.~R.~Araujo}\affiliation{\USP}
\author{D.~M.~Asner}\affiliation{\BNL}
\author{M.~P.~Ave}\affiliation{\USP}
\author{H.~O.~Back}\affiliation{\PNNL}
\author{B.~Baldin}\affiliation{\FNAL}
\author{G.~Batignani}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{K.~Biery}\affiliation{\FNAL}
\author{V.~Bocci}\affiliation{\RMUnoINFN}
\author{G.~Bonfini}\affiliation{\AQLNGS}
\author{W.~Bonivento}\affiliation{\CAINFN}
\author{B.~Bottino}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{F.~Budano}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{S.~Bussino}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{M.~Cadeddu}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{M.~Cadoni}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{F.~Calaprice}\affiliation{\Princeton}
\author{A.~Caminata}\affiliation{\GEINFN}
\author{N.~Canci}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{A.~Candela}\affiliation{\AQLNGS}
\author{M.~Caravati}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{M.~Cariello}\affiliation{\GEINFN}
\author{M.~Carlini}\affiliation{\AQLNGS}
\author{M.~Carpinelli}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{S.~Catalanotti}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{V.~Cataudella}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{P.~Cavalcante}\affiliation{\VTech}\affiliation{\AQLNGS}
\author{S.~Cavuoti}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{A.~Chepurnov}\affiliation{\MSU}
\author{C.~Cical\`o}\affiliation{\CAINFN}
\author{A.~G.~Cocco}\affiliation{\NAINFN}
\author{G.~Covone}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{D.~D'Angelo}\affiliation{\MIUni}\affiliation{\MIINFN}
\author{M.~D'Incecco}\affiliation{\AQLNGS}
\author{D.~D'Urso}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{S.~Davini}\affiliation{\GEINFN}
\author{A.~De~Candia}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{S.~De~Cecco}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{M.~De~Deo}\affiliation{\AQLNGS}
\author{G.~De~Filippis}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{G.~De~Rosa}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{M.~De~Vincenzi}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{P.~Demontis}\affiliation{\SSUniCHP}\affiliation{\CTLNS}\affiliation{\INSTM}
\author{A.~V.~Derbin}\affiliation{\Petersburg}
\author{A.~Devoto}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{F.~Di~Eusanio}\affiliation{\Princeton}
\author{G.~Di~Pietro}\affiliation{\AQLNGS}\affiliation{\MIINFN}
\author{C.~Dionisi}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{M.~Downing}\affiliation{\UMass}
\author{E.~Edkins}\affiliation{\Hawaii}
\author{A.~Empl}\affiliation{\Houston}
\author{A.~Fan}\affiliation{\UCLA}
\author{G.~Fiorillo}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{K.~Fomenko}\affiliation{\JINR}
\author{D.~Franco}\affiliation{\APC}
\author{F.~Gabriele}\affiliation{\AQLNGS}
\author{A.~Gabrieli}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{C.~Galbiati}\affiliation{\Princeton}\affiliation{\AQGSSI}
\author{S.~Giagu}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{C.~Giganti}\affiliation{\LPNHE}
\author{G.~K.~Giovanetti}\affiliation{\Princeton}
\author{O.~Gorchakov}\affiliation{\JINR}
\author{A.~M.~Goretti}\affiliation{\AQLNGS}
\author{F.~Granato}\affiliation{\Temple}
\author{M.~Gromov}\affiliation{\MSU}
\author{M.~Guan}\affiliation{\IHEP}
\author{Y.~Guardincerri}\affiliation{\FNAL}
\author{M.~Gulino}\affiliation{\ENUniCEE}\affiliation{\CTLNS}
\author{B.~R.~Hackett}\affiliation{\Hawaii}
\author{M.~H.~Hassanshahi}\affiliation{\AQLNGS}
\author{K.~Herner}\affiliation{\FNAL}
\author{B.~Hosseini}\affiliation{\CAINFN}
\author{D.~Hughes}\affiliation{\Princeton}
\author{P.~Humble}\affiliation{\PNNL}
\author{E.~V.~Hungerford}\affiliation{\Houston}
\author{Al.~Ianni}\affiliation{\AQLNGS}
\author{An.~Ianni}\affiliation{\Princeton}\affiliation{\AQLNGS}
\author{V.~Ippolito}\affiliation{\RMUnoINFN}
\author{I.~James}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{T.~N.~Johnson}\affiliation{\UCDavis}
\author{K.~Keeter}\affiliation{\BHSU}
\author{C.~L.~Kendziora}\affiliation{\FNAL}
\author{I.~Kochanek}\affiliation{\Princeton}
\author{G.~Koh}\affiliation{\Princeton}
\author{D.~Korablev}\affiliation{\JINR}
\author{G.~Korga}\affiliation{\Houston}\affiliation{\AQLNGS}
\author{A.~Kubankin}\affiliation{\Belgorod}
\author{M.~Kuss}\affiliation{\PIINFN}
\author{M.~La~Commara}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{M.~Lai}\affiliation{\CAUniPHY}\affiliation{\CAINFN}
\author{X.~Li}\affiliation{\Princeton}
\author{M.~Lissia}\affiliation{\CAINFN}
\author{B.~Loer}\affiliation{\PNNL}
\author{G.~Longo}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{Y.~Ma}\affiliation{\IHEP}
\author{A.~A.~Machado}\affiliation{\Campinas}
\author{I.~N.~Machulin}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{A.~Mandarano}\affiliation{\AQGSSI}\affiliation{\AQLNGS}
\author{L.~Mapelli}\affiliation{\Princeton}
\author{S.~M.~Mari}\affiliation{\RMTreINFN}\affiliation{\RMTreUni}
\author{J.~Maricic}\affiliation{\Hawaii}
\author{C.~J.~Martoff}\affiliation{\Temple}
\author{A.~Messina}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{P.~D.~Meyers}\affiliation{\Princeton}
\author{R.~Milincic}\affiliation{\Hawaii}
\author{A.~Monte}\affiliation{\UMass}
\author{M.~Morrocchi}\affiliation{\PIINFN}
\author{B.~J.~Mount}\affiliation{\BHSU}
\author{V.~N.~Muratova}\affiliation{\Petersburg}
\author{P.~Musico}\affiliation{\GEINFN}
\author{A.~Navrer~Agasson}\affiliation{\LPNHE}
\author{A.~O.~Nozdrina}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{A.~Oleinik}\affiliation{\Belgorod}
\author{M.~Orsini}\affiliation{\AQLNGS}
\author{F.~Ortica}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{L.~Pagani}\affiliation{\UCDavis}
\author{M.~Pallavicini}\affiliation{\GEUni}\affiliation{\GEINFN}
\author{L.~Pandola}\affiliation{\CTLNS}
\author{E.~Pantic}\affiliation{\UCDavis}
\author{E.~Paoloni}\affiliation{\PIINFN}\affiliation{\PIUniPHY}
\author{F.~Pazzona}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{K.~Pelczar}\affiliation{\AQLNGS}
\author{N.~Pelliccia}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{A.~Pocar}\affiliation{\UMass}
\author{S.~Pordes}\affiliation{\FNAL}
\author{S.~S.~Poudel}\affiliation{\Houston}
\author{D.~A.~Pugachev}\affiliation{\Kurchatov}
\author{H.~Qian}\affiliation{\Princeton}
\author{F.~Ragusa}\affiliation{\MIUni}\affiliation{\MIINFN}
\author{M.~Razeti}\affiliation{\CAINFN}
\author{A.~Razeto}\affiliation{\AQLNGS}
\author{B.~Reinhold}\affiliation{\Hawaii}
\author{A.~L.~Renshaw}\affiliation{\Houston}
\author{M.~Rescigno}\affiliation{\RMUnoINFN}
\author{Q.~Riffard}\affiliation{\APC}
\author{A.~Romani}\affiliation{\PGUniCBB}\affiliation{\PGINFN}
\author{B.~Rossi}\affiliation{\NAINFN}
\author{N.~Rossi}\affiliation{\RMUnoINFN}
\author{D.~Sablone}\affiliation{\Princeton}\affiliation{\AQLNGS}
\author{O.~Samoylov}\affiliation{\JINR}
\author{W.~Sands}\affiliation{\Princeton}
\author{S.~Sanfilippo}\affiliation{\RMTreUni}\affiliation{\RMTreINFN}
\author{M.~Sant}\affiliation{\SSUniCHP}\affiliation{\CTLNS}
\author{C.~Savarese}\affiliation{\AQGSSI}\affiliation{\AQLNGS}
\author{B.~Schlitzer}\affiliation{\UCDavis}
\author{E.~Segreto}\affiliation{\Campinas}
\author{D.~A.~Semenov}\affiliation{\Petersburg}
\author{A.~Shchagin}\affiliation{\Belgorod}
\author{A.~Sheshukov}\affiliation{\JINR}
\author{P.~N.~Singh}\affiliation{\Houston}
\author{M.~D.~Skorokhvatov}\affiliation{\Kurchatov}\affiliation{\MEPhI}
\author{O.~Smirnov}\affiliation{\JINR}
\author{A.~Sotnikov}\affiliation{\JINR}
\author{C.~Stanford}\affiliation{\Princeton}
\author{S.~Stracka}\affiliation{\PIINFN}
\author{G.~B.~Suffritti}\affiliation{\SSUniCHP}\affiliation{\CTLNS}\affiliation{\INSTM}
\author{Y.~Suvorov}\affiliation{\NAUniPHY}\affiliation{\NAINFN}\affiliation{\Kurchatov}
\author{R.~Tartaglia}\affiliation{\AQLNGS}
\author{G.~Testera}\affiliation{\GEINFN}
\author{A.~Tonazzo}\affiliation{\APC}
\author{P.~Trinchese}\affiliation{\NAUniPHY}\affiliation{\NAINFN}
\author{E.~V.~Unzhakov}\affiliation{\Petersburg}
\author{M.~Verducci}\affiliation{\RMUnoINFN}\affiliation{\RMUnoUni}
\author{A.~Vishneva}\affiliation{\JINR}
\author{B.~Vogelaar}\affiliation{\VTech}
\author{M.~Wada}\affiliation{\Princeton}
\author{T.~J.~Waldrop}\affiliation{\Augustana}
\author{H.~Wang}\affiliation{\UCLA}
\author{Y.~Wang}\affiliation{\UCLA}
\author{A.~W.~Watson}\affiliation{\Temple}
\author{S.~Westerdale}\affiliation{\Carleton}
\author{M.~M.~Wojcik}\affiliation{\Krakow}
\author{X.~Xiang}\affiliation{\Princeton}
\author{X.~Xiao}\affiliation{\UCLA}
\author{C.~Yang}\affiliation{\IHEP}
\author{Z.~Ye}\affiliation{\Houston}
\author{C.~Zhu}\affiliation{\Princeton}
\author{G.~Zuzel}\affiliation{\Krakow}


==> chapters/Supplemental_Material.tex <==
\section{Pathological Events}
\label{sec:Appendix_Pathological}
Among the events that have been analysed in the manuscript, some of them turned out to have some strange behaviour, for which they have not been understood and categorized thoroughly. In particular, we are referring to the vertical population in fig. \ref{fig:SEC-S2} distributed between $350 \mus <\Delta t_{\mathrm{SEC}-\mathrm{S2}}<375 \mus$. 
\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{Final_figures/Pathological_Events.pdf}
\caption{Distribution of the time difference $\Delta t_{\mathrm{SEC}-\mathrm{S2}}$ vs. the time difference $\Delta t_{\mathrm{SEC}-\mathrm{S1}}$ for events with  SEC amplitude $>$70 PE.}
\label{fig:Pathological_Events}
\end{center}
\end{figure}
In fig. \ref{fig:Pathological_Events} the distribution of time requiring a SEC amplitude $>70$ PE is shown. It is visible that the majority of events is represented by S1-echo (the vertical strip at $\Delta t_{\mathrm{SEC}-\mathrm{S1}}\sim 380 \mus$), S2-echo (the horizontal strip corresponding to $\Delta t_{\mathrm{SEC}-\mathrm{S2}}\sim 380 \mus$) and the events gathered on the top-right region of the plot. As a reference, the diagonal of the plot indicates $\Delta t_{\mathrm{S2}-\mathrm{S1}}=0$), so that events close to the diagonal have been generated by interactions happened near the top of the TPC. The origin of this set of events has not a clear explanation, so it needs to be further investigated in future analyses.

==> chapters/energy.tex <==
\section{Supplementary material}
\begin{comment}
\reffiginitpar{Energy_correlation_S1_3} shows S1 vs S2 for S1-echo events while \reffig{Energy_correlation_S2_3} for  S2-echo events and \reffig{Energy_correlation_S1_S2} for  S1-S2 events.
\label{appendix:energy}
\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{Final_figures/S1vsS2e2.pdf}
 \caption{S1 charge {\it vs.} S2 charge distribution for S2-echo events. }
 \label{fig:Energy_correlation_S2_3}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{Final_figures/S1vsS2.pdf}
 \caption{S1 charge {\it vs.} S2 charge distribution for S1-echo events. }
 \label{fig:Energy_correlation_S1_3}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{Final_figures/S1vsS2c.pdf}
 \caption{S1 charge {\it vs.} S2 charge distribution for S1-S2 events. }
 \label{fig:Energy_correlation_S1_S2}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{Final_figures/chanmax.pdf}
 \caption{x vs y  distribution of standard S1 S2 events, with  $50 \mu s< \Delta t_{\mathrm{S2}-\mathrm{S1}}<$ 250 $\mu$s}
 \label{fig:S2xy}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{Final_figures/eneofS1.pdf}
 \caption{S1  distribution of events S1-echo and standard S1 S2 echo summed, with $50 \mu s<\Delta t_{\mathrm{S2}-\mathrm{S1}}<250 \mu s$. }
 \label{fig:S1_echo_ene}
\end{center}
\end{figure}
\end{comment}

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{Final_figures/S1fractiondeltat_small.pdf}
 \caption{Fraction of events with an S1-echo {\it vs.} drift time $\Delta t_{\mathrm{S2}-\mathrm{S1}}$,  with the SEC signal having its maximum in the central top PMT. The red histogram is corrected for the geometrical efficiency and divided by 100. The cuts S1$<$800 PE and S2$<$ 5000 PE are applied.}
 \label{fig:S1_fraction_small}
\end{center}
\end{figure}

\begin{comment}
\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{Final_figures/rayleigh.pdf}
 \caption{UV photon detection efficiency to hit the cathode in the area corresponding to the central PMT vs z  }
 \label{fig:rayleigh}
\end{center}
\end{figure}
\end{comment}

==> ds_macro.tex <==
%--- Packages
\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage[separate-uncertainty,retain-explicit-plus,per-mode=symbol,binary-units]{siunitx}
\usepackage[export]{adjustbox}
\usepackage{wrapfig}
\usepackage{ragged2e}
\usepackage{array,mathtools,dcolumn}
\usepackage{amsmath,amssymb}
\usepackage{wasysym}
\usepackage{stmaryrd}
\usepackage[below]{placeins}
\usepackage[table]{xcolor}
\usepackage{soul}
\usepackage{tikz}
\usepackage{afterpage}
\usepackage{lineno}
\usepackage{listings}
\usepackage{array}
\usepackage[version=4]{mhchem}
\usepackage{multirow}
\usepackage{eurosym}
\usepackage{pagecolor}
\usepackage{fancyhdr}
\usepackage{etoolbox}
\usepackage{calc}
\usepackage{dcolumn}
\newcommand\bmmax{2}
\usepackage{bm}
\usepackage{xargs}
\usepackage{xfrac}
\usepackage[colorinlistoftodos,prependcaption,textsize=small]{todonotes}
\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
\newcommand{\hatset}[1]{\accentset{\wedge}{#1}}
\newcommand{\refref}[1]{Ref.~\cite{#1}}
\newcommand{\reffig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\reftab}[1]{Table~\ref{tab:#1}}
\newcommand{\refeqn}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\refsec}[1]{Sec.~\ref{sec:#1}}
\newcommand{\refapp}[1]{\ref{app:#1}}
\usepackage{paralist}
\usepackage{tcolorbox}
\usepackage{pgfornament}
\usepackage{appendix}
%
%--- paralist
%\setlength\pltopsep{1in} 		% Space between first item and preceding paragraph
%\setlength\plpartopsep{1in} 	% Extra space added to \topsep when environment starts a new paragraph (is called in vmode).
%\setlength\plitemsep{0.5in}		% Space between successive items.
%\setlength\plparsep{0.5in}		% Space between paragraphs within an item Ð the \parskip for this environment.
%--- enumitem
\usepackage{enumitem}
\setdescription{itemsep=0pt,parsep=0pt,labelsep=.2cm,leftmargin=2.2cm,labelwidth=2cm,listparindent=.7cm}
\setlist{nolistsep,leftmargin=1cm}
\newlist{enumcompactitem}{itemize}{3}
\setlist[enumcompactitem]{topsep=0pt,partopsep=0pt,itemsep=0pt,parsep=0pt}
\setlist[enumcompactitem,1]{label=\textbullet}
\setlist[enumcompactitem,2]{label=---}
\setlist[enumcompactitem,3]{label=*}
\newlist{enumcompactdesc}{description}{3}
\setlist[enumcompactdesc]{topsep=0pt,partopsep=0pt,itemsep=0pt,parsep=0pt}
\newlist{enumcompactenum}{enumerate}{3}
\setlist[enumcompactenum]{topsep=0pt,partopsep=0pt,itemsep=0pt,parsep=0pt}
\setlist[enumcompactenum,1]{label=\arabic*}
\setlist[enumcompactenum,2]{label=\alph*}
\setlist[enumcompactenum,3]{label=\roman*}
%
\setlength\textwidth{6.5in}
\setlength\textheight{9in}
\setlength\oddsidemargin{(\paperwidth-\textwidth)/2 - 1in} 
\setlength\evensidemargin{(\paperwidth-\textwidth)/2 - 1in} 
\setlength\topmargin{(\paperheight-\textheight-\headheight-\headsep-\footskip)/2 - 1in}
%--- Language
\lstset{language=C++,basicstyle=\ttfamily}
%--- Floats Placement
\setlength\textfloatsep{5pt}
\setlength\abovecaptionskip{5pt}
%--- Counters
\newcounter{mylistcounter}
%--- Text and References
\newcommand{\myrefs}[2]{\href{http://dx.doi.org/#2}{#1}}
\newcommand{\mref}[1]{\href{http://#1}{#1}}
\newcommand{\elog}[1]{\href{https://blackhole.lngs.infn.it/DS-50kg/#1}{#1}}
\newcommand{\mrefsec}[1]{\href{https://#1}{#1}}
\newcommand{\mrefs}[2]{\href{http://#2}{#1}}
\newcommand{\arxiv}[1]{\href{http://arxiv.org/abs/#1}{arxiv:#1}}
\newcommand{\grant}[2]{#1-#2}
\newcommand{\docdb}[1]{\href{http://darkside-docdb.fnal.gov:8080/cgi-bin/ShowDocument?docid=#1}{\tt DS-DocDB\# #1}}
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}}
\newcommand{\cmo}[1]{\indent{\tt \color{red}#1}}
\newcommand{\cmf}[1]{\indent{\tt \color{blue}#1}}
\newcommand{\cmt}[2]{\indent{\tt \color{blue}#1: \color{red}#2}}
\newcommand{\chk}[1]{{\tt \color{blue}To be checked:\color{red}~#1}}
\newcommand{\fchk}[1]{{\tt \color{red}Figure to be replaced:~#1}}
\newcommand{\tba}{{\tt \color{red}tba}}
\newcommand{\event}[2]{{\tt Event\# #1, Run\# #2}}
\newcommand{\wpo}[1]{{\tt WP\##1}}
\newcommand{\wpt}[2]{{\tt WP\##1-Task\##2}}
\newcommand{\wpf}[4]{{\tt WP\##1-Task\##2 (#3) #4}}
\newcommand{\minitab}[3]{\begin{tabular}{@{}#1@{}}{#2}\\{#3}\end{tabular}}
%--- Internal Reports
\newcommand{\scx}{``Standard Cuts''}
\newcommand{\qcx}{``Quality Cuts''}
\newcommand{\pcx}{``Physics Cuts''}
\newcommand{\zcx}{``Zero Time Gap Cut''}
\newcommand{\dma}{\mbox{\tt dma}}
\newcommand{\dmb}{\mbox{\tt dmb}}
\newcommand{\dwa}{\mbox{\tt dwa}}
\newcommand{\dwb}{\mbox{\tt dwb}}
\newcommand{\etal}{et al.}
\newcommand{\aq}[1]{Answer to Question~\ref{#1}}
\newcommand{\purposecri}[1]{\noindent{\bf Purpose of Criterion:} #1\\}
\newcommand{\purposecut}[1]{\noindent{\bf Purpose of Cut:} #1\\}
\newcommand{\definitioncri}[1]{\noindent{\bf Definition of Criterion:} #1\\}
\newcommand{\definitioncut}[1]{\noindent{\bf Definition of Cut:} #1\\}
\newcommand{\impactcut}[1]{\noindent{\bf Impact of Cut:} #1\\}
\newcommand{\discussioncut}[1]{\noindent{\bf Discussion of Cut:} #1\\}
\newcommand{\precut}[1]{\noindent{\bf Pre-Cuts in Use for Determination of Acceptance of Cut:} #1\\}
\newcommand{\determinationliv}[1]{\noindent{\bf Determination of Residual Livetime after Cut:} #1\\}
\newcommand{\determinationacc}[1]{\noindent{\bf Determination of Acceptance of Cut:} #1\\}
\newcommand{\determinationfid}[1]{\noindent{\bf Determination of Fiducial Mass Set by Cut:} #1\\}
\newcommand{\determinerrliv}[1]{\noindent{\bf Determination of Error on Residual Livetime after Cut:} #1\\}
\newcommand{\determinerracc}[1]{\noindent{\bf Determination of Error on Acceptance of Cut:} #1\\}
\newcommand{\determinerrfid}[1]{\noindent{\bf Determination of Error on Fiducial Mass Set by Cut:} #1\\}
\newcommand{\fiducialcut}[1]{\noindent{\bf Fiducial Mass Set by Cut:} #1\\}
\newcommand{\acceptancecut}[1]{\noindent{\bf Acceptance of Cut:} #1\\}
\newcommand{\livetimecut}[1]{\noindent{\bf Residual Livetime after Cut:} #1\\}
%--- Software Packages
\newcommand{\FLUKA}{\mbox{FLUKA}}
\newcommand{\Geant}{\mbox{Geant4}}
\newcommand{\GFDS}{\mbox{G4DS}}
\newcommand{\SOURCES}{\mbox{SOURCES4A}}
\newcommand{\TALYS}{\mbox{TALYS}}
\newcommand{\SRIM}{\mbox{SRIM}}
\newcommand{\LabVIEW}{\mbox{NI LabVIEW}}
\newcommand{\CERNRoot}{\mbox{Root}}
%--- Functions
\newcommand{\logten}{\ensuremath{\log_{10}}}
%--- Units
\DeclareSIUnit\c{\mbox{$c$}}
\DeclareSIUnit\magn{\mbox{$\times$}}
\DeclareSIUnit\min{min}
\DeclareSIUnit\week{week}
\DeclareSIUnit\month{mo}
\DeclareSIUnit\months{mos}
\DeclareSIUnit\year{yr}
\DeclareSIUnit\years{years}
\DeclareSIUnit\yr{yr}
\DeclareSIUnit\standard{std}
\DeclareSIUnit\str{sr}
\DeclareSIUnit\ppm{ppm}
\DeclareSIUnit\ppb{ppb}
\DeclareSIUnit\ppt{ppt}
\DeclareSIUnit\pe{PE}
\DeclareSIUnit\spe{SPE}
\DeclareSIUnit\pdm{PDM}
\DeclareSIUnit\ev{events}
\DeclareSIUnit\ct{counts}
\DeclareSIUnit\neutron{\mbox{$n$}}
\DeclareSIUnit\smp{samples}
\DeclareSIUnit\Sample{S}
\DeclareSIUnit\ch{ch}
\DeclareSIUnit\hit{hit}
\DeclareSIUnit\hits{hits}
\DeclareSIUnit\bin{(\mbox{5-PE}~bin)}
\DeclareSIUnit\sgm{\mbox{$\sigma$}}
\DeclareSIUnit\rms{RMS}
\DeclareSIUnit\keVee{\mbox{keV$_{e{\rm e}}$}}
\DeclareSIUnit\keVr{\mbox{keV$_{\rm nr}$}}
\DeclareSIUnit\eVee{\mbox{eV$_{\rm ee}$}}
\DeclareSIUnit\eVr{\mbox{eV$_{\rm nr}$}}
\DeclareSIUnit\ph{photon}
\DeclareSIUnit\el{\mbox{$e^-$}}
\DeclareSIUnit\pm{\mbox{PMT}}
\DeclareSIUnit\pixel{\mbox{pixel}}
\DeclareSIUnit\inch{''}
\DeclareSIUnit\foot{'}
\DeclareSIUnit\bit{bit}
\DeclareSIUnit\sample{samples}
\DeclareSIUnit\barn{barn}
\DeclareSIUnit\bara{bar}
\DeclareSIUnit\barg{barg}
\DeclareSIUnit\mlardepth{\mbox(meter~of~\LAr~depth)}
\DeclareSIUnit\Curie{Ci}
\DeclareSIUnit\psi{psi}
\DeclareSIUnit\psf{psf}
\DeclareSIUnit\pcf{pcf}
\DeclareSIUnit\parsec{pc}
\DeclareSIUnit\mwe{\mbox{m.w.e.}}
\DeclareSIUnit\liveday{\mbox{live-days}}
\DeclareSIUnit\days{\mbox{days}}
\DeclareSIUnit\miles{\mbox{miles}}
\DeclareSIUnit\lumens{\mbox{lm}}
\DeclareSIUnit\degreeC{\mbox{$^{\circ}$C}}
\DeclareSIUnit\degreeF{\mbox{$^{\circ}$F}}
\DeclareSIUnit\electron{\mbox{$e^-$}}
\DeclareSIUnit\Euro{\mbox{\euro}}
\DeclareSIUnit\cph{cph}
\DeclareSIUnit\neq{neq}
\DeclareSIUnit\normal{\mbox{N}}
%--- Energies, Branching Ratios, and Abundances
\newcommand{\BR}{\mbox{BR}}
\newcommand{\EC}{\mbox{EC}}
\newcommand{\IgIgMax}{\mbox{$I_\gamma/I_{\gamma,{\rm max}}$}}
\newcommand{\PositronAnnihilationGammaEnergy}{\SI{511}{\keV}}
\newcommand{\PbXRayEnergy}{\SI{46}{\keV}}
\newcommand{\HOneThermalNeutronCaptureCrossSection}{\SI{0.33}{\barn}}
\newcommand{\HOneNeutronCaptureGammaEnergy}{\SI{2223}{\keV}}
\newcommand{\HOneNeutronCaptureGammaEnergyFraction}{\SI{100}{\percent}}
\newcommand{\LiSixNaturalAbundance}{\SI{7.5}{\percent}}
\newcommand{\LiSixNeutronCaptureCrossSection}{\SI{941}{\barn}}
\newcommand{\LiSixNeutronCaptureTritonEnergy}{\SI{2.73}{\MeV}}
\newcommand{\LiSixNeutronCaptureAlphaEnergy}{\SI{2.05}{\MeV}}
\newcommand{\LiSixNeutronCaptureTritonAlphaQuenchedEnergy}{\SIrange[range-units=single]{400}{500}{\keVee}}
\newcommand{\BTenNaturalAbundance}{\SI{20}{\percent}}
\newcommand{\BTenNeutronCaptureCrossSection}{\SI{3840}{\barn}}
\newcommand{\BTenNeutronCaptureGroundDecayBR}{\SI{6.4}{\percent}}
\newcommand{\BTenNeutronCaptureGroundDecayAlphaEnergy}{\SI{1775}{\keV}}
\newcommand{\BTenNeutronCaptureGroundDecayLiSevenRecoilEnergy}{\SI{1015}{\keV}}
\newcommand{\BTenNeutronCaptureExcitedDecayBR}{\SI{93.6}{\percent}}
\newcommand{\BTenNeutronCaptureExcitedDecayGammaEnergy}{\SI{478}{\keV}}
\newcommand{\BTenNeutronCaptureExcitedDecayAlphaEnergy}{\SI{1471}{\keV}}
\newcommand{\BTenNeutronCaptureExcitedDecayLiSevenRecoilEnergy}{\SI{839}{\keV}}
\newcommand{\BTenNeutronCaptureExcitedDecayAlphaQuenchedEnergy}{\SIrange[range-units=single]{30}{35}{\keVee}}
\newcommand{\BTenNeutronCaptureExcitedDecayAlphaPE}{\SIrange[range-units=single]{25}{35}{\pe}}
\newcommand{\COneTwoThermalNeutronCaptureCrossSection}{\SI{0.0034}{\barn}}
\newcommand{\COneTwoNeutronCaptureGammaEnergyOne}{\SI{3090}{\keV}}
\newcommand{\COneTwoNeutronCaptureGammaEnergyOneFraction}{\SI{100}{\percent}}
\newcommand{\COneTwoNeutronCaptureGammaEnergyTwo}{\SI{4945}{\keV}}
\newcommand{\COneTwoNeutronCaptureGammaEnergyTwoFraction}{\SI{67}{\percent}}
\newcommand{\COneTwoNeutronCaptureGammaEnergyThree}{\SI{1860}{\keV}}
\newcommand{\COneTwoNeutronCaptureGammaEnergyThreeFraction}{\SI{57}{\percent}}
\newcommand{\COneFourQValue}{\SI{156}{\keV}}
\newcommand{\FOneNineNeutronCaptureGammaEnergy}{\SI{6.6}{\MeV}}
\newcommand{\FOneNineThermalNeutronCaptureCrossSection}{\SI{0.01}{\barn}}
\newcommand{\ArThreeSevenDecay}{\EC}
\newcommand{\ArThreeSevenBR}{\SI{100}{\percent}}
\newcommand{\ArThreeSevenQValue}{\SI{2.7}{\keV}}
\newcommand{\ArThreeSevenMeanLife}{\SI{50.51(3)}{\day}}
\newcommand{\ArThreeSevenHalfLife}{\SI{35.04}{\day}}
\newcommand{\ArThreeSevenKOneBR}{\SI{81.5}{\percent}}
\newcommand{\ArThreeSevenKTwoToFourBR}{\SI{8.7}{\percent}}
\newcommand{\ArThreeSevenLCaptureXRaysEnergy}{\SI{0.27}{\keV}}
\newcommand{\ArThreeSevenKCaptureXRaysEnergy}{\SI{2.82}{\keV}}
\newcommand{\ArThreeSevenLCapturetoKCaptureRatio}{\num{0.11(1)}}
\newcommand{\ArThreeNineQValue}{\SI{565}{\keV}}
\newcommand{\ArThreeNineMeanLife}{\SI{388}{\year}}
\newcommand{\KFourZeroHalfLife}{\SI{1.25E9}{\year}}
\newcommand{\KFourZeroNaturalAbundance}{\SI{0.012}{\percent}}
\newcommand{\KFourZeroBetaQValue}{\SI{1.31}{\MeV}}
\newcommand{\KFourZeroGammaEnergy}{\SI{1.46}{\MeV}}
\newcommand{\KFourZeroXRayEnergy}{\SI{2.66}{\keV}}
\newcommand{\KFourTwoQValue}{\SI{3.5}{\MeV}}
\newcommand{\KFourTwoGammaEnergy}{\SI{1.5}{\MeV}}
\newcommand{\KFourTwoGammaBR}{\SI{18}{\percent}}
\newcommand{\FeFiveSixNeutronCaptureGammaEnergy}{\SI{7.6}{\MeV}}
\newcommand{\FeFiveSixThermalNeutronCaptureCrossSection}{\SI{2.5}{\barn}}
\newcommand{\CoFiveSevenQValue}{\SI{122}{\keV}}
\newcommand{\CoSixZeroHalfLife}{\SI{5.27}{\year}}
\newcommand{\CoSixZeroGammaOneEnergy}{\SI{1.17}{\MeV}}
\newcommand{\CoSixZeroGammaTwoEnergy}{\SI{1.33}{\MeV}}
\newcommand{\RbEightThreeMeanLife}{\SI{124.4}{\day}}
\newcommand{\RbEightFiveMGammaEnergy}{\SI{514}{\keV}}
\newcommand{\RbEightFiveMMeanLife}{\SI{1.464}{\micro\s}}
\newcommand{\KrEightThreeQValue}{\SI{41.5}{\keV}}
\newcommand{\KrEightThreeMOneMeanLife}{\SI{2.64}{\hour}}
\newcommand{\KrEightThreeMOneECEnergy}{\SI{32.1}{\keV}}
\newcommand{\KrEightThreeMTwoMeanLife}{\SI{222}{\nano\second}}
\newcommand{\KrEightThreeMTwoECEnergy}{\SI{9.4}{\keV}}
\newcommand{\KrEightThreeMOneTwoECEnergy}{\SI{41.5}{\keV}}
\newcommand{\KrEightFiveHalfLife}{\SI{10.8}{\year}}
\newcommand{\KrEightFiveGroundDecayQValue}{\SI{687}{\keV}}
\newcommand{\KrEightFiveExcitedDecayBR}{\SI{0.43}{\percent}}
\newcommand{\KrEightFiveExcitedDecayQValue}{\SI{173}{\keV}}
\newcommand{\BaOneThreeThreeHalfLife}{\SI{13.16}{\day}}
\newcommand{\BaOneThreeThreeQValue}{\SI{356}{\keV}}
\newcommand{\CsOneThreeSixQValue}{\SI{2548}{\keV}}
\newcommand{\CsOneThreeSixHalfLife}{\SI{13.2}{\day}}
\newcommand{\XeOneThreeSixQValue}{\SI{2458}{\keV}}
\newcommand{\CsOneThreeSevenQValue}{\SI{662}{\keV}}
\newcommand{\XeOneThreeSevenQValue}{\SI{4173}{\keV}}
\newcommand{\GdNatNeutronCaptureCrossSection}{\SI{48890}{\barn}}
\newcommand{\GdOneFiveFiveNeutronCaptureCrossSection}{\SI{60700}{\barn}}
\newcommand{\GdOneFiveFiveNaturalAbundance}{\SI{14.8}{\percent}}
\newcommand{\GdOneFiveFiveGammaCascadeEnergy}{\SI{8.5}{\MeV}}
\newcommand{\GdOneFiveSevenNeutronCaptureCrossSection}{\SI{254000}{\barn}}
\newcommand{\GdOneFiveSevenNaturalAbundance}{\SI{15.7}{\percent}}
\newcommand{\GdOneFiveSevenGammaCascadeEnergy}{\SI{7.9}{\MeV}}
\newcommand{\TlTwoZeroEightGammaEnergy}{\SI{2614}{\keV}}
\newcommand{\PbTwoOneZeroHalfLife}{\SI{22.3}{\yr}}
\newcommand{\PbTwoOneZeroMeanLife}{\SI{32.0}{\yr}}
\newcommand{\PoTwoOneZeroAlphaEnergy}{\SI{5.3}{\MeV}}
\newcommand{\PoTwoOneTwoAlphaEnergy}{\SI{8.78}{\MeV}}
\newcommand{\BiTwoOneTwoAlphaOneEnergy}{\SI{6.09}{\MeV}}
\newcommand{\BiTwoOneTwoAlphaTwoEnergy}{\SI{6.05}{\MeV}}
\newcommand{\BiTwoOneTwoHalfLife}{\SI{10.6}{\hour}}
\newcommand{\BiTwoOneFourGammaEnergy}{\SI{2448}{\keV}}
\newcommand{\PoTwoOneSixAlphaEnergy}{\SI{6.78}{\MeV}}
\newcommand{\RnTwoTwoZeroHalfLife}{\SI{56}{\second}}
\newcommand{\RnTwoTwoZeroAlphaEnergy}{\SI{6.29}{\MeV}}
\newcommand{\RnTwoTwoTwoHalfLife}{\SI{3.8}{\day}}
\newcommand{\RaTwoTwoFourHalfLife}{\SI{3.6}{\day}}
\newcommand{\RaTwoTwoSixHalfLife}{\SI{1600}{\year}}
\newcommand{\ThTwoTwoEightHalfLife}{\SI{1.9}{\year}}
\newcommand{\ThTwoThreeTwoHalfLife}{\SI{1.4E10}{\year}}
\newcommand{\UTwoThreeFiveHalfLife}{\SI{4.47E9}{\year}}
\newcommand{\UTwoThreeEightHalfLife}{\SI{4.47E9}{\year}}
\newcommand{\UTwoThreeEightNaturalAbundance}{\SI{99.27}{\percent}}
\newcommand{\UTwoThreeEightSFAvgNeutronMult}{\num{2.01}}
\newcommand{\AmTwoFourGammaOneEnergy}{\SI{59.5}{\keV}}
\newcommand{\AmTwoFourOneGammaTwoBR}{\SI{56}{\percent}}
\newcommand{\AmBeGammaEnergy}{\SI{4.4}{\MeV}}
\newcommand{\AmBe}{\ce{^241AmBe}}
\newcommand{\AmC}{\ce{^241Am^13C}}
\newcommand{\AmLi}{\ce{^241AmLi}}
\newcommand{\AmCNeutronEnergy}{\SI{4}{\MeV}}
\newcommand{\DD}{\ce{^2D}-\ce{^2D}}
\newcommand{\DDNeutronEnergy}{\SI{2.45}{\MeV}}
\newcommand{\AArArThreeNineOverArFourZeroRatio}{\num{8E-16}}
\newcommand{\AArArThreeNineActivity}{\SI{1}{\becquerel\per\kg}}
\newcommand{\NeutronsPerChainDecayUTh}{\numrange{E-5}{E-7}}
\newcommand{\LArRadiogenicNeutronInteractionLength}{\SI{~10}{\cm}}
\newcommand{\alphan}{($\alpha$,$n$)}
%--- Cosmology
\newcommand{\LCDM}{\mbox{$\Lambda$CDM}}
%--- General Names
\newcommand{\DE}{\mbox{DE}}
\newcommand{\DM}{\mbox{DM}}
\newcommand{\IH}{\mbox{IH}}
\newcommand{\NH}{\mbox{NH}}
\newcommand{\SM}{\mbox{SM}}
\newcommand{\BSM}{\mbox{BSM}}
\newcommand{\STP}{\mbox{STP}}
\newcommand{\PDF}{\mbox{PDF}}
%--- Double Beta
\newcommand{\bb}{\mbox{$\beta\beta$}}
\newcommand{\tnbb}{\mbox{$2\nu\beta\beta$}}
\newcommand{\znbb}{\mbox{$0\nu\beta\beta$}}
\newcommand{\mnu}{\mbox{$m_{\nu}$}}
\newcommand{\mbb}{\mbox{$m_{\beta\beta}$}}
\newcommand{\Qbb}{\mbox{$Q_{\beta\beta}$}}
\newcommand{\tozn}{\mbox{$T^{0\nu}_{1/2}$}}
\newcommand{\totn}{\mbox{T$^{2\nu}_{1/2}$}}
\newcommand{\aSe}{\mbox{a-\ce{Se}}}
\newcommand{\eSiPM}{\mbox{eSiPM}}
\newcommand{\eSiPMs}{\mbox{eSiPMs}}
\newcommand{\tSiPM}{\mbox{tSiPM}}
\newcommand{\tSiPMs}{\mbox{tSiPMs}}
%--- Solar Neutrinos
\newcommand{\PP}{\mbox{$pp$}}
\newcommand{\PEP}{\mbox{$pep$}}
\newcommand{\CNO}{\mbox{CNO}}
\newcommand{\HEP}{\mbox{$hep$}}
\newcommand{\CEnNS}{\mbox{CE$\nu$NS}}
%--- Names
\newcommand{\DS}{\mbox{DarkSide}}
\newcommand{\DSt}{\mbox{DarkSide-10}}
\newcommand{\DSf}{\mbox{DarkSide-50}}
\newcommand{\DSp}{\mbox{DarkSide-Proto}}
\newcommand{\DSz}{\mbox{DarkSide-ProtoZero}}
\newcommand{\DSk}{\mbox{DarkSide-20k}}
\newcommand{\DSh}{\mbox{DarkSide-HighMass}}
\newcommand{\DSl}{\mbox{DarkSide-LowMass}}
\newcommand{\DSn}{\mbox{DarkNoon}}
\newcommand{\Argo}{\mbox{Argo}}
\newcommand{\DSs}{\mbox{DS}}
\newcommand{\DSts}{\mbox{DS-10}}
\newcommand{\DSfs}{\mbox{DS-50}}
\newcommand{\DSps}{\mbox{DS-Proto}}
\newcommand{\DSzs}{\mbox{DS-ProtoZero}}
\newcommand{\DSks}{\mbox{DS-20k}}
\newcommand{\DShs}{\mbox{DS-HM}}
\newcommand{\DSls}{\mbox{DS-LM}}
\newcommand{\DSns}{\mbox{DNoon}}
\newcommand{\JuTernesecche}{\ce{Ar}:\ce{CH_4}(:\ce{Xe})}
\newcommand{\JTS}{\JuTernesecche}
\newcommand{\JT}{\ce{Ar}:\ce{CH_4}}
\newcommand{\JS}{\ce{Ar}:\ce{Xe}}
\newcommand{\IAB}{\mbox{IAB}}
\newcommand{\OAB}{\mbox{OAB}}
\newcommand{\GdAS}{\mbox{\ce{Gd}AS}}
\newcommand{\DSCollaborators}{\num{\sim~350}}
\newcommand{\DSInstitutes}{\num{\sim~70}}
\newcommand{\DSCountries}{\num{15}}
\newcommand{\DSCERNCurrentUsers}{\num{\sim~50}}
\newcommand{\DSCERNFutureUsers}{\num{\sim~100}}
\newcommand{\WArP}{\mbox{WArP}}
\newcommand{\GADMC}{\mbox{GADMC}}
\newcommand{\DEAPOne}{\mbox{DEAP-1}}
\newcommand{\DEAP}{\mbox{DEAP-3600}}
\newcommand{\mCLEAN}{\mbox{MiniCLEAN}}
\newcommand{\ArDM}{\mbox{ArDM}}
\newcommand{\DArT}{\mbox{DArT}}
\newcommand{\EXO}{\mbox{EXO-200}}
\newcommand{\ThreeDPi}{\mbox{3D$\pi$}}
\newcommand{\DMNDS}{\mbox{DIAMONDS}}
\newcommand{\FBP}{\mbox{FBP}}
\newcommand{\BX}{\mbox{Borexino}}
\newcommand{\SNO}{\mbox{SNO}}
\newcommand{\SCENE}{\mbox{SCENE}}
\newcommand{\ReD}{\mbox{ReD}}
\newcommand{\ARIS}{\mbox{ARIS}}
\newcommand{\Urania}{\mbox{Urania}}
\newcommand{\Aria}{\mbox{Aria}}
\newcommand{\Seruci}{\mbox{Seruci}}
\newcommand{\SeruciZero}{\mbox{Seruci-0}}
\newcommand{\SeruciOne}{\mbox{Seruci-I}}
\newcommand{\SeruciTwo}{\mbox{Seruci-II}}
\newcommand{\LOGAN}{\mbox{LOGAN}}
\newcommand{\MAWG}{M\&A\,WG}
\newcommand{\CTF}{\mbox{CTF}}
\newcommand{\WBS}{\mbox{WBS}}
\newcommand{\CROne}{\mbox{CR1}}
\newcommand{\CRH}{\mbox{CRH}}
\newcommand{\LSV}{\mbox{LSV}}
\newcommand{\WCV}{\mbox{WCV}}
\newcommand{\PSV}{\mbox{PSV}}
\newcommand{\LArSV}{\mbox{LArSV}}
\newcommand{\OC}{\mbox{OC}}
\newcommand{\MLI}{\mbox{MLI}}
\newcommand{\CV}{\mbox{CV}}
\newcommand{\WT}{\mbox{WT}}
\newcommand{\TPC}{\mbox{TPC}}
\newcommand{\TPCs}{\mbox{TPCs}}
\newcommand{\LArTPC}{\mbox{LAr~TPC}}
\newcommand{\LArTPCs}{\mbox{LAr~TPCs}}
\newcommand{\IV}{\mbox{Inner~Vessel}}
\newcommand{\CALIS}{\mbox{CALIS}}
\newcommand{\UV}{\mbox{UV}}
\newcommand{\NUV}{\mbox{NUV}}
\newcommand{\TMF}{\mbox{TMF}}
\newcommand{\PMT}{\mbox{PMT}}
\newcommand{\PMTs}{\mbox{\PMT s}}
\newcommand{\MCP}{\mbox{MCP}}
\newcommand{\MCPPMT}{\mbox{\MCP-\PMT}}
\newcommand{\MCPPMTs}{\mbox{\MCPPMT s}}
\newcommand{\SiPM}{\mbox{SiPM}}
\newcommand{\SiPMs}{\mbox{SiPMs}}
\newcommand{\RGBHd}{\mbox{RGB-HD}}
\newcommand{\RGBHdSf}{\mbox{RGB-HD-SF}}
\newcommand{\RGBHdSfHRq}{\mbox{RGB-HD-HR$_q$}}
\newcommand{\RGBHdSfLRq}{\mbox{RGB-HD-LR$_q$}}
\newcommand{\NUVHd}{\mbox{NUV-HD}}
\newcommand{\NUVHdSf}{\mbox{NUV-HD-SF}}
\newcommand{\NUVHdLf}{\mbox{NUV-HD-LF}}
\newcommand{\NUVHdLfTdd}{\mbox{NUV-HD-LF-3dd}}
\newcommand{\NUVHdSfHRq}{\mbox{NUV-HD-SF-HR$_q$}}
\newcommand{\NUVHdSfLRq}{\mbox{NUV-HD-SF-LR$_q$}}
\newcommand{\NUVHdLfHRq}{\mbox{NUV-HD-LF-HR$_q$}}
\newcommand{\NUVHdLfLRq}{\mbox{NUV-HD-LF-LR$_q$}}
\newcommand{\HRq}{\mbox{HR$_q$}}
\newcommand{\LRq}{\mbox{LR$_q$}}
\newcommand{\HD}{\mbox{HD}}
\newcommand{\CTE}{\mbox{CTE}}
\newcommand{\PCB}{\mbox{PCB}}
\newcommand{\PCBs}{\mbox{PCBs}}
\newcommand{\TSV}{\mbox{TSV}}
\newcommand{\TSVs}{\mbox{TSVs}}
\newcommand{\tile}{\mbox{tile}}
\newcommand{\tiles}{\mbox{tiles}}
\newcommand{\SPAD}{\mbox{SPAD}}
\newcommand{\SPADs}{\mbox{SPADs}}
\newcommand{\QE}{\mbox{QE}}
\newcommand{\PDE}{\mbox{PDE}}
\newcommand{\OV}{\mbox{OV}}
\newcommand{\LV}{\mbox{LV}}
\newcommand{\SCR}{\mbox{SCR}}
\newcommand{\DCR}{\mbox{DCR}}
\newcommand{\DiCT}{\mbox{DiCT}}
\newcommand{\DeCT}{\mbox{DeCT}}
\newcommand{\AP}{\mbox{AP}}
\newcommand{\DLED}{\mbox{DLED}}
\newcommand{\TCNR}{\mbox{TCNR}}
\newcommand{\TCNP}{\mbox{TCNP}}
\newcommand{\CMOS}{\mbox{CMOS}}
\newcommand{\HLST}{\mbox{HLST}}
\newcommand{\SQB}{\mbox{SQB}}
\newcommand{\SQBs}{\mbox{\SQB s}}
\newcommand{\TRB}{\mbox{TRB}}
\newcommand{\TRBs}{\mbox{\TRB s}}
\newcommand{\WIMP}{\mbox{WIMP}}
\newcommand{\WIMPs}{\mbox{\WIMP s}}
\newcommand{\MC}{\mbox{MC}}
\newcommand{\DAQ}{\mbox{DAQ}}
\newcommand{\ADC}{\mbox{ADC}}
\newcommand{\ADCs}{\mbox{\ADC s}}
\newcommand{\DAC}{\mbox{DAC}}
\newcommand{\DACs}{\mbox{\DAC s}}
\newcommand{\TDC}{\mbox{TDC}}
\newcommand{\TDCs}{\mbox{\TDC s}}
\newcommand{\FPGA}{\mbox{FPGA}}
\newcommand{\FIFO}{\mbox{FIFO}}
\newcommand{\FIFOs}{\mbox{\FIFO s}}
\newcommand{\IO}{\mbox{I/O}}
\newcommand{\artdaq}{\mbox{artdaq}}
\newcommand{\TMB}{\mbox{TMB}}
\newcommand{\PC}{\mbox{PC}}
\newcommand{\PCTMB}{\mbox{\PC-\TMB}}
\newcommand{\PPO}{\mbox{PPO}}
\newcommand{\BisMSB}{\mbox{BisMSB}}
\newcommand{\POPOP}{\mbox{POPOP}}
\newcommand{\DIN}{\mbox{DIN}}
\newcommand{\LAB}{\mbox{LAB}}
\newcommand{\PXE}{\mbox{PXE}}
\newcommand{\ITO}{\mbox{ITO}}
\newcommand{\PTFE}{\mbox{PTFE}}
\newcommand{\FEP}{\mbox{FEP}}
\newcommand{\PMMA}{\mbox{PMMA}}
\newcommand{\ESR}{\mbox{ESR}}
\newcommand{\PUR}{\mbox{PUR}}
\newcommand{\TPB}{\mbox{TPB}}
\newcommand{\og}{\mbox{Operations Group}}
\newcommand{\VUV}{\mbox{VUV}}
\newcommand{\LAr}{\ce{LAr}}
\newcommand{\GAr}{\ce{GAr}}
\newcommand{\AAr}{\ce{AAr}}
\newcommand{\UAr}{\ce{UAr}}
\newcommand{\DAr}{\ce{DAr}}
\newcommand{\LRAr}{\ce{LRAr}}
\newcommand{\LIN}{\ce{LN2}}
\newcommand{\LXe}{\ce{LXe}}
\newcommand{\LNe}{\ce{LNe}}
\newcommand{\LHe}{\ce{LHe}}
\newcommand{\HPGe}{\mbox{HPGe}}
\newcommand{\NAA}{\mbox{NAA}}
\newcommand{\HVFT}{\mbox{HVFT}}
\newcommand{\UHMWPE}{\mbox{UHMWPE}}
\newcommand{\TOF}{\mbox{TOF}}
\newcommand{\PET}{\mbox{PET}}
\newcommand{\TOFPET}{\mbox{\TOF-\PET}}
\newcommand{\PETCT}{\mbox{\PET /CT}}
\newcommand{\FDG}{\mbox{\ce{^18F}-FDG}}
\newcommand{\LOR}{\mbox{LOR}}
\newcommand{\CT}{\mbox{CT}}
\newcommand{\CPU}{\mbox{CPU}}
\newcommand{\CPUs}{\mbox{CPUs}}
\newcommand{\STEM}{\mbox{STEM}}
\newcommand{\ROI}{\mbox{ROI}}
\newcommand{\SPE}{\mbox{SPE}}
\newcommand{\SNR}{\mbox{SNR}}
\newcommand{\SNRAmp}{\mbox{SNR$_{\rm Amplitude}$}}
\newcommand{\SNRCharge}{\mbox{SNR$_{\rm Charge}$}}
\newcommand{\SNRFast}{\mbox{SNR$_{\rm Fast}$}}
\newcommand{\SNRFilter}{\mbox{SNR$_{\rm Filtered}$}}
\newcommand{\OA}{\mbox{OA}}
\newcommand{\GBP}{\mbox{GBP}}
\newcommand{\TIA}{\mbox{TIA}}
\newcommand{\TIAs}{\mbox{\TIA s}}
\newcommand{\FEB}{\mbox{FEB}}
\newcommand{\FEBs}{\mbox{\FEB s}}
\newcommand{\VFEB}{\mbox{VFEB}}
\newcommand{\VFEBs}{\mbox{\VFEB s}}
\newcommand{\VDCB}{\mbox{VDCB}}
\newcommand{\VDCBs}{\mbox{\VDCB s}}
\newcommand{\AVol}{\mbox{$A_{\tiny\rm Vol}$}}
\newcommand{\NoG}{\mbox{NG}}
\newcommand{\NoGTrue}{\mbox{$\NoG_{\rm True}$}}
\newcommand{\Tz}{\mbox{$T_z$}}
\newcommand{\eno}{\mbox{$e_n$}}
\newcommand{\enot}{\mbox{$e_n^2$}}
\newcommand{\ino}{\mbox{$i_n$}}
\newcommand{\inot}{\mbox{$i_n^2$}}
\newcommand{\Vno}{\mbox{$V_n$}}
\newcommand{\Vnot}{\mbox{$V_n^2$}}
\newcommand{\VnoTot}{\mbox{$V_n^{\rm Tot}$}}
\newcommand{\fRes}{\mbox{$f_{\rm Res}$}}
\newcommand{\FTDb}{\mbox{$f_{\rm 3Db}$}}
\newcommand{\FSDb}{\mbox{$f_{\rm 6Db}$}}
\newcommand{\TDb}{\SI{3}{\decibel}}
\newcommand{\SDb}{\SI{6}{\decibel}}
\newcommand{\PSDno}{\mbox{$\rm PSD_{n}$}}
\newcommand{\PSDnoReferencePower}{\SI{1}{\milli\watt}}
\newcommand{\NSF}{\mbox{NSF}}
\newcommand{\RAS}{\mbox{RAS}}
\newcommand{\GSSI}{\mbox{GSSI}}
\newcommand{\INFN}{\mbox{INFN}}
\newcommand{\MIUR}{\mbox{MIUR}}
\newcommand{\CERN}{\mbox{CERN}}
\newcommand{\INDPT}{\mbox{IN2P3}}
\newcommand{\DOE}{\mbox{DOE}}
\newcommand{\BNL}{\mbox{BNL}}
\newcommand{\FNAL}{\mbox{FNAL}}
\newcommand{\Fermilab}{\mbox{Fermilab}}
\newcommand{\PNNL}{\mbox{PNNL}}
\newcommand{\IHEP}{\mbox{CAS-IHEP}}
\newcommand{\EOk}{\mbox{E-1000}}
\newcommand{\RETS}{\mbox{RE-37}}
\newcommand{\LHC}{\mbox{LHC}}
\newcommand{\HLLHC}{\mbox{HL-LHC}}
\newcommand{\ATLAS}{\mbox{ATLAS}}
\newcommand{\CMS}{\mbox{CMS}}
\newcommand{\BTL}{\mbox{BTL}}
\newcommand{\CFI}{\mbox{CFI}}
\newcommand{\NSERC}{\mbox{NSERC}}
\newcommand{\LNGS}{\mbox{LNGS}}
\newcommand{\LSC}{\mbox{LSC}}
\newcommand{\SNOLAB}{\mbox{SNOLAB}}
\newcommand{\TRIUMF}{\mbox{TRIUMF}}
\newcommand{\LNF}{\mbox{LNF}}
\newcommand{\LNS}{\mbox{LNS}}
\newcommand{\DUNE}{\mbox{DUNE}}
\newcommand{\pDUNE}{\mbox{ProtoDUNE}}
\newcommand{\nEXO}{\mbox{nEXO}}
\newcommand{\NEXT}{\mbox{NEXT}}
\newcommand{\XENON}{\mbox{XENON}}
\newcommand{\LZ}{\mbox{LZ}}
\newcommand{\DAMA}{\mbox{DAMA}}
\newcommand{\JUNO}{\mbox{JUNO}}
\newcommand{\CNAF}{\mbox{CNAF}}
\newcommand{\PoliMi}{\mbox{PoliMi}}
\newcommand{\FBKTIFPA}{\mbox{FBK/TIFPA}}
\newcommand{\FBK}{\mbox{FBK}}
\newcommand{\LFoundry}{\mbox{LFoundry}}
\newcommand{\CAEN}{\mbox{CAEN}}
\newcommand{\MPD}{\mbox{MPD}}
\newcommand{\HPK}{\mbox{Hamamatsu Photonics}}
\newcommand{\SensL}{\mbox{SensL}}
\newcommand{\NOA}{\mbox{NOA}}
\newcommand{\LSO}{\mbox{LSO}}
\newcommand{\LYSO}{\mbox{LYSO}}
\newcommand{\LYSOCe}{\mbox{LYSO:Ce}}
\newcommand{\CRT}{\mbox{CRT}}
\newcommand{\IC}{\mbox{IC}}
\newcommand{\ICs}{\mbox{ICs}}
\newcommand{\ASIC}{\mbox{ASIC}}
\newcommand{\ASICs}{\mbox{\ASIC s}}
\newcommand{\CAASIC}{\mbox{CA\ASIC}}
\newcommand{\CAASICs}{\mbox{\CAASIC s}}
\newcommand{\FTASIC}{\mbox{FT\ASIC}}
\newcommand{\FTASICs}{\mbox{\FTASIC s}}
\newcommand{\LED}{\mbox{LED}}
\newcommand{\LEDs}{\mbox{LEDs}}
\newcommand{\PSA}{\mbox{PSA}}
\newcommand{\UHV}{UHV}
\newcommand{\HalfLife}{\mbox{$\tau_{\frac{1}{2}}$}}
\newcommand{\ICPMS}{\mbox{ICP-MS}}
\newcommand{\LA}{\mbox{LA}}
\newcommand{\LAICPMS}{\mbox{\LA-\ICPMS}}
\newcommand{\GDMS}{\mbox{GDMS}}
\newcommand{\BiPo}{\mbox{BiPo-3}}
\newcommand{\PEB}{\mbox{PEB}}
\newcommand{\PEBs}{\mbox{PEBs}}
\newcommand{\MIDAS}{\mbox{MIDAS}}
\newcommand{\VO}{\mbox{VO}}
\newcommand{\LiDaR}{\mbox{LiDaR}}
\newcommand{\ArlonFiveFiveNT}{\mbox{Arlon~55-NT}}
\newcommand{\ArlonEightFiveN}{\mbox{Arlon~85-N}}
\newcommand{\ArlonEightFiveNT}{\mbox{Arlon~85-NT}}
\newcommand{\THERMOUNT}{\mbox{THERMOUNT\textregistered RT\textsuperscript{TM}}}
\newcommand{\Vikuiti}{\mbox{3M Vikuiti\textsuperscript{TM}}}
\newcommand{\PEDOT}{\mbox{PEDOT:PSS}}
\newcommand{\Clevios}{\mbox{Clevios\textsuperscript{TM}}}
%--- Global Symbols
\newcommand{\OmegaNonBaryonicFraction}{\num{0.85}}
\newcommand{\OmegaNonBaryonicPercent}{\SI{85}{\percent}}
\newcommand{\RhoDMSymbol}{\mbox{$\rho_{\rm dm}$}}
\newcommand{\RhoDMValue}{\SI{0.3}{\GeV\per\square\c\per\cubic\cm}}
\newcommand{\VelocityNaughtSymbol}{\mbox{$v_0$}}
\newcommand{\VelocityNaughtValue}{\SI{220}{\km\per\s}}
\newcommand{\VelocityEarthSymbol}{\mbox{$v_{\rm Earth}$}}
\newcommand{\VelocityEarthValue}{\SI{232}{\km\per\s}}
\newcommand{\VelocityEscapeSymbol}{\mbox{$v_{\rm escape}$}}
\newcommand{\VelocityEscapeValue}{\SI{544}{\km\per\s}}
\newcommand{\WIMPMassSymbol}{\mbox{m_\chi}}
\newcommand{\WIMPMassLowLimit}{\SI{50}{\GeV\per\square\c}}
\newcommand{\WIMPMassHundredGev}{\SI{100}{\GeV\per\square\c}}
\newcommand{\WIMPMassOneTev}{\SI{1}{\TeV\per\square\c}}
\newcommand{\WIMPMassTenTev}{\SI{10}{\TeV\per\square\c}}
\newcommand{\LArNormalTemperature}{\SI{87}{\kelvin}}
\newcommand{\LINNormalTemperature}{\SI{77}{\kelvin}}
\newcommand{\LXeNormalTemperature}{\SI{165}{\kelvin}}
\newcommand{\RoomTemperature}{\SI{300}{\kelvin}}
\newcommand{\ElectronMass}{\SI{511}{\keV\per\square\c}}
\newcommand{\LHCCenterOfMassEnergy}{\SI{13}{TeV}}
\newcommand{\LHCDirectSearchesWIMPMassTurnoverThreshold}{\text{a few hundred~\si{GeV\per\square\c}}}
\newcommand{\BackgroundFreeRequirement}{\SI{<0.1}{\ev}}
\newcommand{\ZeroBackgroundNinetyPerCentCLEventsLimit}{\SI{2.3}{\ev}}
\newcommand{\NinetyPerCentCL}{\mbox{\SI{90}{\percent}~C.L.}}
\newcommand{\ArScintillationYield}{\SI{4E4}{\ph\per\MeV}}
\newcommand{\TPBWaveLength}{\SI{420}{\nano\meter}}
\newcommand{\ArWaveLength}{\SI{128}{\nano\meter}}
\newcommand{\XeWaveLength}{\SI{172}{\nano\meter}}
\newcommand{\NR}{\mbox{NR}}
\newcommand{\NRs}{\mbox{NRs}}
\newcommand{\ER}{\mbox{ER}}
\newcommand{\ERs}{\mbox{ERs}}
\newcommand{\bg}{\mbox{$\beta/\gamma$}}
\newcommand{\bgs}{\mbox{$\beta/\gamma$'s}}
\newcommand{\ar}{\mbox{$\alpha$-ray}}
\newcommand{\ars}{\mbox{$\alpha$-rays}}
\newcommand{\br}{\mbox{$\beta$-ray}}
\newcommand{\brs}{\mbox{$\beta$-rays}}
\newcommand{\gr}{\mbox{$\gamma$-ray}}
\newcommand{\grs}{\mbox{$\gamma$-rays}}
\newcommand{\grsnh}{\mbox{$\gamma$~rays}}														% nh = no hyphen
\newcommand{\xr}{\mbox{X-ray}}
\newcommand{\xrs}{\mbox{X-rays}}
\newcommand{\bta}{\mbox{$\beta$}}
\newcommand{\btas}{\mbox{$\beta$'s}}
\newcommand{\LEff}{\mbox{$\mathcal{L}_{\rm eff}$}}
\newcommand{\SOne}{\mbox{S1}}
\newcommand{\STwo}{\mbox{S2}}
\newcommand{\STwoSoneRatio}{\mbox{S2/S1}}
\newcommand{\SThree}{\mbox{S3}}
\newcommand{\gTwo}{\mbox{$g_2$}}
\newcommand{\Qy}{\mbox{$Q_y$}}
\newcommand{\Ne}{\mbox{$N_{e^-}$}}
\newcommand{\GWL}{\mbox{GWL}}
\newcommand{\LWL}{\mbox{LWL}}
\newcommand{\CDR}{\mbox{CDR}}
\newcommand{\TDR}{\mbox{TDR}}
\newcommand{\tz}{\mbox{$t_0$}}
\newcommand{\roo}{\mbox{$\rm \rho_o$}}
%--- Local Symbols
\newcommand{\ArDimerSingletMeanLife}{\SI{6}{\nano\second}}
\newcommand{\ArDimerTripletMeanLife}{$\sim$\SI{1.5}{\us}}
\newcommand{\XeDimerSingletMeanLife}{\SI{2}{\nano\second}}
\newcommand{\XeDimerTripletMeanLife}{\SI{22}{\nano\second}}
\newcommand{\PSD}{\mbox{PSD}}
\newcommand{\FPrompt}{\mbox{$f_{\rm prompt}$}}
\newcommand{\FNine}{\mbox{$f_{90}$}}
\newcommand{\FOneFive}{\mbox{$f_{150}$}}
\newcommand{\FOneTwo}{\mbox{$f_{120}$}}
\newcommand{\FTwoZero}{\mbox{$f_{200}$}}
\newcommand{\SigmaFNine}{\mbox{$\sigma_{\FNine}$}}
\newcommand{\SigmaFOneFive}{\mbox{$\sigma_{\FOneFive}$}}
\newcommand{\SigmaFTwoZero}{\mbox{$\sigma_{\FTwoZero}$}}
\newcommand{\WindowFNine}{\SI{90}{\nano\second}}
\newcommand{\WindowFOneTwo}{\SI{120}{\nano\second}}
\newcommand{\WindowFOneFive}{\SI{150}{\nano\second}}
\newcommand{\WindowFTwoZero}{\SI{200}{\nano\second}}
\newcommand{\WindowSOne}{\SI{7}{\us}}
\newcommand{\FractionSOneERWindowFNine}{\SI{30}{\percent}}
\newcommand{\VThreshold}{\mbox{$V_{\rm Threshold}$}}
\newcommand{\SigmaBaseline}{\mbox{$\sigma_{\rm Baseline}$}}
\newcommand{\SigmaSPE}{\mbox{$\sigma_{\rm SPE}$}}
\newcommand{\SigmaSPEt}{\mbox{$\sigma_{\rm SPE}^2$}}
\newcommand{\SigmaTPB}{\mbox{$\sigma_{\rm TPB}$}}
\newcommand{\SigmaP}{\mbox{$\sigma_{\rm p}$}}
\newcommand{\SigmaL}{\mbox{$\sigma_{\rm l}$}}
\newcommand{\GPSAbsoluteTimeAccuracy}{\SI{20}{\nano\second}}
\newcommand{\LNGSMuonResidualFlux}{\SI{1.2}{\per\square\m\per\hour}}
\newcommand{\SNOLABMuonResidualFlux}{\SI{1.2E-2}{\per\square\m\per\hour}}
\newcommand{\LNGSDepthMWE}{\SI{3800}{\mwe}}						%BX, JCAP 08, 049 (2013)
\newcommand{\SNOLABDepthMWE}{\SI{6000}{\mwe}}
\newcommand{\LArNoBubblingHeatDissipation}{\SI{20}{\milli\watt\per\square\cm\per\mlardepth}}
%--- Buffer detectors
\newcommand{\ABSingleThreshold}{\SI{800}{\keV}}
\newcommand{\ABCoincidenceThreshold}{\SI{100}{\keV}}
\newcommand{\ABPhotocathodicCoverage}{\SI{4}{\square\meter}}
\newcommand{\IABPhotocathodicCoverage}{\SI{2}{\square\meter}}
\newcommand{\OABPhotocathodicCoverage}{\SI{2}{\square\meter}}

%--- Supernova Neutrinos in DS-20k
\newcommand{\DSkSupernovaBaseline}{\SI{10}{\kilo\parsec}}
\newcommand{\DSkSupernovaVetoEvents}{\num{E2}}
\newcommand{\DSkSupernovaVetoWindow}{\SI{10}{\ms}}
%--- Radon
\newcommand{\RadonMonitorLimit}{\mbox{some tens of~\si{\micro\becquerel}}}
\newcommand{\RadonFilterLimit}{\SI{1}{\milli\becquerel}}
\newcommand{\RadonFilterSuppression}{\num{1E5}}
\newcommand{\RadonCRHLimit}{\SI{5}{\milli\becquerel\per\cubic\meter}}
\newcommand{\RadonCRHSuppression}{\num{2E4}}
\newcommand{\RadonPrincetonCRLimit}{\SI{<1}{\becquerel\per\cubic\meter}}
\newcommand{\RadonPrincetonCRSuppression}{\num{E2}}
\newcommand{\RadonAirRate}{\SI{220}{\cubic\meter\per\hour}}
\newcommand{\RadonAirRadonActivity}{\SI{20}{\milli\becquerel\per\cubic\meter}}
\newcommand{\RadonDetectorSensitivty}{\SI{100}{\micro\becquerel\per\cubic\meter}}
%--- Facilities
\newcommand{\LNGSWaterTemp}{\SI{\sim~8}{\degreeC}}
\newcommand{\LNGSWaterPressure}{\SIrange{6}{8}{\bar}}
\newcommand{\LNGSWaterFlowRate}{\SI{1}{\cubic\meter\per\hour}}
\newcommand{\LNGSAirCompressorPressure}{\SI{8}{\bar}}
\newcommand{\LNGSHallCLength}{\SI{100}{\meter}}
\newcommand{\LNGSHallCWidthHeight}{\SI{20}{\meter}}
\newcommand{\LNGSHallCDoubleHookCraneLoadBare}{20}
\newcommand{\LNGSHallCDoubleHookCraneLoad}{\SI{\LNGSHallCDoubleHookCraneLoadBare}{\tonne}}
\newcommand{\LNGSHallCSmallCraneLoad}{\SI{5}{\tonne}}
\newcommand{\LNGSHallCLargeCraneLoad}{\SI{25}{\tonne}}
\newcommand{\LNGSHallCLiquidCollectionRate}{\SI{\sim~1000}{\cubic\meter\per\hour}}
\newcommand{\LNGSHallCFreshAirRate}{\SI{\sim~7000}{\cubic\meter\per\hour}}
\newcommand{\LNGSHallCScintillatorStorageNumTanks}{\num{4}}
\newcommand{\LNGSHallCScintillatorStorageTanksSize}{\SI{100}{\cubic\meter}}
\newcommand{\LNGSHallCPureWaterProductionRate}{\SI{1}{\cubic\meter\per\hour}}
\newcommand{\LNGSHallCPCRecoveryTankSize}{\SI{\sim~8}{\cubic\meter}}
%--- SiPMs FBK Cold Tests
\newcommand{\FBKColdSetupTemperatureRange}{\SIrange{233}{300}{\kelvin}}
\newcommand{\FBKColdSetupTemperatureColdLimit}{\SI{233}{\kelvin}}
%--- LNGS Cryogenic Tests
\newcommand{\LNGSCryoSetupTemperatureRange}{\SIrange{40}{300}{\kelvin}}
\newcommand{\LNGSCryoSetupTemperatureColdLimit}{\SI{40}{\kelvin}}
\newcommand{\LNGSCryoSetupTemperatureStability}{\SI{0.1}{\kelvin}}
\newcommand{\LNGSCryoSetupTemperatureAccuracy}{\SI{3}{\kelvin}}
\newcommand{\LNGSCryoSetupTemperatureControllerModule}{Lakeshore~335}
\newcommand{\LNGSCryoSetupTemperatureMonitorModule}{Lakeshore~218}
\newcommand{\LNGSCryoSetupCooldownTime}{\SI{40}{\min}}
\newcommand{\LNGSCryoSetupCryostatHeight}{\SI{500}{\mm}}
\newcommand{\LNGSCryoSetupCryostatFlangeModel}{DN~320~ISO-K}
\newcommand{\LNGSCryoSetupOperatingPressure}{\SI{E-2}{\milli\bar}}
\newcommand{\LNGSCryoSetupEvacuationPumpModel}{Pfeiffer~ACP15}
\newcommand{\LNGSCryoSetupCryocoolerModel}{Cryomech~PT90}
\newcommand{\LNGSCryoSetupCryocoolerLINPower}{\SI{90}{\W}}
\newcommand{\LNGSCryoSetupConductiveEpoxyModel}{MasterBond~EP21TDCS-LO}
\newcommand{\LNGSCryoSetupIMSPCBThickness}{\SI{1.6}{\mm}}
\newcommand{\LNGSCryoSetupSiPMBiasModel}{Keithley~2450~SourceMeter}
\newcommand{\LNGSCryoSetupOscilloscopeModel}{LeCroy~204MXi-A}
\newcommand{\LNGSCryoSetupOscilloscopeSamplingRate}{\SI{10}{\giga\sample\per\second}}
\newcommand{\LNGSCryoSetupLaserModel}{Edinburgh~Instruments~EPL-405}
\newcommand{\LNGSCryoSetupSiPMBiasCurrentResolution}{\SI{1}{\nano\ampere}}
\newcommand{\LNGSCryoSetupAmplifierBiasModel}{Elind~32DP8}
\newcommand{\LNGSCryoSetupAmplifierBiasRMSNoise}{Elind~32DP8}
\newcommand{\LNGSCryoSetupDigitizerModel}{CAEN~V1751}
\newcommand{\LNGSCryoSetupDigitizerSamplingRate}{\SI{1}{\giga\Sample\per\second}}
\newcommand{\LNGSCryoSetupDigitizerResolution}{\SI{10}{\bit}}
\newcommand{\LNGSCryoSetupDigitizerIntegrationGate}{\SI{500}{\nano\second}}
\newcommand{\LNGSCryoSetupTimeIndicatorFineResolution}{\SI{8}{\nano\second}}
\newcommand{\LNGSCryoSetupTimeIndicatorFineOverflow}{\SI{37}{\second}}
\newcommand{\LNGSCryoSetupTimeIndicatorCoarsePrecision}{\SI{10}{\milli\second}}
\newcommand{\LNGSCryoSetupGateShortWidth}{\SI{10}{\micro\second}}
\newcommand{\LNGSCryoSetupGateLongWidth}{\SI{2}{\milli\second}}
\newcommand{\LNGSCryoNUVHDSPADSize}{\SI[product-units=power]{25 x 25}{\square\micro\meter}}
\newcommand{\LNGSCryoRGBHDHRSPADSize}{\SI[product-units=power]{25 x 25}{\square\micro\meter}}
\newcommand{\LNGSCryoRGBHDLRSPADSize}{\SI[product-units=power]{20 x 20}{\square\micro\meter}}
%--- Naples Cryogenic Tests
\newcommand{\NaplesCryoCleanRoomSurface}{\SI{70}{\square\meter}}
\newcommand{\NaplesCryoUltrasonicBathVolume}{\SI{50}{\liter}}
\newcommand{\NaplesCryoDryStationCoolingPower}{\SI{60}{\watt}}
\newcommand{\NaplesCryoDryStationCryostatHeight}{\SI{50}{\cm}}
\newcommand{\NaplesCryoDryStationCryostatDiameter}{\SI{40}{\cm}}
\newcommand{\NaplesCryoDryStationCryostatVacuum}{\SI{E-9}{\bara}}
\newcommand{\NaplesCryoDryStationPlateDiameter}{\SI{36}{\cm}}
\newcommand{\NaplesCryoDryStationPlatesHosted}{\num{4}}
\newcommand{\NaplesCryoDryStationSQBPerPlate}{\num{1}}
\newcommand{\NaplesCryoDryStationSQBHosted}{\num{4}}
\newcommand{\NaplesCryoDryStationPdmHosted}{\num{100}}
\newcommand{\NaplesCryoWetStationCoolingPower}{\SI{60}{\watt}}
\newcommand{\NaplesCryoWetStationCryostatHeight}{\SI{120}{\cm}}
\newcommand{\NaplesCryoWetStationCryostatDiameter}{\SI{60}{\cm}}
\newcommand{\NaplesCryoWetStationPlateDiameter}{\SI{55}{\cm}}
\newcommand{\NaplesCryoWetStationCryostatVacuum}{\SI{E-9}{\bara}}
\newcommand{\NaplesCryoWetStationPlatesHosted}{\num{2}}
\newcommand{\NaplesCryoWetStationSQBPerPlate}{\num{2}}
\newcommand{\NaplesCryoWetStationSQBHosted}{\num{4}}
\newcommand{\NaplesCryoWetStationPdmHosted}{\num{100}}
\newcommand{\NaplesCryoFractionPDEMeasurementInPdm}{\SI{1}{\percent}}
%--- PMT-SiPM Comparison
\newcommand{\HamamatsuModel}{Hamamatsu~S11828-3344M}
\newcommand{\HamamatsuSiPMsNumber}{\num{16}}
\newcommand{\HamamatsuSiPMTotalArea}{\SI[product-units=power]{3.0 x 3.0}{\square\mm}}
\newcommand{\HamamatsuArrayArea}{\SI[product-units=power]{12.0 x 12.0}{\square\mm}}
\newcommand{\HamamatsuSiPMLightYield}{\SI{1.1}{\pe\per\keVee}}
\newcommand{\HamamatsuPMTLightYield}{\SI{2.1}{\pe\per\keVee}}
\newcommand{\HamamatsuPMTAperture}{\SI[product-units=power]{20.0 x 20.0}{\square\mm}}
\newcommand{\HamamatsuSiPMLightPerAreaYield}{\SI{0.76}{\pe\per\keVee\per\square\cm}}
\newcommand{\HamamatsuPMTLightPerAreaYield}{\SI{0.53}{\pe\per\keVee\per\square\cm}}
\newcommand{\HamamatsuSiPMOverPMTLightYieldGain}{\SI{45}{\percent}}
\newcommand{\LNGSCellActiveDiameter}{\SI{80}{\mm}}
\newcommand{\LNGSCellActiveHeight}{\SI{80}{\mm}}
\newcommand{\LNGSCellPMTOpeningArea}{\SI[product-units=power]{20 x 20}{\square\mm}}
\newcommand{\SensLModel}{\mbox{SensL-ArrayC-60035-64P}}
\newcommand{\SensLSiPMsNumber}{\num{64}}
\newcommand{\SensLSiPMTotalArea}{\SI[product-units=power]{7.2 x 7.2}{\square\mm}}
\newcommand{\SensLSiPMActiveArea}{\SI[product-units=power]{6.0 x 6.0}{\square\mm}}
\newcommand{\SensLArrayArea}{\SI[product-units=power]{57.2 x 57.2}{\square\mm}}
\newcommand{\SensLSPADArea}{\SI[product-units=power]{35 x 35}{\square\micro\m}}
\newcommand{\SensLSPADCapacitance}{\SI{150}{\femto\farad}}
\newcommand{\SensLFillFactor}{\SI{75}{\percent}}
\newcommand{\SensLSPADCapacity}{\SI{150}{\femto\farad}}
\newcommand{\SensLBoardChannels}{\num{2}}
\newcommand{\SensLBoardSiPMPerChannel}{\num{32}}
\newcommand{\SensLLeaDCollimatorDiameter}{\SI{10}{\mm}}
\newcommand{\SensLLeadCollimatorLength}{\SI{30}{\mm}}
\newcommand{\SensLSiPMLightYield}{\SI{5.6}{\pe\per\keVee}}
\newcommand{\SensLPMTLightYield}{\SI{4.4}{\pe\per\keVee}}
\newcommand{\SensLTotalLightYield}{\SI{10}{\pe\per\keVee}}
\newcommand{\SensLSiPMOverPMTLightYieldGainOne}{\SI{43}{\percent}}
\newcommand{\SensLSiPMOverPMTLightYieldGainTwo}{\SI{25}{\percent}}
\newcommand{\SensLCorrelatedPulsesEffect}{\SI{25}{\percent}}
%--- GADMC
\newcommand{\GADMCFiducialMass}{\SI{300}{\tonne}}
\newcommand{\GADMCTotalMass}{\SI{500}{\tonne}}
\newcommand{\GADMCExtractionPeriod}{\SI{8}{\year}}
%--- DEAP-3600
\newcommand{\DEAPTotalMass}{\SI{3200}{\kg}}
\newcommand{\DEAPExposure}{\SI{2.1}{\tonne\year}}
\newcommand{\DEAPUArBackgroundFreeExtrapolatedExposure}{\SI{3000}{\tonne\yr}}
\newcommand{\DEAPInternalArea}{\SI{10}{\square\m}}
\newcommand{\DEAPPSDRejection}{\num{2.4E8}}
\newcommand{\DEAPDesignSensitivity}{\SI{2E-46}{\square\cm}}
\newcommand{\DEAPRadonLevel}{\SI{200}{\nano\becquerel\per\kg}}
%--- DarkNoon
\newcommand{\DSnRunTime}{\SI{20}{\year}}
\newcommand{\DSnExposure}{\SI{1000}{\tonne\year}}
\newcommand{\DSnSoupLXeMolarConcentration}{\SI{20}{\percent}}
\newcommand{\DSnSoupLXeMassConcentration}{\SI{45}{\percent}}
\newcommand{\DSnSoupLXeIsotopeMassConcentration}{\SI{41}{\percent}}
\newcommand{\DSnLXeEnrichment}{\SI{90}{\percent}}
\newcommand{\DSnFiducialLXeIsotopeMass}{\SI{50}{\tonne}}
\newcommand{\DSnFiducialLXeNonIsotopeMass}{\SI{5}{\tonne}}
\newcommand{\DSnFiducialUArIsotopeMass}{\mbox{t.b.d.}}
\newcommand{\DSnActiveLXeIsotopeMass}{\mbox{t.b.d.}}
\newcommand{\DSnActiveLXeNonIsotopeMass}{\mbox{t.b.d.}}
\newcommand{\DSnActiveUArIsotopeMass}{\mbox{t.b.d.}}
\newcommand{\DSnActiveVolumeHeigth}{\SI{670}{\cm}}
\newcommand{\DSnActiveVolumeOctagonSide}{\SI{175}{\cm}}
\newcommand{\DSnFiducialVolumeCut}{\SI{30}{\cm}}
\newcommand{\DSnPMMAVesselThickness}{\SI{25}{\cm}}
\newcommand{\DSnEnergyResolutionAtQbb}{\SI{0.7}{\percent}}
\newcommand{\DSfEnergyResolutionAtQbb}{\SI{1.5}{\percent}}
\newcommand{\EXOEnergyResolutionAtQbb}{\SI{1.6}{\percent}}
%--- DarkSide-20k
\newcommand{\DSkNuInducedBackgroundBare}{1.6}
\newcommand{\DSkNuInducedBackgroundUnit}{\SI{\DSkNuInducedBackgroundBare}{\ev}}
\newcommand{\DSkNuInducedBackgroundExtendedExposureBare}{3.2}
\newcommand{\DSkNuInducedBackgroundExtendedExposureUnit}{\SI{\DSkNuInducedBackgroundExtendedExposureBare}{\ev}}
\newcommand{\DSkTotalMass}{\SI{51.1}{\tonne}} 
\newcommand{\DSkActiveMass}{\SI{49.7}{\tonne}}
\newcommand{\DSkFiducialMass}{\SI{20.2}{\tonne}}
\newcommand{\DSkActiveDiameter}{\SI{355}{\cm}} 
\newcommand{\DSkActiveHeight}{\SI{350}{\cm}} 
\newcommand{\DSkFiducialCut}{\SI{10}{\cm}} 
\newcommand{\DSkFiducialVolumeDiameter}{\SI{335}{\cm}} 
\newcommand{\DSkFiducialHeight}{\SI{330}{\cm}} 
\newcommand{\DSkExposure}{\SI{100}{\tonne\year}}
\newcommand{\DSkRunTimePlanned}{\SI{5}{\year}}
\newcommand{\DSkRunTimePlannedVerbal}{\mbox{five years}}
\newcommand{\DSkSensitivityImprovementOneGeV}{\num{>50}}
\newcommand{\DSkSensitivityImprovementOneTeV}{\num{>50}}
\newcommand{\DSkSensitivityOneGeVBare}{1.2E-47}
\newcommand{\DSkSensitivityOneGeVUnit}{\SI{\DSkSensitivityOneGeVBare}{\square\cm}}
\newcommand{\DSkSensitivityTenGeVBare}{1.1E-46}
\newcommand{\DSkSensitivityTenGeVUnit}{\SI{\DSkSensitivityTenGeVBare}{\square\cm}}
\newcommand{\DSkExtendedExposure}{\SI{200}{\tonne\year}}
\newcommand{\DSkExtendedRunTimePlanned}{\SI{10}{\year}}
\newcommand{\DSkExtendedRunTimePlannedVerbal}{\mbox{ten years}}
\newcommand{\DSkExtendedSensitivityOneGeVBare}{7.4E-48}
\newcommand{\DSkExtendedSensitivityOneGeVUnit}{\SI{\DSkExtendedSensitivityOneGeVBare}{\square\cm}}
\newcommand{\DSkExtendedSensitivityTenGeVBare}{6.9E-47}
\newcommand{\DSkExtendedSensitivityTenGeVUnit}{\SI{\DSkExtendedSensitivityTenGeVBare}{\square\cm}}
\newcommand{\DSkNullFieldLightYieldProjected}{\SI{10}{\pe\per\keV}}
\newcommand{\DSkWithFieldLightYieldProjected}{\SI{9}{\pe\per\keV}}
\newcommand{\DSkNullFieldLightYieldRequirement}{\SI{8}{\pe\per\keV}}
\newcommand{\DSkDMSArThreeNineBackgroundCondition}{\SI{0.005}{\ev\per\bin}}
\newcommand{\DSkDMSArThreeNinePSDAcceptanceMax}{\SI{90}{\percent}}
\newcommand{\DSkROIEnergyRange}{\SIrange{30}{200}{\keVr}}
\newcommand{\DSkROIPERange}{\SIrange{50}{460}{\pe}}
\newcommand{\DSkROIElectronEquivalentEnergyRange}{\SIrange{7}{50}{\keVee}}
\newcommand{\DSkROIElectronEquivalentEnergyRangeSim}{\SIrange{<1}{50}{\keVee}}
\newcommand{\DSkROIPPRate}{\SI{200}{\ev\per\tonne\per\yr}}
\newcommand{\DSkROIPPBare}{2.0E4}
\newcommand{\DSkROIPPUnit}{\SI{\DSkROIPPBare}{\ev}}
\newcommand{\DSkROIBiTwoOneFourRate}{\SI{100}{\ev\per\tonne\per\yr}}
\newcommand{\DSkROIBiTwoOneFourUnit}{\SI{1.0E4}{\ev}}
\newcommand{\DSkROITotalUnit}{\SI{7.0E4}{\ev}}
\newcommand{\DSkROISimulatedNR}{\SI{1.0E6}{\ev}}
\newcommand{\DSkROISimulatedBeta}{\SI{3.5E6}{\ev}}
\newcommand{\DSkROISimulatedBetaBare}{\num{3.5E6}}
\newcommand{\DSkROISimulatedFractionBeta}{\SI{1}{\percent}}
\newcommand{\DSkUArPSDRejectionFromGFourDS}{\num{>3E9}}
\newcommand{\DSkAArThreeNineRate}{\SI{20}{\kilo\becquerel}}
\newcommand{\DSkUArChemicalPurity}{\SI{<0.1}{\ppb}}
\newcommand{\DSkUArThreeNineActivity}{\SI{10}{\micro\becquerel\per\kg}}
\newcommand{\DSkUArThreeNineDepletion}{\num{E5}}
\newcommand{\DSkDArThreeNineDepletion}{\DSfUArDepletion}
\newcommand{\DSkDArArThreeNineROIBare}{\num{1.8E6}}
\newcommand{\DSkUArArThreeNineROIBare}{\num{1.8E8}}
\newcommand{\DSkAArArThreeNineROIBare}{\num{2.6E11}}
\newcommand{\DSkDArArThreeNineFullBare}{\num{2.3E7}}
\newcommand{\DSkUArArThreeNineFullBare}{\num{2.3E9}}
\newcommand{\DSkAArArThreeNineFullBare}{\num{3.2E12}}
\newcommand{\DSkDArThreeNineAbatementMissing}{19}
\newcommand{\DSkUArKrActivity}{\SI{1}{\micro\becquerel\per\cubic\meter}}
\newcommand{\DSkTPCHeight}{\DSkActiveHeight} 
\newcommand{\DSkDriftLength}{\DSkActiveHeight} 
\newcommand{\DSkDriftField}{\SI{200}{\volt\per\centi\meter}}
\newcommand{\DSkExtractionField}{\SI{2.8}{\kilo\volt\per\centi\meter}}
\newcommand{\DSkElectroLuminescenceField}{\SI{4.2}{\kilo\volt\per\centi\meter}}
\newcommand{\DSkElectronMeanLife}{\SI{3}{\ms}}
\newcommand{\DSkDriftTime}{\SI{2.5}{\ms}}
\newcommand{\DSkXYResolution}{\SI{10}{\mm}}
\newcommand{\DSkZResolution}{\SI{1}{\mm}}
\newcommand{\DSkGasPocketThickness}{\SI{7}{\milli\meter}}
\newcommand{\DSkLArOverGridThickness}{\SI{3}{\milli\meter}}
\newcommand{\DSkLArOverGridPitch}{\SI{3}{\milli\meter}}
\newcommand{\DSkGridTrasparency}{\SI{97}{\percent}} 
\newcommand{\DSkAnodePillarsNumber}{\num{24}}
\newcommand{\DSkAnodePillarsDiameter}{\SI{3}{\mm}}
\newcommand{\DSkAnodePillarsSpacing}{\SI{500}{\mm}}
\newcommand{\DSkAnodePillarsRadialThermalShift}{\SI{2}{\cm}}
\newcommand{\DSkAnodePillarsWindowBowingPrevented}{\SI{1}{\cm}}
\newcommand{\DSkAnodePotential}{\mbox{ground}}
\newcommand{\DSkCathodePotential}{\SI{-73.8}{\kilo\volt}} 
\newcommand{\DSkGridPotential}{\SI{-3.8}{\kilo\volt}}
\newcommand{\DSkHHVTest}{\SI{-150}{\kilo\volt}}
\newcommand{\DSkHHVUHMWPEDesignBreakdown}{\SI{>100}{\kilo\volt}}
\newcommand{\DSkWindowTestHHV}{\SI{-65}{\kilo\volt}}
\newcommand{\DSkWindowTestFusedSilicaWindow}{\SI{6.5}{\mm}}
\newcommand{\DSkPMMATPCThickness}{\SI{5}{\cm}}
\newcommand{\DSkPMMATPCInnerPanelThickness}{\SI{0.1}{\cm}}
\newcommand{\DSkPMMAGdLoadingByMassFraction}{\SI{2}{\percent}}
\newcommand{\DSkPTFEPanelsHeight}{\SI{119}{\cm}}
\newcommand{\DSkPTFEPanelsWidth}{\SI{120}{\cm}}
\newcommand{\DSkPTFEPanelsThickness}{\SI{2.5}{\cm}}
\newcommand{\DSkTPBThickness}{\SI{200}{\micro\gram\per\square\centi\meter}}
\newcommand{\DSkCathodeToTopITOBotPlate}{\SI{5}{\cm}}
\newcommand{\DSkBotSiPMToBotITOBotPlate}{\SI{<2}{\mm}}
\newcommand{\DSkFieldCageRingsNumber}{\num{119}}
\newcommand{\DSkFieldCageRingsTubeHeight}{\SI{1.6}{\cm}}
\newcommand{\DSkFieldCageRingsSpacing}{\SI{2}{\cm}}
\newcommand{\DSkFieldCageMiddleResistorComponentsValue}{\SI{4}{\giga\ohm}}
\newcommand{\DSkFieldCageMiddleResistorValue}{\SI{1}{\giga\ohm}}
\newcommand{\DSkFieldCageMiddleResistorComponentsNumber}{\num{4}}
\newcommand{\DSkFieldCageTopResistorValue}{\SI{0.225}{\giga\ohm}}
\newcommand{\DSkCathodeWirePitch}{\SI{3}{\mm}}
\newcommand{\DSkWirePitch}{\SI{3}{\mm}}
\newcommand{\DSkCathodeWireThickness}{\SI{50}{\micro\m}}
\newcommand{\DSkCathodeWireTension}{\SI{1}{\newton}}
\newcommand{\DSkCathodeWireVerticalDeflection}{\SI{<2}{\mm}}
\newcommand{\DSkCathodeWireFrameDiameter }{\SI{325}{\cm}}
\newcommand{\DSkCathodeWireFrameRadialDeflection }{\SI{<1}{\mm}}
\newcommand{\DSkPTFEShrinkInPercent}{\SI{2}{\percent}}
\newcommand{\DSkPTFECageShrinkInCircumference}{\SI{14.4}{\cm}}
\newcommand{\DSkPTFECageShrinkInRadius}{\SI{2.2}{\cm}}
\newcommand{\DSkPTFECageShrinkInHeight}{\SI{3.6}{\cm}}
\newcommand{\DSkFieldCageRingCuTubesNumber}{\num{8}}
\newcommand{\DSkFieldCageCuCornerWingLength}{\SI{2.6}{\cm}}
\newcommand{\DSkAcrylicWindowThickness}{\SI{15}{\mm}}
\newcommand{\DSkAcrylicWindowTransparency}{\SI{90}{\percent}}
\newcommand{\DSkITOThickness}{\SI{15}{\nano\meter}}
\newcommand{\DSkITOTransparency}{\SI{98}{\percent}}
\newcommand{\DSkTopSiPMToBotITOTopPlate}{\SI{5}{\cm}}
\newcommand{\DSkExtractionGridVerticalDeflection }{\SI{<1}{\mm}}
\newcommand{\DSkAnodeVerticalDeflection }{\SI{<0.1}{\mm}}
\newcommand{\DSkExtractionGridThickness}{\SI{50}{\micro\m}}
\newcommand{\DSkCryostatSSThUActivityRequirement}{\SI{<1}{\milli\becquerel\per\kg}}
\newcommand{\DSkCryostatTitaniumThUActivityRequirement}{\SI{<1}{\milli\becquerel\per\kg}}
\newcommand{\DSkCryostatTitaniumIngotDiameter}{\SI{120}{\milli\meter}}
\newcommand{\DSkCryostatTitaniumIngotLength}{\SI{2}{\meter}}
\newcommand{\DSkCryostatTitaniumIngotCutLength}{\SI{0.7}{\meter}}
\newcommand{\DSkCryostatTitaniumLargeIngotMass}{\SI{\sim20}{\kg}}
\newcommand{\DSkCryostatTitaniumSampleThreeULimit}{\SI{<3.8E-2}{\milli\becquerel\per\kg}}
\newcommand{\DSkCryostatTitaniumSampleThreeThLimit}{\SI{<2.0E-1}{\milli\becquerel\per\kg}}
\newcommand{\DSkCryostatBottomLArNoBubblingHeatPerAreaDissipation}{\SI{60}{\milli\watt\per\square\cm}}
\newcommand{\DSkCryostatBottomLArNoBubblingHeatDissipation}{\SI{>5}{\kilo\watt}}
\newcommand{\DSkExternalCryostatDiameter}{\SI{3.75}{\meter}}
\newcommand{\DSkExternalCryostatHeight}{\SI{4.35}{\meter}}
\newcommand{\DSkInternalCryostatDiameter}{\SI{3.40}{\meter}}
\newcommand{\DSkInternalCryostatHeight}{\SI{4.00}{\meter}}
\newcommand{\DSkCryogenicsGasFlowTotal}{\SI{1000}{\standard\liter\per\minute}}
\newcommand{\DSkCryogenicsGasFlowNormalOperations}{\SI{200}{\standard\liter\per\minute}}
\newcommand{\DSkCryogenicsGasFlowGWL}{\SI{350}{\standard\liter\per\minute}}
\newcommand{\DSkCryogenicsGasFlowLWL}{\SI{650}{\standard\liter\per\minute}}
\newcommand{\DSkCryogenicsQdriveSpeed}{\SI{500}{\standard\liter\per\minute}}
\newcommand{\DSkCryogenicsLiquidFlow}{\SI{1}{\liter\per\minute}}
\newcommand{\DSkCryogenicsCryostatPowerLeak}{\SI{150}{\watt}}
\newcommand{\DSkCryogenicsFullCoolingPowerEquivalent}{\SI{8}{\kilo\watt}}
\newcommand{\DSkCryogenicsFullHeatingPowerEquivalent}{\SI{4}{\kilo\watt}}
\newcommand{\DSkCryogenicsTransferLineLength}{\chk{\SI{5}{\m}}}
\newcommand{\DSkCryogenicsLINLocalBufferVolume}{\SI{250}{\liter}}
\newcommand{\DSkCryogenicsLINLocalBackupTime}{\SI{3}{\days}}
\newcommand{\DSkCryogenicsLINStorageMass}{\SI{30}{\tonne}}
\newcommand{\DSkCryogenicsLINStorageBackupTime}{\SI{>30}{\days}}
\newcommand{\DSkCryogenicsRecoveryCryostatOne}{\mbox{Recovery~I}}
\newcommand{\DSkCryogenicsRecoveryCryostatTwo}{\mbox{Recovery~II}}
\newcommand{\DSkCryogenicsRecoveryCryostatPowerLeak}{\SI{150}{\watt}}
\newcommand{\DSkCryogenicsRecoveryExchangerEfficiency}{\SI{95}{\percent}}
\newcommand{\DSkCryogenicsRecoveryExchangerInefficiency}{\SI{5}{\percent}}
\newcommand{\DSkCryogenicsRecoveryExchangerCoolingPower}{\SI{0.4}{\kilo\watt}}
\newcommand{\DSkCryogenicsRecoveryExchangerLINPower}{\SI{1.2}{\kilo\watt}}
\newcommand{\DSkCryogenicsCapableLArMass}{\SI{50}{\tonne}}
\newcommand{\DSkCryogenicsDSfElectronMeanLife}{\SI{5}{\milli\second}}
\newcommand{\DSkCryogenicsCondenserCoolingPowerRange}{\SIrange{0}{5}{\kilo\watt}}
\newcommand{\DSkCryogenicsCondenserCoolingPowerMax}{\SI{5}{\kilo\watt}}
\newcommand{\DSkCryogenicsCondenserCoolingPowerMaxTested}{\SI{2.2}{\kilo\watt}}
\newcommand{\DSkCryogenicsCondenserCoolingPowerFilling}{\SI{5}{\kilo\watt}}
\newcommand{\DSkCryogenicsCondenserCoolingPowerNormal}{\SI{1.5}{\kilo\watt}}
\newcommand{\DSkCryogenicsCondenserCoolingPowerTPCOff}{\SI{150}{\watt}}
\newcommand{\DSkCryogenicsCondenserTubesNumber}{\num{61}}
\newcommand{\DSkCryogenicsCondenserTubesDiameter}{\SI{0.5}{\inch}}
\newcommand{\DSkCryogenicsCondenserTubesWallThickness}{\SI{0.035}{\inch}}
\newcommand{\DSkCryogenicsCondenserTubesLenghtLong}{\SI{5}{\inch}}
\newcommand{\DSkCryogenicsCondenserTubesLenghtShort}{\SI{3}{\inch}}
\newcommand{\DSkCryogenicsTubesDiameter}{\SI{1}{\inch}}
\newcommand{\DSkCryogenicsDSfCirculationSpeed}{\SI{50}{\standard\liter\per\minute}}
\newcommand{\DSkCryogenicsRadonTrapEfficiency}{\SI{100}{\percent}}
\newcommand{\DSkCryogenicsDetectorOperationPressure}{\SI{1.075}{\bar}}
\newcommand{\DSkCryogenicsDetectorOperationImperialPressure}{\SI{15.6}{\psi}}
\newcommand{\DSkCryogenicsPressureStability}{\SI{\pm0.1}{\psi}}
\newcommand{\DSkCryogenicsHeatExchangerArHeadPressure}{\SI{0.8}{\bar}}
\newcommand{\DSkCryogenicsAfterQDriveArPressure}{\SI{2.5}{\bar}}
\newcommand{\DSkCryogenicsAfterGetterArPressure}{\SI{2.0}{\bar}}
\newcommand{\DSkCryogenicsAfterRegulatorArPressure}{\SI{1.2}{\bar}}
\newcommand{\DSkCryogenicsDSfArPressureStability}{\SI{0.023}{\psi}}
\newcommand{\DSkCryogenicsLINSupplyPressure}{\SI{1}{\bar}}
\newcommand{\DSkCryogenicsInsulationVacuum}{\SI{1E-5}{\milli\bar}}
\newcommand{\DSkCryogenicsHeliumLeakDetectorSensitivity}{\SI{1E-10}{\standard\cubic\cm\per\second}}
\newcommand{\DSkCryogenicsHeliumLeakCheckRequirement}{\SI{2E-9}{\standard\cubic\cm\per\second}}
\newcommand{\DSkCryogenicsRuptureDiskLimit}{\SI{1.7}{\bar}}
\newcommand{\DSkCryogenicsReliefValveSetting}{\SI{1.6}{\bar}}
\newcommand{\DSkCryogenicsReliefValveTransducerMonitor}{\SI{0.1}{\bar}}
\newcommand{\DSkCryogenicsSpringLoadedReliefPressure}{\SI{10}{\bar}}
\newcommand{\DSkCryogenicsLArHeadHeight}{\SI{1.5}{\meter}}
\newcommand{\DSkCryogenicsUArTransportationPressure}{\SI{1.2}{\bar}}
\newcommand{\DSkCryogenicsHOne}{\mbox{H1D}}
\newcommand{\DSkCryogenicsHTwo}{\mbox{H2D}}
\newcommand{\DSkCryogenicsHThree}{\mbox{H3D}}
\newcommand{\DSkCryogenicsHFour}{\mbox{H4D}}
\newcommand{\DSkCryogenicsHFive}{\mbox{H5D}}
\newcommand{\DSkCVPressureDifferential}{\SI{100}{\milli\bar}}
\newcommand{\DSkSOneTilePileUpProbability}{\SI{0.4}{\percent}}
\newcommand{\DSkWIMPMinPE}{\SI{15}{\pe}}
\newcommand{\DSkWIMPMinPETimeWindow}{\SI{5}{\mu\second}}
\newcommand{\DSkWIMPMinTwoHundredns}{\SIrange{6}{8}{\pe}}
\newcommand{\DSkSOneMax}{\num{600}}
\newcommand{\DSkSTwoOverSOne}{\num{40}}
\newcommand{\DSkSTwoMaxPerChannel}{\SI{4000}{\pe}}
\newcommand{\DSkSTwoRateMaxPerChannel}{\SI{0.4}{\pe\per\nano\second}}
\newcommand{\DSkOverDSfAreaRatio}{\num{55}}
\newcommand{\DSkTriggerThresholdHits}{\num{7}}
\newcommand{\DSkTriggerThresholdWindow}{\SI{200}{\nano\second}}
\newcommand{\DSkTriggerRandomRate}{\SI{0.1}{\hertz}}
\newcommand{\DSkTriggerArThreeNineRate}{\SI{1}{\hertz}}
\newcommand{\DSkTriggerDArThreeNineRate}{\SI{16}{\hertz}}
\newcommand{\DSkTriggerSurfaceRate}{\SI{27}{\hertz}}
\newcommand{\DSkTriggerTotalRate}{\SI{45}{\hertz}}
\newcommand{\DSkDarkCountHitsPerTwoHundred}{\SI{0.26}{\mbox{noise }\hits}}
\newcommand{\DSkDarkCountHitsPerMaxDriftTime}{\SI{3.3E3}{\mbox{noise }\hits}}
\newcommand{\DSkDarkCountHitsPerRecordLength}{\SI{1E4}{\mbox{noise }\hits}}
\newcommand{\DSkDataRate}{\SI{5.6}{\mega\byte\per\second}}
\newcommand{\DSkSingleTotRate}{\SI{1.3}{\mega\hertz}}
\newcommand{\DSkCrateDataTrasferRate}{\SI{200}{\mega\byte\per\second}}
\newcommand{\DSkElectronicsDynamicRange}{\SI{6}{\bit}}
\newcommand{\DSkDataStorageTotalDisk}{\SI{2}{\peta\byte}}
\newcommand{\DSkDataStorageTotalDiskNewProposal}{\SI{10}{\peta\byte}}
\newcommand{\DSkDataStorageTotalDiskNewProposalExtended}{\SI{20}{\peta\byte}}
\newcommand{\DSkDataStorageLNGSShortDisk}{\SI{20}{\tera\byte}}
\newcommand{\DSkDSfDataReductionFactor}{\numrange{3}{4}}
\newcommand{\DSkOffLineCoresRealtimeReconNumber}{\num{100}}
\newcommand{\DSkOffLineCoresTotalNewProposal}{\num{1500}}
\newcommand{\DSkComputingRealtimeMaxEventRate}{\SI{200}{\hertz}}
\newcommand{\DSkRealtimeCalibrationEventRate}{\SI{100}{\hertz}}
\newcommand{\DSkOffLineCoresSimulationNumber}{\num{1000}}
\newcommand{\DSkOffLineCoresReprocessOneYearNumber}{\num{2000}}
\newcommand{\DSkAnnualDataProduction}{\SI{2}{\peta\byte}}
%Luca Added 05/19
\newcommand{\DSkPMMATPCInnerPanelThicknessESR}{\SI{3}{\mm}}
\newcommand{\DSkPMMATPCBackPanelThicknessESR}{\SI{4}{\mm}}
\newcommand{\DSkPMMAVetoPanelThickness}{\SI{10}{\cm}}
\newcommand{\DSkVetoLArThickness}{\SI{40}{\cm}} 
\newcommand{\DSkEdgeActiveVolumeShrinkage}{\SI{2.7}{\cm}} 
\newcommand{\DSkESRReflectivity}{\SI{98}{\percent}}
\newcommand{\DSkESRThickness}{\SI{50}{\micro\meter}} 
\newcommand{\LArRelativePermittivity}{\SI{1.54}}
\newcommand{\GArRelativePermittivity}{\SI{1.03}}
\newcommand{\DSkCathodePotentialNew}{\SI{-52.6}{\kilo\volt}}
\newcommand{\DSkGridPotentialNew}{\SI{-3.78}{\kilo\volt}}
\newcommand{\DSkMultiplicationField}{\SI{4.2}{\kilo\volt\per\centi\meter}}
\newcommand{\CleviosFirstTestSampleMass}{\SI{100}{\gram}}
\newcommand{\CleviosSampleThicknessFour}{\SI{4}{\micro\meter}}
\newcommand{\CleviosSampleThicknessEight}{\SI{8}{\micro\meter}}
\newcommand{\CleviosSampleThicknessTwelve}{\SI{12}{\micro\meter}}
\newcommand{\CleviosTestAbsorptionFour}{\SI{1.5}{\percent}}
\newcommand{\DSkCommissioningTime}{\SI{\le 60}{\day}}
\newcommand{\DSkLArBoilingThreshold}{\SI{60}{\milli\watt\per\centi\meter\squared}}
\newcommand{\DSkLArBoilingThresholdDepth}{\SI{3}{\meter}}
\newcommand{\DSkCryogenicsAArFlowTotal}{\SI{10000}{\standard\liter\per\minute}}
\newcommand{\DSkVetoIABThickness}{\SI{40}{\centi\meter}}
\newcommand{\DSkVetoOABThickness}{\SI{40}{\centi\meter}}
\newcommand{\DSkVetoGdASThickness}{\SI{10}{\centi\meter}}
\newcommand{\DSkVetoTotalPDMs}{\num{3000}}   %% Added Marco Oct 2019
\newcommand{\DSkVetoIABPDMs}{\num{2000}}
\newcommand{\DSkVetoOABPDMs}{\num{1000}}
\newcommand{\DSkVetoGdAsSheetThickness}{\SI{5}{\cm}} 
\newcommand{\DSkVetoMaxSectorPerSide}{\num{5}}
\newcommand{\DSkVetoGdPercentage}{\SIrange[range-units=single]{1}{2}{\percent}}  %% updated by Xiang, new number is from Gemma
\newcommand{\DSkVetoPDMTPCineff}{\num{2.4E-4}}
\newcommand{\DSkVetoPDMVetoineff}{\num{0.08}}
\newcommand{\DSkVetoPDMNeutronNum}{\num{2000}}
\newcommand{\DSkVetoPDMNeutronResidualBackground}{\num{0.04}}
\newcommand{\DSkVetoPMMATPCineff}{\num{3.3E-4}}
\newcommand{\DSkVetoPMMAVetoineff}{\num{0.10}}
\newcommand{\DSkVetoPMMANeutronNum}{\num{5}}
\newcommand{\DSkVetoPMMANeutronResidualBackground}{\num{<E-3}}
\newcommand{\DSkVetoGdASTPCineff}{\num{2.3E-5}}
\newcommand{\DSkVetoGdASVetoineff}{\num{0.10}}
\newcommand{\DSkVetoGdASNeutronNum}{\num{750}}
\newcommand{\DSkVetoGdASNeutronResidualBackground}{\num{0.002}}
\newcommand{\DSkVetoTotalNeutronResidualBackground}{\num{<0.05}}
\newcommand{\DSkVetoTimeCut}{\SI{800}{\micro\second}} %% updated by Xiang, new number is from Gemma
%Xiang added 05/19
\newcommand{\DSkTPBCoverage}{\SI{100}{\percent}}
\newcommand{\CleviosSecondTestSampleMass}{\SI{1}{\kg}}
\newcommand{\DSkActiveMassRatio}{\SI{97.3}{\percent}}
\newcommand{\HVFTs}{\mbox{HVFTs}}
\newcommand{\HV}{\mbox{HV}}
\newcommand{\pDUNECryostatInnerWidth}{\SI{8548}{\mm}}
\newcommand{\pDUNECryostatInnerHeight}{\SI{7900}{\mm}}
\newcommand{\pDUNELiquidHeight}{\SI{7500}{\mm}}
\newcommand{\pDUNEWallHeatLeakArea}{\SI{6.5}{\W\per\square\m}}
\newcommand{\pDUNECryostatHeatLoad}{\SI{2.7}{\kilo\W}}
\newcommand{\TPCPdmPower}{\SI{1.5}{\kilo\W}}
\newcommand{\VetoPdmPower}{\SI{0.5}{\kilo\W}}
\newcommand{\DSkUArTurnOverTime}{\SI{20}{\day}}
\newcommand{\DSkAArTurnOverTime}{\SI{30}{\day}}
\newcommand{\DSkAArCryogenicsTotalPower}{\SI{10}{\kilo\W}}
\newcommand{\DSkUArCryogenicsTotalPower}{\SI{500}{\W}}
\newcommand{\pDUNEAArTopPressure}{\SI{1.075}{\bara}}
\newcommand{\DSkCondenserTubeNumber}{\num{127}}
\newcommand{\DSkCryogenicsRadonLevelAfterTrap}{\SI{<2}{\micro\becquerel\per\kg}}
\newcommand{\DSkSiPMDCRSpecificationBig}{\SI{0.08}{\hertz\per\square\milli\meter}}
\newcommand{\DSkTileDCRSpecificationBig}{\SI{200}{\hertz}}
\newcommand{\DSkSingleTotRateBig}{\SI{1.6}{\mega\hertz}}
\newcommand{\DSkDriftTimeBig}{\SI{4}{\milli\second}}
\newcommand{\DSkTriggerTotalRateBig}{\SI{50}{\hertz}}
\newcommand{\DSkVetoFVTPCcut}{\SI{30}{\cm}}
\newcommand{\DSpZeroPdmsNumber}{\num{50}}
\newcommand{\DSpZeroDriftLength}{\SI{12}{\cm}}
\newcommand{\DSpZeroMBNumber}{\num{2}}
\newcommand{\DSpMBNumber}{\num{18}}
\newcommand{\DSpSipmsNumber}{\num{\sim~9000}}
\newcommand{\DSpSipmsBondingRate}{\SI{3}{tiles~\per\day}}
\newcommand{\DSpSipmsBondingTime}{\SI{60}{\day}}
\newcommand{\Rn}{\ce{^220Rn}}
\newcommand{\Kr}{\ce{^{83m}Kr}}
\newcommand{\ArThirtyNine}{\ce{^39Ar}}
\newcommand{\Co}{\ce{^60Co}}
\newcommand{\Ba}{\ce{^133Ba}}
\newcommand{\Cs}{\ce{^137Cs}}
\newcommand{\CoEnergy}{\SI{122}{\keV}}
\newcommand{\BaEnergy}{\SI{356}{\keV}}
\newcommand{\CsEnergy}{\SI{662}{\keV}}
\newcommand{\YBe}{\ce{YBe}}
\newcommand{\YBeNeutronEnergy}{\SI{157}{\keV}}
\newcommand{\TungstenShieldThickness}{\SI{15}{\cm}}
\newcommand{\fNinety}{\mbox{f90}}
\newcommand{\DSkVetoFVTPCcutz}{\SI{70}{\cm}}
\newcommand{\DSzApproximateMass}{\SI{\sim~10}{\kg}}

%--- DS Prototype
\newcommand{\DSpApproximateMass}{\SI{\sim~1}{\tonne}}
\newcommand{\DSpTotalMass}{\SI{800}{\kg}}
\newcommand{\DSpActiveMass}{\SI{360}{\kg}}
\newcommand{\DSpBackgroundRate}{\SI{5}{\Hz}}
\newcommand{\DSpDataRate}{\SI{1}{\tera\byte\per\day}}
\newcommand{\DSpTPCHeight}{\SI{60}{\cm}}
\newcommand{\DSpTPBThickness}{\DSkTPBThickness}
\newcommand{\DSpElectrodesWindowsThickness}{\SI{5}{\cm}}
\newcommand{\DSpDriftField}{\DSkDriftField}
\newcommand{\DSpExtractionField}{\DSkExtractionField}
\newcommand{\DSpElectroLuminescenceField}{\DSkElectroLuminescenceField}
\newcommand{\DSpGasPocketThickness}{\DSkGasPocketThickness}
\newcommand{\DSpLArOverGridThickness}{\DSkLArOverGridThickness}
\newcommand{\DSpDriftLength}{\SI{58}{\cm}}
\newcommand{\DSpDriftTime}{\SI{7}{\us}}
\newcommand{\DSpCryostatSSMass}{\SI{600}{\kg}}
\newcommand{\DSpCryostatTiMass}{\SI{340}{\kg}}
\newcommand{\DSpCryostatOuterVesselDiameter}{\SI{1210}{\mm}}
\newcommand{\DSpCryostatInnerVesselDiameter}{\SI{1010}{\mm}}
\newcommand{\DSpCryostatWallThickness}{\SI{5}{\mm}}
\newcommand{\DSpCryogenicsGasFlowTotal}{\SI{500}{\standard\liter\per\minute}}
\newcommand{\DSpFieldCageRingsNumber}{\num{28}}
\newcommand{\DSpTPCDiameter}{\SI{72}{\cm}}
\newcommand{\DSpCathodePotential}{\SI{-15}{\kilo\volt}}
\newcommand{\DSpPMMAPanelHeight}{\SI{30}{\cm}}
\newcommand{\DSpPMMAPanelWidth}{\SI{30}{\cm}}
\newcommand{\DSpPMMAPanelsNumber}{\num{16}}
\newcommand{\DSpPdmsHalfNumber}{\num{185}}
\newcommand{\DSpPdmsNumber}{\num{370}}
\newcommand{\DSpSQBsNumber}{\num{5}}
\newcommand{\DSpTRBsNumber}{\num{4}}
\newcommand{\DSpPhaseZero}{\mbox{Proto~0}}
\newcommand{\DSpPhaseOne}{\mbox{Proto~I}}
\newcommand{\DSpPhaseTwo}{\mbox{Proto~II}}
%--- DS-LM
\newcommand{\DSlRunTimePlanned}{\SI{1}{\year}}
\newcommand{\DSlExposure}{\SI{1E5}{\kg\day}}
\newcommand{\DSlFiducialMass}{\SI{260}{\kg}}
\newcommand{\DSlApproxMassScale}{\SI{1}{\tonne}}
\newcommand{\DSkHighMassThreshold}{\SI{30}{\GeV\per\square\c}}
\newcommand{\DSlLowMassThreshold}{\SI{10}{\GeV\per\square\c}}
\newcommand{\DSlCryostatUCont}{\SI{1}{\milli\becquerel\per\kg}}
\newcommand{\DSlCryostatThCont}{\SI{1}{\milli\becquerel\per\kg}}
\newcommand{\DSlCryostatCoCont}{\SI{1}{\milli\becquerel\per\kg}}
\newcommand{\DSlCryostatPDMCont}{\SI{0.01}{\milli\becquerel\per\pdm}}
\newcommand{\DSlUArCont}{\SI{1}{\micro\becquerel\per\kg}}
\newcommand{\DSlRadialCut}{\SI{5}{\cm}}
\newcommand{\DSkHighMassSensitivityImprovementOverLZ}{\num{5}}
\newcommand{\DSkHighMassSensitivityImprovementOverLZVerbal}{\mbox{five}}
%--- DSk SQB
\newcommand{\DSkSQBDModArray}{\num[product-units=power]{5 x 5}}
\newcommand{\DSkSQBTRBSize}{\SI{25}{\cm}}
\newcommand{\DSkArraySQBNumber}{\num{156}}
\newcommand{\DSkArrayTRBNumber}{\num{16}}
\newcommand{\DSkSQBNumber}{\num{312}}
\newcommand{\DSkTRBNumber}{\num{32}}
\newcommand{\DSkSQBPdmsNumber}{\num{25}}
\newcommand{\DSkTRBPdmsNumber}{\num{15}}
\newcommand{\DSkSQBArea}{\SI[product-units=power]{25 x 25}{\square\cm}}
\newcommand{\DSkTRBArea}{\SI[product-units=power]{15 x 25}{\square\cm}}
%--- Mother Boards
\newcommand{\DSkMB}{\mbox{MB}}
\newcommand{\DSkMBs}{\mbox{\DSkMB s}}
\newcommand{\DSkMBWeight}{\SI{2}{\kg}}
\newcommand{\DSkMBsNumber}{\num{220}}
\newcommand{\DSkMBStripsNumber}{\num{440}}
%--- DSk Photodetector Modules
\newcommand{\DSkPdm}{\mbox{PDM}}
\newcommand{\DSkPdms}{\mbox{\DSkPdm s}}
\newcommand{\DSkPdmAreaStd}{\DSkTileAreaStd}
\newcommand{\DSkPdmsGap}{\SI{2}{\milli\meter}}
\newcommand{\DSkPdmsGeometricEfficiency}{\SI{92.5}{\percent}}
\newcommand{\DSkPdmsFirstBatchNumber}{\num{50}}
\newcommand{\DSkPdmsSecondBatchNumber}{\num{400}}
\newcommand{\DSkPdmsNumber}{\DSkTilesNumber}
\newcommand{\DSkPdmsNumberWithSpares}{\num{10000}}
\newcommand{\DSkPdmIndiumPelletVolume}{\SI{1}{\cubic\mm}}
\newcommand{\DSkPdmFEBNumber}{\num{3}}
\newcommand{\DSkPdmTransmitterNumber}{\num{1}}
\newcommand{\DSkPdmPDESpecification}{\SI{40}{\percent}}
\newcommand{\DSkPdmDCRSpecification}{\SI{0.1}{\hertz\per\square\mm}}
\newcommand{\DSkPdmWeight}{\SI{250}{\g}}
\newcommand{\DSkPdmsContructionTime}{\SI{2.5}{\year}}
\newcommand{\DSkPdmsCleanRoomSurface}{\SI{700}{\square\meter}}
%--- DSk Tiles
\newcommand{\DSkTileAmplitudeSNRSpecification}{\num{3}}
\newcommand{\DSkTileAmplitudeThreshold}{\SI{1}{\pe}}
\newcommand{\DSkTileChargeSNRSpecification}{\num{8}}
\newcommand{\DSkTileChargeThreshold}{\SI{0.5}{\pe}}
\newcommand{\DSkTileTimeResolutionSpecification}{\SI{10}{\nano\second}}
\newcommand{\DSkTileDynamicRangeSpecification}{\SI{50}{\pe}}
\newcommand{\DSkTileAreaMin}{\SI[product-units=power]{20 x 20}{\square\mm}}
\newcommand{\DSkTileAreaXtr}{\SI[product-units=power]{35 x 35}{\square\mm}}
\newcommand{\DSkTileAreaStd}{\SI[product-units=power]{50 x 50}{\square\mm}}
\newcommand{\DSkTestedTileAreaStd}{\SI{24}{\square\cm}}
\newcommand{\DSkTilesArea}{\SI{21}{\square\meter}}
\newcommand{\DSkTilesHalfNumber}{\num{4140}}
\newcommand{\DSkTilesNumber}{\num{8280}}
\newcommand{\DSkTileSNR}{\num{5}}
\newcommand{\DSkTilePower}{\SI{250}{\milli\watt}}
\newcommand{\DSkTileDensityPower}{\SI{100}{\micro\watt\per\square\mm}}
\newcommand{\DSkTileSapphireSupportThickness}{\SI{0.7}{\mm}}
\newcommand{\DSkTileswithSOneSTwo}{\numrange{6}{8}}
\newcommand{\DSkTileDCRSpecification}{\SI{250}{\hertz}}
\newcommand{\DSkTileFillFactorSpecification}{\SI{90}{\percent}}
\newcommand{\DSkTileDeadTime}{\SI{100}{\nano\second}}
\newcommand{\DSkTileEpoxyThickness}{\SI{60}{\micro\meter}}
\newcommand{\DSkTileGoldBallsDiameter}{\SI{50}{\micro\meter}}
\newcommand{\DSkTileSiPMsMaxNumber}{\num{25}}
\newcommand{\DSkTileSiPMsCustomNumber}{\num{24}}
%--- DSk DAQ
\newcommand{\DSkDAQSOneAvgPE}{\SI{600}{\pe}}
\newcommand{\DSkDAQSTwoDigitizationWindow}{\SI{20}{\micro\second}}
\newcommand{\DSkDAQCratesNumber}{\mbox{O\num{10}}}
\newcommand{\DSkDAQSOneSizeTotal}{\SI{8}{\byte}}
\newcommand{\DSkDAQSOneSizeChannelID}{\SI{2}{\byte}}
\newcommand{\DSkDAQSOneSizeTiming}{\SI{4}{\byte}}
\newcommand{\DSkDAQSOneSizeCharge}{\SI{2}{\byte}}
\newcommand{\DSkDAQSTwoSamples}{\num{200}}
\newcommand{\DSkDAQSTwoSize}{\SI{300}{\byte}}
\newcommand{\DSKDAQClockCycle}{\SI{1}{\second}}
\newcommand{\DSKDAQClockRate}{\SI{50}{\mega\hertz}}
\newcommand{\DSKDAQClockTicksMax}{\num{E8}}
\newcommand{\DSKDAQClockTickSize}{\SI{4}{\byte}}
\newcommand{\DSKDAQClockDeadTimeFraction}{\num{1/400}}
\newcommand{\DSKDAQClockResetScale}{\si{\micro\second}}
\newcommand{\DSKDAQPLLClockRate}{\SI{100}{\mega\hertz}}
\newcommand{\DSkDAQSimulationAP}{\SI{10}{\percent}}
\newcommand{\DSkDAQSimulationDiCT}{\SI{15}{\percent}}
\newcommand{\DSkDAQADCBits}{\num{14}}
\newcommand{\DSkDAQADCSamplingRate}{\SI{125}{\mega\hertz}}
\newcommand{\DSkDAQADCDownSampledRate}{\SI{10}{\mega\hertz}}
\newcommand{\DSkDAQADCBinWidth}{\SI{100}{\nano\second}}
\newcommand{\DSkDAQADCMaxDeadTimePerSecond}{\SI{2.5}{\milli\second}}
\newcommand{\DSkDAQVetoWindow}{\SI{50}{\micro\second}}
\newcommand{\DSkDAQVetoHitSamples}{\SI{20}{\smp}}
\newcommand{\DSkDAQVetoHitSize}{\SI{30}{\byte}}
\newcommand{\DSkDAQVetoHitAvgNumber}{\SI{300}{\hits}}
\newcommand{\DSkDAQGlobalEventSizeUpperLimit}{\SI{1}{\mega\byte}}
\newcommand{\DSkDAQEthernetRate}{\SIrange{1}{10}{\giga\bit\per\second}}
%--- DSk HLST
\newcommand{\DSkHLSTBufferNumber}{\mbox{O(\num{10})}}
\newcommand{\DSkHLSTBufferSize}{\num{512}}
\newcommand{\DSkHLSTRateMax}{\SI{400}{Hz}}
%--- DSk FEB
\newcommand{\DSkFEBTIANumber}{\num{4}}
%--- DSk SiPMs
\newcommand{\DSkSiPMSPADSizeMin}{\SI[product-units=power]{20 x 20}{\square\micro\meter}}
\newcommand{\DSkSiPMSPADSizeStd}{\SI[product-units=power]{25 x 25}{\square\micro\meter}}
\newcommand{\DSkSiPMSPADSizeMax}{\SI[product-units=power]{35 x 35}{\square\micro\meter}}
\newcommand{\DSkSiPMSPADSizeTripleDoping}{\SI[product-units=power]{30 x 30}{\square\micro\meter}}
\newcommand{\DSkSiPMSPADQuenchingResistorTripleDoping}{\SI{5}{\mega\ohm}}
\newcommand{\DSkSiPMSPADQuenchingResistorSingleDoping}{\SI{10}{\mega\ohm}}
\newcommand{\DSkSiPMInactiveGapSpecification}{\SI{100}{\um}}
\newcommand{\DSkSiPMPDESpecification}{\SI{45}{\percent}}
\newcommand{\DSkSiPMDCRSpecification}{\SI{0.1}{\hertz\per\square\mm}}
\newcommand{\DSkSiPMTCNPSpecification}{\SI{60}{\percent}}
\newcommand{\DSkSiPMNUVHDLFRoomTempDCR}{\SI{100}{\kilo\hertz\per\square\mm}}
\newcommand{\DSkSiPMDCRLArTemperature}{\SI{E-2}{\hertz\per\square\mm}}
\newcommand{\DSkSiPMNUVHDLFLArTempDCR}{\SI{0.01}{\hertz\per\square\mm}}
\newcommand{\DSkSiPMNUVHDLFLArTempTCNP}{\SI{28}{\percent}}
\newcommand{\DSkSiPMsNumber}{\num{125040}}
\newcommand{\DSkSiPMPolysiliconResistanceTempVariationRange}{\numrange{2}{20}}
\newcommand{\DSkSiPMAreaMin}{\SI[product-units=power]{4 x 4}{\square\mm}}
\newcommand{\DSkSiPMAreaStd}{\SI[product-units=power]{5 x 5}{\square\mm}}
\newcommand{\DSkSiPMAreaMax}{\SI[product-units=power]{10 x 10}{\square\mm}}
\newcommand{\DSkSiPMAreaMaxcm}{\SI{1}{\square\cm}}
\newcommand{\DSkSiPMAreaCustom}{\SI[product-units=power]{7.9 x 11.7}{\square\mm}}
\newcommand{\DSkSiPMBumpsNumber}{\numrange{10}{15}}
\newcommand{\DSkSiPMBumpsDiameterMinimum}{\SI{100}{\um}}
\newcommand{\DSkSiPMActiveEdgeToCutEdgeDistance}{\SI{40}{\um}}
\newcommand{\DSkSiPMCapacitancePerArea}{\SI{50}{\pico\farad\per\square\mm}}
\newcommand{\DSkSiPMSPEResolution}{\SI{5}{\percent}}
\newcommand{\DSkSiPMGainRange}{\numrange{E5}{E6}}
\newcommand{\DSkSiPMDynamicRange}{\SI{E4}{\pe\per\square\mm}}
\newcommand{\DSkSiPMBaselineAmplWindow}{\SI{100}{\nano\second}}
\newcommand{\DSkSiPMSNRChargeWindow}{\SI{1}{\micro\second}}
%--- TIA
\newcommand{\DSkTIAGain}{\SI{0.5}{\milli\volt\per\micro\ampere}}
\newcommand{\DSkTIAsPerTile}{\num{12}}
\newcommand{\DSkTIAPower}{\SI{40}{\milli\watt}}
\newcommand{\DSkFourTIAsPower}{\SI{160}{\milli\watt}}
\newcommand{\DSkTIAOpAmpModel}{LMH~6629}
\newcommand{\DSkTIAOpAmpSurface}{\SI{0.1}{\square\cm}}
\newcommand{\DSkTIAOpAmpRoomTempGBP}{\SI{4}{\giga\hertz}}
\newcommand{\DSkTIAOpAmpLArTempGBP}{\SI{11}{\giga\hertz}}
\newcommand{\DSkTIAOpAmpThreeDbBandwidth}{\SI{900}{\mega\hertz}}
\newcommand{\DSkTIAOpAmpAVol}{\SI{78}{\deci\bel}}
\newcommand{\DSkTIAOpAmpInputVoltageNoiseDensity}{\SI{0.69}{\nano\volt\per\sqrt{\hertz}}}
\newcommand{\DSkTIAOpAmpInputCurrentNoiseDensity}{\SI{2.6}{\pico\ampere\per\sqrt{\hertz}}}
\newcommand{\DSkTIANoiseDensityFrequencyThreshold}{\SI{1}{\mega\hertz}}
\newcommand{\DSkTIAOpAmpOutputNoiseDensityRMS}{\SI{100}{\micro\volt}}
\newcommand{\DSkTIAInputResistance}{\SI{20}{\ohm}}
\newcommand{\DSkTIAFeedbackResistance}{\SI{500}{\ohm}}
\newcommand{\DSkTIAFeedbackResistanceRange}{\SIrange{2}{6}{\kilo\ohm}}
\newcommand{\DSkTIANonInvPinResistanceRange}{\SIrange{10}{20}{\ohm}}
\newcommand{\DSkTIANonInvPinResistanceVnoTotImpact}{\SI{38}{\percent}}
\newcommand{\DSkTIAFeedbackCapacitance}{\SI{1}{\pico\farad}}
\newcommand{\DSkTIAFeedbackCapacitanceScale}{\SI{1}{\pico\farad}}
\newcommand{\DSkTIANoiseEquivalentResistor}{\SI{22}{\ohm}}
\newcommand{\DSkTIATimeResolution}{\SI{10}{\nano\second}}
\newcommand{\DSkTIABandwidthForTimeResolution}{\SIrange{20}{30}{\mega\hertz}}
\newcommand{\DSkTIABandwidthForFastPeak}{\SI{50}{\mega\hertz}}
\newcommand{\DSkTIAOpAmpGBP}{\SI{4}{\giga\hertz}}
%--- Adder
\newcommand{\DSkAdderPower}{\SI{50}{\milli\watt}}
\newcommand{\DSkAdderOpAmpModelOld}{LMH~6624}
\newcommand{\DSkAdderOpAmpModelNew}{OPA~838}
%--- Transmitter
\newcommand{\DSkTransmitterGainVal}{\SI{27}{\volt\per\volt}}
\newcommand{\DSkTransmitterGainFlatness}{\SI{1}{\decibel}}
\newcommand{\DSkTransmitterBandwidth}{\SI{65}{\mega\hertz}}
\newcommand{\DSkTransmitterBandwidthFlatness}{}
\newcommand{\DSkTransmitterInputVoltageNoiseDensity}{\SI{2.3}{\nano\volt\per\sqrt{\hertz}}}
\newcommand{\DSkTransmitterOutputNoiseDensityRMS}{\SI{600}{\micro\volt}}
\newcommand{\DSkTransmitterOutputSwing}{\SI{1.3}{\volt}}
\newcommand{\DSkTransmitterOutputCompression}{\SI{1}{\decibel}}
\newcommand{\DSkTransmitterSPEVal}{\SI{12}{\milli\volt}}
\newcommand{\DSkTransmitterSNR}{\num{20}}
\newcommand{\DSkTransmitterDynamicRange}{\num{100}}
\newcommand{\DSkTransmitterCryoPower}{\SI{5}{\milli\watt}}
%--- Cabling
\newcommand{\DSkCablingTwistedPairAvgLength}{\SI{7}{\meter}}
\newcommand{\DSkCablingTwistedPairImpedance}{\SI{100}{\ohm}}
\newcommand{\DSkCablingTwistedPairFTDb}{\SI{60}{\mega\hertz}}
\newcommand{\DSkCablingTwistedPairFSDb}{\SI{100}{\mega\hertz}}
\newcommand{\DSkCablingTwistedPairCrossTalk}{\SI{40}{\decibel}}
\newcommand{\DSkCablingTwistedPairGauge}{\mbox{AWG 26}}
\newcommand{\DSkCablingTwistedPairMinBendingRadiusAfterGrouping}{\SI{10}{\centi\meter}}
%--- Steering Modules
\newcommand{\DSkSM}{\mbox{SM}}
\newcommand{\DSkSMs}{\mbox{\DSkSM s}}
\newcommand{\DSkSMTilesNumber}{\num{50}}
\newcommand{\DSkSMPower}{\SI{<200}{\milli\watt}}
\newcommand{\DSkSMOutputLowVoltage}{\SI{\pm 2}{\volt}}
\newcommand{\DSkSMOutputHighVoltage}{\SI{150}{\volt}}
\newcommand{\DSkSMsNumber}{\DSkMBsNumber}
%--- Discriminator
\newcommand{\DSkDiscriminatorThresholdRange}{\SIrange{0.5}{0.7}{\pe}}
\newcommand{\DSkDiscriminatorThresholdMin}{\SI{0.3}{\pe}}
%--- WA
\newcommand{\DSkWAOpAmpModel}{OPA~847}
\newcommand{\DSkWAOpAmpGBP}{\SI{3}{\giga\hertz}}
\newcommand{\DSkWAOpAmpThreeDbBandwidth}{\SI{50}{\mega\hertz}}
\newcommand{\DSkWAOpAmpAVOL}{\SI{98}{\deci\bel}}
\newcommand{\DSkWAOpAmpInputVoltageNoiseDensity}{\SI{0.85}{\nano\volt\per\sqrt{\hertz}}}
\newcommand{\DSkWAOpAmpInputVoltageNoiseRMS}{\SI{11}{\micro\volt}}
\newcommand{\DSkWANoiseDensityFrequencyThreshold}{\SI{1}{\mega\hertz}}
\newcommand{\DSkWAOpAmpInputCurrentNoiseDensity}{\SI{2.5}{\pico\ampere\per\sqrt{\hertz}}}
\newcommand{\DSkWAGain}{\SI{28.8}{\volt\per\volt}}
\newcommand{\DSkWARiseTime}{\SI{7}{\nano\second}}
\newcommand{\DSkWASignalLength}{\chk{\SI{300}{\nano\second}}}
\newcommand{\DSkSteeringModuleTilesServed}{\num{50}}
\newcommand{\DSkSteeringModulePower}{\SI{<20}{\milli\watt}}
%--- Matched RC Filter
\newcommand{\DSkMatchedRCFilterTau}{\SI{400}{\nano\second}}
%---
\newcommand{\RGBHdSfFillFactor}{\SI{73}{\percent}}
\newcommand{\NUVHdSfFillFactor}{\SI{73}{\percent}}
\newcommand{\NUVHdLfFillFactor}{\SI{73}{\percent}}
\newcommand{\RGBHdSfRoomTempBreakdownVoltage}{\SI{28.0}{\volt}}
\newcommand{\NUVHdSfRoomTempBreakdownVoltage}{\SI{26.5}{\volt}}
\newcommand{\NUVHdLfRoomTempBreakdownVoltage}{\SI{32.0}{\volt}}
\newcommand{\RGBHdSfRoomTempPDE}{\SI{34}{\percent}}
\newcommand{\NUVHdSfRoomTempPDE}{\SI{50}{\percent}}
\newcommand{\NUVHdLfRoomTempPDE}{\SI{50}{\percent}}
\newcommand{\RGBHdSfRoomTempPeakPDEWavelength}{\SI{550}{\nano\meter}}
\newcommand{\NUVHdSfRoomTempPeakPDEWavelength}{\SI{410}{\nano\meter}}
\newcommand{\NUVHdLfRoomTempPeakPDEWavelength}{\SI{410}{\nano\meter}}
\newcommand{\RGBHdSfRoomTempDCR}{\SI{<300}{\kilo\hertz\per\square\mm}}
\newcommand{\NUVHdSfRoomTempDCR}{\SI{<150}{\kilo\hertz\per\square\mm}}
\newcommand{\NUVHdLfRoomTempDCR}{\SI{<100}{\kilo\hertz\per\square\mm}}
\newcommand{\RGBHdSfRoomTempDiCT}{\SI{20}{\percent}}
\newcommand{\NUVHdSfRoomTempDiCT}{\SI{25}{\percent}}
\newcommand{\NUVHdLfRoomTempDiCT}{\SI{25}{\percent}}
\newcommand{\RGBHdSfRoomTempDeCTAP}{\SI{20}{\percent}}
\newcommand{\NUVHdSfRoomTempDeCTAP}{\SI{2}{\percent}}
\newcommand{\NUVHdLfRoomTempDeCTAP}{\SI{2}{\percent}}
\newcommand{\RGBHdSfLINTempBreakdownVoltage}{\SI{23.6}{\volt}}
\newcommand{\NUVHdSfLINTempBreakdownVoltage}{\SI{21.5}{\volt}}
\newcommand{\NUVHdLfLINTempBreakdownVoltage}{\SI{27.0}{\volt}}
\newcommand{\RGBHdSfLINTempPDE}{\SI{25}{\percent}}
\newcommand{\NUVHdSfLINTempPDE}{\SI{40}{\percent}}
\newcommand{\NUVHdLfLINTempPDE}{\SI{40}{\percent}}
\newcommand{\RGBHdSfLINTempPeakPDEWavelength}{\SI{550}{\nano\meter}}
\newcommand{\NUVHdSfLINTempPeakPDEWavelength}{\SI{410}{\nano\meter}}
\newcommand{\NUVHdLfLINTempPeakPDEWavelength}{\SI{410}{\nano\meter}}
\newcommand{\RGBHdSfLINTempBreadkdownVoltage}{\SI{23.6}{\volt}}
\newcommand{\NUVHdSfLINTempBreadkdownVoltage}{\SI{21.5}{\volt}}
\newcommand{\NUVHdLfLINTempBreadkdownVoltage}{\SI{27.0}{\volt}}
\newcommand{\RGBHdSfLINTempDCR}{\SI{8}{\hertz\per\square\mm}}
\newcommand{\NUVHdSfLINTempDCR}{\SI{0.5}{\hertz\per\square\mm}}
\newcommand{\NUVHdLfLINTempDCR}{\SI{5E-3}{\hertz\per\square\mm}}
\newcommand{\RGBHdSfLINTempDiCT}{\SI{15}{\percent}}
\newcommand{\NUVHdSfLINTempDiCT}{\SI{15}{\percent}}
\newcommand{\NUVHdLfLINTempDiCT}{\SI{15}{\percent}}
\newcommand{\RGBHdSfLINTempDeCTAP}{\SI{10}{\percent}}
\newcommand{\NUVHdSfLINTempDeCTAP}{\SI{25}{\percent}}
\newcommand{\NUVHdLfLINTempDeCTAP}{\SI{15}{\percent}}
\newcommand{\RGBHdSfLINTempOV}{\SI{7}{\volt}}
\newcommand{\NUVHdSfLINTempOV}{\SI{5}{\volt}}
\newcommand{\NUVHdLfLINTempOV}{\SI{5}{\volt}}
%--- SiPM Performance
\newcommand{\RGBHdSfLRqMaxThreePThreeSArea}{\SI{9}{\square\centi\meter}}
\newcommand{\RGBHdSfLRqStdIntGate}{\SI{20}{\nano\second}}
\newcommand{\NUVHdSfHRqPeakDuration}{\SI{20}{\nano\second}}
\newcommand{\NUVHdLfHRqStdFourPFourSArea}{\SI{4}{\square\centi\meter}}
\newcommand{\FBKSiPMAmplDispersion}{\SI{4}{\percent}}
\newcommand{\FBKSiPMChargeDispersion}{\SI{2}{\percent}}
%--- Rq
\newcommand{\LRqTimeScale}{\mbox{a few hundreds of \si{\nano\second}}}
\newcommand{\HRqTimeScale}{\mbox{a few \si{\micro\second}}}
\newcommand{\NUVHdLfRoomTempRq}{\SI{2}{\mega\ohm}}
\newcommand{\NUVHdLfLINTempRq}{\SI{40}{\mega\ohm}}
\newcommand{\RGBHdSfLRqLINTempRechargeTime}{\SI{70}{\nano\second}}
\newcommand{\NUVHdSfHRqLINTempRechargeTime}{\SI{2.5}{\micro\second}}
\newcommand{\NUVHdLfHRqLINTempRechargeTime}{\SI{2.5}{\micro\second}}
%--- Proto
\newcommand{\DSkProtoActiveMass}{\SI{800}{\kg}}
\newcommand{\DSkProtoCryostatOuterDiameter}{\SI{128}{\cm}}
\newcommand{\DSkProtoCryostatHeight}{\SI{100}{\cm}}
%--- CATIROC
\newcommand{\CATIROCNumChannels}{\num{16}}
\newcommand{\CATIROCChargeResolution}{\SI{\sim~30}{\femto\coulomb}}
\newcommand{\CATIROCDynamicRange}{\SIrange{160}{100E3}{\femto\coulomb}}
\newcommand{\CATIROCGainFactor}{\num{4}}
\newcommand{\CATIROCGainFactorBits}{\num{8}}
\newcommand{\CATIROCMaxShapeTime}{\SI{100}{\nano\second}}
\newcommand{\CATIROCADCBits}{\num{10}}
\newcommand{\CATIROCSamplingRate}{\SI{160}{\mega\hertz}}
\newcommand{\CATIROCFastShaper}{\SI{5}{\nano\second}}
\newcommand{\CATIROCAutoTriggerThreshold}{\SI{50}{\femto\coulomb}}
\newcommand{\CATIROCClockBits}{\num{26}}
\newcommand{\CATIROCClockRate}{\SI{40}{\mega\hertz}}
\newcommand{\CATIROCCoarseTimeResolution}{\SI{25}{\nano\second}}
\newcommand{\CATIROCClockOverflowTime}{\SI{1.67}{\second}}
\newcommand{\CATIROCFineTimeResolution}{\SI{1}{\nano\second}}
%--- Vetoes
\newcommand{\DSkVetoPMTDiameter}{\SI{20}{\inch}}
\newcommand{\DSkVetoPMTsNumber}{\num{230}}
\newcommand{\DSkVetoPMTTMFPDELossRequirement}{\SI{10}{\percent}}
\newcommand{\DSkVetoPMTUTHActivity}{\SI{1}{\becquerel\per\kilo\gram}}
\newcommand{\DSkVetoPMTSPEHeight}{\SI{\sim~10}{\milli\volt}}
\newcommand{\DSkVetoPMTSPEWidth}{\SI{10}{\nano\second}}
\newcommand{\DSkVetoPMTDCR}{\SI{30}{\kilo\hertz}}
\newcommand{\DSkVetoPMTAfterPulseProb}{\SI{<3}{\percent}}
\newcommand{\DSkVetoPMTAfterPulseTime}{\SI{4.5}{\micro\second}}
\newcommand{\DSkVetoPMTMuCagePermeability}{\num{3E4}}
\newcommand{\DSkVetoPMTMuCageRadius}{\SI{30}{\centi\meter}}
\newcommand{\DSkVetoPMTMuCageCellSize}{\SI{50}{\milli\meter}}
\newcommand{\DSkVetoPMTMuCageWireDiameter}{\SI{1}{\milli\meter}}
\newcommand{\DSkVetoPMTMuCageLightLoss}{\SI{4}{\percent}}
\newcommand{\DSkVetoPMTMuCageExpectedReductionFactor}{\num{\sim3.5}}
\newcommand{\DSkVetoPMTMuCageMeasuredReductionFactor}{\num{2}}
\newcommand{\DSkVetoDAQSampleRate}{\SI{1}{\giga\sample\per\second}}
\newcommand{\DSkVetoDAQADCMinBits}{\num{10}}
\newcommand{\DSkVetoPreAmpBandwidth}{\SI{300}{\mega\hertz}}
\newcommand{\DSkVetoPreAmpGain}{\SI{10}{\volt\per\volt}}
\newcommand{\DSkVetoPreAmpInputImpedance}{\SI{50}{\ohm}}
\newcommand{\DSkVetoPreAmpSNR}{\num{10}}
\newcommand{\DSkVetoVFEBDimensions}{\SI[product-units=power]{233 x 160}{\square\mm}}
\newcommand{\DSkVetoVFEBChannels}{\num{8}}
\newcommand{\DSkVetoPerCrateVFEBs}{\num{8}}
\newcommand{\DSkVetoHVDecouplerChannels}{\num{8}}
\newcommand{\DSkVetoPerCrateDecouplers}{\num{8}}
\newcommand{\DSkVetoPerCrateChannels}{\num{64}}
\newcommand{\DSkVetoCratesNumber}{\num{4}}
%--- DS-20k LSV
\newcommand{\DSkLSVDiameter}{\SI{8.0}{\meter}}
\newcommand{\DSkLSVTopFlangeDiameter}{\SI{1.0}{\meter}}
\newcommand{\DSkLSVBottomFlangeDiameter}{\SI{6.6}{\meter}}
\newcommand{\DSkLSVRapidFlangeDiameter}{\SI{1.0}{\meter}}
\newcommand{\DSkLSVPMTsNumber}{\num{130}}
\newcommand{\DSkLSVPMTCoverage}{\SI{13}{\percent}}
\newcommand{\DSkLSVWaterShield}{\SI{3.5}{\meter}}
\newcommand{\DSkLSVMinShielding}{\SI{1}{\meter}}
\newcommand{\DSkLSVExternalNeutronReduction}{\num{E6}}
\newcommand{\DSkLSVNeutronReductionFactor}{\num{100}}
\newcommand{\DSkLSVTMBFraction}{\SI{20}{\percent}}
\newcommand{\DSkLSVAccidentalCoincidence}{\SI{20}{\percent}}
\newcommand{\DSkLSVHighRate}{\SI{<4}{\kilo\becquerel}}
\newcommand{\DSkLSVLowRate}{\SI{<2}{\kilo\becquerel}}
\newcommand{\DSkLSVShortWindow}{\SI{50}{\micro\second}}
\newcommand{\DSkLSVLongWindow}{\SI{100}{\micro\second}}
\newcommand{\DSkLSVWCVOffset}{\SI{1}{\meter}}
\newcommand{\DSkScintillatorPCConcentration}{\SI{95}{\percent}}
\newcommand{\DSkScintillatorTMBConcentration}{\SI{5}{\percent}}
\newcommand{\DSkScintillatorPPOConcentration}{\SI{2}{\gram\per\liter}}
\newcommand{\DSkScintillatorPCInventory}{\SI{250}{\tonne}}
\newcommand{\DSkScintillatorTMBInventory}{\SI{13}{\tonne}}
\newcommand{\DSkScintillatorPPOInventory}{\SI{580}{\kg}}
\newcommand{\DSkScintillatorPurificationLossInventory}{\SI{10}{\percent}}
\newcommand{\DSkScintillatorContingencyMarginInventory}{\SI{5}{\percent}}
\newcommand{\DSkScintillatorPCProcurementIsotanks}{\numrange{8}{13}}
\newcommand{\BXScintillatorPPOConcentration}{\SI{1.5}{\gram\per\liter}}
\newcommand{\BXIsoTankVolume}{\SI{20}{\cubic\meter}}
\newcommand{\BXScintillatorPCProcurementIsotanksPerWeek}{\num{3}}
%--- DSk WCV
\newcommand{\DSkWCVPMTsNumber}{\num{100}}
\newcommand{\DSkWCVPMTCoverage}{\SI{2}{\percent}}
\newcommand{\DSkWCVDiameter}{\SI{15}{\meter}}
\newcommand{\DSkWCVTotalHeight}{\SI{14.65}{\meter}}
\newcommand{\DSkWCVBarrelHeight}{\SI{7.5}{\meter}}
\newcommand{\DSkWCVDomeRadius}{\SI{7.5}{\meter}}
\newcommand{\DSkWCVTopFlange}{\SI{4.5}{\meter}}
\newcommand{\DSkWCVManHoleSize}{\SI[product-units=power]{7.5 x 6.0}{\square\meter}}
\newcommand{\DSkWCVCleanRoomAccessSize}{\SI[product-units=power]{1 x 1}{\square\meter}}
\newcommand{\DSkWCVSteelSlabThickness}{\SI{8}{\centi\meter}}
%--- DSkSimulation
\newcommand{\DSkSimulationPrimaries}{\num{E6}}
\newcommand{\DSkSimulationEnergyRange}{\SIrange{1}{200}{\keVr}}
\newcommand{\DSkSimulationFLUKALivetime}{\SI{34}{\year}}
\newcommand{\DSkSimulationFLUKAMass}{\SI{3.3}{\tonne}}
\newcommand{\DSkSimulationFLUKAExposure}{\SI{112}{\tonne\year}}
\newcommand{\DSkSimulationFLUKACTFEventRate}{\SI{0.06}{\ev\per\second}}
\newcommand{\DSkSimulationFLUKAMuonlessEvents}{\SI{23}{\percent}}
\newcommand{\DSkSimulationFLUKALSVEventRate}{\SI{0.005}{\ev\per\second}}
\newcommand{\DSkSimulationFLUKATPCEventRate}{\SI{0.001}{\ev\per\second}}
\newcommand{\DSkSimulationFLUKAEventsNoCTF}{\num{7.9}}
\newcommand{\DSkSimulationFLUKATPCEventRateYear}{\SI{581}{\ev\per\year}}
\newcommand{\DSkSimulationFLUKATPCEventRateYearWithCTF}{\SI{0.3}{\ev\per\year}}
\newcommand{\DSkSimulationFLUKATPCEventRateYearWithLSV}{\SI{0.6}{\ev\per\year}}
\newcommand{\DSkSimulationGeantExposure}{\SI{1000}{\tonne\year}}
\newcommand{\DSkSimulationGeantTPCNeutronScatterProb}{\SI{>99.5}{\percent}}
\newcommand{\DSkSimulationGeantTPCNeutronOuterShellSize}{\SI{20}{\centi\meter}}
\newcommand{\DSkSimulationGeantLSVCollectionTime}{\SIrange{100}{200}{\nano\second}}
\newcommand{\DSkSimulationGeantLSVTailsTime}{\SIrange{300}{500}{\nano\second}}
\newcommand{\DSkSimulationGeantNeutronsPerChainDecayUTh}{\num{4E6}}
\newcommand{\DSkSimulationGeantLSVQuenchedEnergyCut}{\SI{<5}{\keV}}
\newcommand{\KMThreePMTSize}{\SI{10}{\inch}}
%--- Calibrations
\newcommand{\CalDDNeutronGeneratorModel}{\mbox{Thermoscientific~API-\num{120}}}
\newcommand{\CalDDNeutronGeneratorCommercialFlux}{\SI{>E7}{\mbox{~n}\per\second}}
\newcommand{\CalDDNeutronGeneratorFlux}{\SI{E4}{\neutron\per\second}}
\newcommand{\CalDDNeutronGeneratorTiming}{\SI{1}{\nano\second}}
\newcommand{\CalDDNeutronGeneratorAngleResolution}{\SI{40}{\milli\radian}}
\newcommand{\CalPyroGunEField}{\SI{E5}{\kilo\volt\per\centi\meter}}
\newcommand{\CalPyroGunTestCrystalSize}{\SI{2}{\centi\meter\cubed}}
\newcommand{\CalPyroGunPressure}{\SI{1}{\micro\bara}}
\newcommand{\CalPyroGunXRayEnergy}{\SI{100}{\keV}}
\newcommand{\CalPyroGunDiameter}{\SIrange{40}{50}{\milli\meter}}
\newcommand{\CalPyroGunLength}{\SIrange{50}{70}{\milli\meter}}
\newcommand{\CalPyroGunFlux}{\SI{160}{\mbox{~n}\per\second}}
\newcommand{\CalAmCSourcePbThickness}{\SI{2}{\milli\meter}}
\newcommand{\CalAmCSourceAlphaEnergyLimit}{\SI{4}{\MeV}}
\newcommand{\CalAmCSourceGammasEnergy}{\SI{4}{\MeV}}
\newcommand{\CalAmCSourceDSfActivity}{\SI{3.7}{\mega\becquerel}}
\newcommand{\CalAmCSourceDSkFlux}{\SI{10}{\neutron\per\second}}
\newcommand{\CalCfSourceNeutronsPerFission}{\num{3.756(1)}}
\newcommand{\CalCfSourceActivity}{\num{30}}
\newcommand{\CalCfSourceFissionFragmentEnergy}{\SI{190}{\MeV}}
\newcommand{\CalCfSourceAlphaMaxEnergy}{\SI{6.7}{\MeV}}
\newcommand{\CalCfSourceHeight}{\SI{20}{\milli\meter}}
\newcommand{\CalCfSourceDiameter}{\SI{20}{\milli\meter}}
\newcommand{\CalCfSourceFissionActivity}{\num{10}}
\newcommand{\CalCfSourceNeutronFlux}{\SI{37.6}{\mbox{~n}\per\second}}
\newcommand{\CalCfSourceAlphaActivity}{\num{316}}
\newcommand{\CalDSfKrSourceActivity}{\SI{8.5}{\kilo\becquerel}}
\newcommand{\CalLEDWaveLength}{\SI{265(5)}{\nano\meter}}
\newcommand{\CalLEDCurrent}{\SI{200}{\milli\ampere}}
\newcommand{\CalLEDLowEnergy}{\SI{100}{\keV}}
\newcommand{\CalLEDHighEnergy}{\SI{100}{\MeV}}
\newcommand{\CalAmBeSourceDiameter}{\SI{2}{\milli\meter}}
\newcommand{\CalAmBeSourceLength}{\SI{7}{\milli\meter}}
\newcommand{\CalAmBeSourceNeutronYield}{\num{50}}
\newcommand{\CalAmBeAmSourceAmActivity}{\SI{1.9}{\mega\becquerel}}
\newcommand{\CalGuideTubeDiameter}{\SI{3}{\centi\meter}}
\newcommand{\CalGuideTubeDiameterInches}{\SI{1.18}{\inch}}
\newcommand{\CalNeutronGunTubeDiameter}{\SI{15}{\centi\meter}}
\newcommand{\CalNeutronGunTubeLength}{\SI{8}{\meter}}
\newcommand{\CalNeutronGunHorizontalTubeDiameter}{\SI{5}{\centi\meter}}
\newcommand{\CalNeutronGunHorizontalTubeLength}{\SI{1.7}{\meter}}
\newcommand{\CalNeutronGunTubeColiimationAngle}{\SI{1.7}{\degree}}
\newcommand{\CalNeutronGunNeutronsToTPC}{\num{18}}
%--- Urania
\newcommand{\UraniaTotalDSkProduction}{\SI{60}{\tonne}}
\newcommand{\UraniaUArRate}{\SI{330}{\kg\per\day}}  % Andrew Changed Oct 2019
\newcommand{\UraniaExtractionTimeActual}{\SI{0.75}{\year}}
\newcommand{\UraniaGasFeedFraction}{\SI{15}{\percent}}
\newcommand{\UraniaOutputInputBalance}{$\pm$\SI{3}{\percent}}
\newcommand{\UraniaCOTwoFeedFraction}{$\sim$\SI{95}{\percent}}
\newcommand{\UraniaArFeedFraction}{\SI{430}{\ppm}}
\newcommand{\UraniaHeFeedFraction}{\SI{0.5}{\percent}}
\newcommand{\UraniaGasFeedAvePressure}{\SI{49(1)}{\bara}}
\newcommand{\UraniaGasFeedMaxPressure}{\SI{58}{\bara}}
\newcommand{\UraniaGasFeedMinPressure}{\SI{39}{\bara}}
\newcommand{\UraniaGasFeedAveTemperature}{\SI{79(2)}{\degreeF}}
\newcommand{\UraniaGasFeedMaxTemperature}{\SI{87}{\degreeF}}
\newcommand{\UraniaGasFeedMinTemperature}{\SI{63}{\degreeF}}
\newcommand{\UraniaGasFeedFlow}{\SI{20000}{\standard\cubic\meter\per\hour}}         % Update from Marino Oct/3rd/2019
\newcommand{\UraniaGasReturnPressure}{\SI{50}{\bara}}                                               % Update from Marino Oct/3rd/2019
\newcommand{\UraniaFirstUnitOutputFlow}{\SI{3300}{\standard\cubic\meter\per\hour}}  % Update from Marino Oct/3rd/2019
\newcommand{\UraniaFirstUnitFlowReduction}{\num{5}}                                                  % Update from Marino Oct/3rd/2019
%\newcommand{\UraniaGasFeedFlow}{\SI{16250}{\standard\cubic\meter\per\hour}}
%\newcommand{\UraniaGasReturnPressure}{\SI{120}{\bara}}
%\newcommand{\UraniaFirstUnitOutputFlow}{\SI{1300}{\standard\cubic\meter\per\hour}}  %Needs to be updated for larger production rate
%\newcommand{\UraniaFirstUnitFlowReduction}{\num{5}}  %Needs to be updated for larger production rate
\newcommand{\UraniaArGasReturnFraction}{\SI{99.9}{\percent}}
\newcommand{\UraniaFirstChillerTemperature}{\SI{5}{\celsius}}  %Needs to be updated for larger production rate
\newcommand{\UraniaSecondChillerTemperature}{\SI{-50}{\celsius}}  %Needs to be updated for larger production rate
\newcommand{\UraniaArFinalPurity}{\SI{99.9}{\percent}}
\newcommand{\UraniaHeProductionRate}{\SI{6.5E9}{\standard\liter\per\yr}}
\newcommand{\UraniaHeNationalReserveFractionEquivalentRate}{\SI{15}{\percent}}
\newcommand{\UraniaHeStartDate}{\mbox{July~2015}}
\newcommand{\UraniaUArShipmentMass}{\SI{11}{\tonne}}
\newcommand{\UraniaLNTwoShipmentMass}{\SI{4.8}{\tonne}}
\newcommand{\UraniaCortezMinTemperature}{\SI{-32}{\celsius}}
\newcommand{\UraniaCortezMaxTemperature}{\SI{40}{\celsius}}
\newcommand{\UraniaCortezAverageYearlySnowfall}{\SI{105}{\centi\meter}}
\newcommand{\UraniaCortezGroundSnowLoad}{\SI{40}{\psf}}
\newcommand{\UraniaCortezRoofLiveLoad}{\SI{40}{\psf}}
\newcommand{\UraniaCortezRoofSlopeFlatLoad}{\SI{28}{\psf}}
\newcommand{\UraniaCortezWindDesignLevel}{\num{90}}
\newcommand{\UraniaCortezSeismicDesignCategory}{{\bf B}}
\newcommand{\UraniaCortezWeatherDesignLevel}{Severe}
\newcommand{\UraniaCortezFrostLineDepth}{\SI{32}{\inch}}
\newcommand{\UraniaCortezTermiteInfestationLevel}{Moderate/Heavy}
\newcommand{\UraniaCortezWinterDesignTemp}{\SI{-14}{\celsius}}
\newcommand{\UraniaCortezIceBarrierUnderlayment}{Required}
\newcommand{\UraniaCortezFloodHazardLevels}{5-17-74}
\newcommand{\UraniaCortezAirFreezingIndex}{\num{1500}}
\newcommand{\UraniaCortezAverageAnnualTemp}{\SI{9}{\celsius}}
\newcommand{\UraniaOutputSampleFlowRate}{\SI{20}{\standard\liter\per\minute}}
\newcommand{\UraniaOutputSampleMaxTime}{\SI{12}{\hour}}
\newcommand{\UraniaHeightLimit}{\SI{16}{\meter}}
\newcommand{\UraniaFootprintWidthLimit}{\SI{16}{\meter}}
\newcommand{\UraniaFootprintLengthLimit}{\SI{19.2}{\meter}}
\newcommand{\UraniaCoolersMaxDistanceToPlant}{\SI{60}{\meter}}
\newcommand{\UraniaCoolersWidthLimit}{\SI{5}{\meter}}
\newcommand{\UraniaCoolersLengthLimit}{\SI{25}{\meter}}
\newcommand{\UraniaTransportVesselLength}{\SI{20}{\foot}}
\newcommand{\UraniaLNConsumption}{\SI{125}{\kilo\gram\per\hour}}  
\newcommand{\UraniaGNConsumption}{\SI{25}{\standard\cubic\meter\per\hour}}  
\newcommand{\UraniaAirConsumption}{\SI{125}{\standard\cubic\meter\per\hour}}  
\newcommand{\UraniaMaxPowerConsumption}{\SI{3.25}{\mega\watt}}
\newcommand{\UraniaTransportVesselReliefPressure}{\SI{22}{\bara}}
\newcommand{\UraniaPlantConstructionTimeBare}{\num{270}}
\newcommand{\UraniaPlantConstructionTime}{\SI{\UraniaPlantConstructionTimeBare}{\day}}
\newcommand{\UraniaPlantCommissionConsecutiveRunTime}{\SI{7}{\day}}
%--- Aria
\newcommand{\AriaChemicalPerPass}{\num{E3}}
\newcommand{\AriaChemicalRate}{O(\SI{1}{\tonne\per\day})}
\newcommand{\AriaArFinalPurity}{\SI{99.999}{\percent}}
\newcommand{\AriaDepletionPerPass}{\num{10}}
\newcommand{\AriaDepletionPerTwoPass}{\num{100}}
\newcommand{\AriaArgonRecoveryFactor}{\SI{85}{\percent}}
\newcommand{\AriaUArToGetDAr}{\SI{50}{\tonne}}
\newcommand{\AriaUArProducedRange}{\SIrange{32}{35}{\tonne}}
\newcommand{\AriaSeruciOneRate}{\SI{10}{\kg\per\day}}
\newcommand{\AriaSeruciTwoRate}{\SI{150}{\kg\per\day}}
\newcommand{\AriaSeruciZeroOperationPeriod}{\SIrange{6}{12}{\month}}
\newcommand{\AriaSeruciOneOperationPeriod}{\SI{3}{\year}}
\newcommand{\AriaSeruciHeight}{\SI{350}{\m}}
\newcommand{\AriaNuraxiHeight}{\SI{24}{\m}}
\newcommand{\AriaMonteSinniDiameter}{\SI{5}{\m}}
\newcommand{\AriaArVolatiityRatio}{\num{1.0015(1)}}
\newcommand{\AriaArVolatiityOrder}{\num{E-3}}
\newcommand{\AriaModulesNumber}{\num{30}}
\newcommand{\AriaCentralModulesNumber}{\num{28}}
\newcommand{\AriaCentralModulesHeight}{\SI{12}{\m}}
\newcommand{\AriaSeruciZeroHeight}{\SI{30}{\m}}
\newcommand{\AriaPlatformVerticalSpacing}{\SI{4}{\m}}
\newcommand{\AriaHeliumLeakCheckPolarisBackground}{\SI{1E-9}{\standard\cubic\cm\per\second}}
\newcommand{\AriaHeliumLeakCheckCERNBackground}{\SIrange{1E-8}{1E-9}{\standard\cubic\cm\per\second}}
\newcommand{\AriaArDistillationTemperatureRange}{\SIrange{84}{100}{\kelvin}}
\newcommand{\AriaDetectorSensitivity}{\SI{1}{\milli\becquerel\per\kg}}
\newcommand{\AriaDetectorActiveMass}{$\sim$\SI{1}{\kg}}
\newcommand{\AriaCOSMOActivationRate}{\SI{1.5E-8}{\becquerel\per\kilogram\per\day}}
\newcommand{\AriaACTIVIAActivationRate}{\SI{0.54E-8}{\becquerel\per\kilogram\per\day}}
%--- DART
\newcommand{\DArTinArDM}{\mbox{\DArT\ in \ArDM}}
\newcommand{\DArTVolume}{\SI{1}{\liter}}
\newcommand{\DArTMass}{\SI{1.4}{\kg}}
\newcommand{\DArTLeadBeltThickness}{\SI{10}{\cm}}
\newcommand{\DArTLeadBeltHeight}{\SI{140}{\cm}}
\newcommand{\DArTLeadBeltMass}{\SI{6}{\tonne}}
\newcommand{\DArTExternalBackgroundRate}{\SI{70}{\ev\per\day}}
\newcommand{\DArTMaterialBackgroundRate}{\SI{85}{\ev\per\day}}
\newcommand{\DArTUArDepletionWithLead}{\num{25200}}
\newcommand{\DArTUArPercentErrorWithLead}{\num{7}\%}
\newcommand{\DArTUArPercentErrorWithoutLeadWithDepletionTen}{\%}
\newcommand{\DArTUArPercentErrorWithoutLeadWithDepletionHundred}{\num{2}\%}
\newcommand{\DArTUArSensitivityUltimate}{\num{10000}}
%--- Argo
\newcommand{\ArgoExtractionPeriod}{\SI{6}{\year}}
\newcommand{\ArgoStartDate}{\num{2028}}
\newcommand{\ArgoTotalMass}{\SI{400}{\tonne}}
\newcommand{\ArgoFiducialMass}{\SI{300}{\tonne}}
\newcommand{\ArgoMassScale}{\SI{100}{\tonne}}
\newcommand{\ArgoExposure}{\SI{1000}{\tonne\year}}
\newcommand{\ArgoExtendedExposure}{\SI{3000}{\tonne\year}}
\newcommand{\ArgoNuFidExposure}{\SI{400}{\tonne\year}}
\newcommand{\ArgoSensitivityOneGeVBare}{2.7E-48}
\newcommand{\ArgoSensitivityOneGeVUnit}{\SI{\DSkSensitivityOneGeVBare}{\square\cm}}
\newcommand{\ArgoSensitivityTenGeVBare}{2.5E-47}
\newcommand{\ArgoSensitivityTenGeVUnit}{\SI{\DSkSensitivityTenGeVBare}{\square\cm}}
\newcommand{\ArgoArThreeNineAbatementMissing}{190}
\newcommand{\ArgoBeSevenSolarNeutrinosAccuracy}{\SI{2}{\percent}}
\newcommand{\ArgoPEPSolarNeutrinosAccuracy}{\SI{10}{\percent}}
\newcommand{\ArgoCNOSolarNeutrinosAccuracy}{\SI{15}{\percent}}
\newcommand{\ArgoImprovementOverCurrent}{\num{1000}}
\newcommand{\DSkImprovementOverDEAP}{\num{60}}
\newcommand{\ArgoImprovementOverDSk}{\num{15}}
\newcommand{\ArgoSolarNuExposure}{\SI{1500}{\tonne\year}}
\newcommand{\ArgoCNOHighZSolarNus}{\num{5000}}
\newcommand{\ArgoCNOLowZSolarNus}{\num{3500}}
\newcommand{\ArgoPEPSolarNus}{\num{6000}}
\newcommand{\ArgoSevenBeSolarNus}{\num{16000}}
\newcommand{\MetallicitySolarNuUncertainty}{\SI{38}{\percent}}
%--- SCENE
\newcommand{\SCENERecoilsEnergyMaxBare}{57.3}
\newcommand{\SCENERecoilsEnergyMax}{\SI{57.3}{\keVr}}
\newcommand{\SCENEDirectionalityThreshold}{\SI{57.3}{\keV}}
\newcommand{\SCENERecoilsLightEnergyRange}{\SIrange{10.3}{\SCENERecoilsEnergyMaxBare}{\keVr}}
\newcommand{\SCENERecoilsIonizationEnergyRange}{\SIrange{16.9}{\SCENERecoilsEnergyMaxBare}{\keVr}}
\newcommand{\SCENENRQuenchingRatio}{\SI{<25}{\percent}}
\newcommand{\SCENENRQuenchingRatioRange}{\SIrange{0}{1000}{\volt\per\cm}}
\newcommand{\SCENEERQuenchingRatio}{\SI{50}{\percent}}
\newcommand{\SCENEERQuenchingRatioField}{\SI{100}{\volt\per\cm}}
%--- ARIS
\newcommand{\ARISRecoilsEnergyMaxBare}{119.4}
\newcommand{\ARISRecoilsLightEnergyRange}{\SIrange{7.9}{\ARISRecoilsEnergyMaxBare}{\keVr}}
%--- DarkSide-10
\newcommand{\DStExposure}{\SI{502}{day}}													%DocDb#562
%--- AAr
\newcommand{\DSfAArArThreeNineActivity}{\SI{1}{\becquerel\per\kg}}
\newcommand{\DSfAArRunTime}{\CriterionSRAArLiveTime}
\newcommand{\DSfAArAfterQualityCutsLiveTime}{\totalliv}
\newcommand{\DSfAArNullFieldLightYield}{\SI{8.1(2)}{\pe\per\keV}}							%Statistical error only; DocDB 1358
\newcommand{\DSfAArDriftFieldLightYield}{\SI{7.0(3)}{\pe\per\keV}}							%New sys err, PDM email 10/1/2014
\newcommand{\DSfAArDriftFieldLightYieldfeb}{\SI{6.99(2)}{\pe\per\keV}}
\newcommand{\DSfAArLightYieldStability}{\SI{0.7}{\percent}}
\newcommand{\DSfAArDiscriminatorEfficiency}{\num{0.887}}
\newcommand{\DSfAArTriggerRate}{\SI{50}{\Hz}}												%PDM: changed from 0.60
\newcommand{\DSfAArGTwoTriggerRate}{\SI{13}{\hertz}}
\newcommand{\DSfAArGTwoTriggerReduction}{\num{4}}
\newcommand{\DSfAArExposure}{\DSfAArDFExposure}
\newcommand{\DSfAArDFExposure}{\SI{1422(67)}{\kg\day}}
\newcommand{\DSfAArSRExposure}{\SI{605(33)}{\kg\day}}
\newcommand{\DSfAArFNExposure}{\SI{236(13)}{\kg\day}}
\newcommand{\DSfAArLimitHundredGev}{\SI{6.1E-44}{\square\cm}}
\newcommand{\DSfAArLimitOneTeV}{\SI{2.3E-43}{\square\cm}}
\newcommand{\DSfAArLimitTenTeV}{\SI{2.2E-42}{\square\cm}}
\newcommand{\DSfAArNeutronsRadiogenicObserved}{\num{3}}
\newcommand{\DSfAArNeutronsCosmogenicObserved}{\num{1}}
\newcommand{\DSfAArNeutronsAllObserved}{\num{4}}
\newcommand{\DSfAArNeutronsRadiogenicExpected}{$\sim$\SI{1.3}{\ev}}							%DocDb#1011 v2
\newcommand{\DSfAArNeutronsBackground}{\SI{0.2}{\ev}}
\newcommand{\DSfAArROIEventsNumber}{\num{1.5E7}}   											%2014 DS-50 Physics paper
%--- UAr
\newcommand{\DSfUArExposure}{\SI{2616(43)}{\kg\day}}
\newcommand{\DSfUArPhysicsCutsEfficiency}{\SI{>70}{\percent}}
\newcommand{\DSfUArFillDate}{\mbox{April 1, 2015}}											%DocDB#2592
\newcommand{\DSfUArAfterQualityCutsLiveTime}{\SI{70.9}{\liveday}}
\newcommand{\DSfUArTriggerRate}{\SI{1}{\Hz}}
\newcommand{\DSfUArLimitHundredGev}{\SI{2.0E-44}{\square\cm}}
\newcommand{\DSfUArLimitOneTeV}{\SI{8.6E-44}{\square\cm}}
\newcommand{\DSfUArLimitTenTeV}{\SI{8.0E-43}{\square\cm}}					
\newcommand{\DSfUArROIPERange}{\SIrange{20}{460}{\pe}}
\newcommand{\DSfUArROIEnergyRange}{\SIrange{13}{201}{\keVr}}
\newcommand{\DSfUArROIEventsNumber}{\num{1.26E5}}
\newcommand{\DSfUArFiducialDiameter}{\SI{200}{\mm}}
\newcommand{\DSfUArFiducialHeight}{\SI{90}{\mm}}
\newcommand{\DSfUArFiducialFraction}{$\sim$\SI{10}{\percent}}
\newcommand{\DSfUArFiducialMass}{\SI{4}{\kg}}
\newcommand{\DSfAAronUArinterval}{\SIrange{1000}{2500}{\pe}}
\newcommand{\DSfUArDepletion}{1400}
\newcommand{\DSfUArDepletionWithUncertainty}{$1400\pm 200$}
\newcommand{\DSfAAronUArratio}{\num{\DSfUArDepletion(200)}}
\newcommand{\DSfAAronUArratioNoUncertainty}{\num{\DSfUArDepletion}}
\newcommand{\DSfUArArThreeNineActivity}{\SI{0.73(11)}{\milli\becquerel\per\kg}}				%DocDB#1366  % Update from P. Agnes email 2015-09-17
\newcommand{\DSfUArGTwoTriggerReduction}{\num{2}}
\newcommand{\DSfUArActivityLessThan}{\SI{3}{\milli\becquerel\per\kg}}	
\newcommand{\DSfUArBackgroundFreeExtrapolatedExposure}{\SI{5.5}{\tonne\yr}}
\newcommand{\DSfUArArThreeNineDepletion}{\num{1.4(2)E3}}
\newcommand{\DSfUArAArRunTimeEquivalent}{\SI{23}{\year}}
\newcommand{\DSfUArKrEightFiveActivity}{\SI{2.05(13)}{\milli\becquerel\per\kg}}				%DocDB#1366 % Update from P. Agnes email 2015-09-17
\newcommand{\DSfUArKrEightFiveMRateFromFit}{\SI{35.3(22)}{\ev\per\day}}						%DocDB#1366 Corrected by Davide
\newcommand{\DSfUArKrEightFiveMRateFromCoincidences}{\SI{33.1(9)}{\ev\per\day}}				%DocDB#1314, updated for full UAr statistics
\newcommand{\DSfUArRbEightFiveMCoincidenceWindow}{\SIrange{0.1}{2.2}{\micro\s}}
\newcommand{\DSfUArRbEightFiveMMeasuredMeanLife}{\SI{1.64(12)}{\micro\s}}
\newcommand{\DSfUArRbEightFiveMMeanLife}{\SI{1.46}{\micro\s}}
\newcommand{\DSfUArNeutronsRadiogenicObserved}{\num{1}}
\newcommand{\DSfUArNeutronsCosmogenicObserved}{\num{0}}
\newcommand{\DSfUArMassDelivered}{\SI{156(1)}{\kg}}
\newcommand{\DSfUArMassApprox}{\SI{150}{\kg}}
\newcommand{\DSfUArExtractionRate}{\SI{0.3}{\kg\per\day}}
\newcommand{\DSfUArPurificationRate}{\SI{20}{\kg\per\day}}
\newcommand{\DSfUArConcentrationWell}{\SI{400}{\ppm}}
\newcommand{\DSfUArConcentrationCrude}{\SI{5}{\percent}}
\newcommand{\DSfUArConcentrationDistillate}{\SI{99.999}{\percent}}
\newcommand{\DSfUArImpuritiesDistillate}{\SI{<10}{\ppm}}
\newcommand{\DSfUArSTwoLossToElectroNegativeMax}{\SI{<7}{\percent}}
\newcommand{\DSfUArSOneRadialVariabilityMax}{\SI{<3}{\percent}}
\newcommand{\DSfComptonPeakPE}{$\sim$\SI{600}{\pe}}
\newcommand{\DSfPulserTriggerRate}{\SI{0.05}{\Hz}}
%--- Materials and Assay Krakow
\newcommand{\MatAssayKrakowXIASampleSurface}{\SI[product-units=power]{43 x 43}{\square\cm}}
\newcommand{\MatAssayKrakowXIASampleThickness}{\SI{3}{\mm}}
\newcommand{\MatAssayKrakowXIABackground}{\SI{45(4)}{\ct\per\day\square\meter}}
\newcommand{\MatAssayKrakowXIASampleRate}{\SI{22}{\smp\per\year}}
\newcommand{\MatAssayKrakowXIAThreshold}{\SI{1.5}{\MeV}}
\newcommand{\MatAssayKrakowXIASurfaceSensitivity}{\SI{1}{\milli\becquerel\per\square\meter}}
\newcommand{\MatAssayKrakowXIABulkSensitivity}{\SI{100}{\milli\becquerel\per\kg}}
%\newcommand{\MatAssayKrakowXIAbulkPbsensitivity}{\SI{50}{\milli\becquerel\per\kg}}
\newcommand{\MatAssayKrakowXIACapacityReservedForDSk}{\SI{60}{\percent}}
\newcommand{\MatAssayKrakowPoReductionFromTiEtching}{\num{\sim2}}
\newcommand{\MatAssayKrakowEtchingAlphaEenrgyLowerLimit}{\SI{6}{\MeV}}
\newcommand{\MatAssayKrakowPoReductionfromCuSSElectroPolishing}{\num{\sim25}}
\newcommand{\MatAssayKrakowRnChamberTemperaturePrecision}{\SI{\pm1}{\kelvin}}
\newcommand{\MatAssayKrakowRnChamberTemperatureHigh}{\SI{373}{\kelvin}}
\newcommand{\MatAssayKrakowRnChamberTemperatureMax}{\SI{423}{\kelvin}}
\newcommand{\MatAssayKrakowRnChamberOneVolume}{\SI{12}{\liter}}
\newcommand{\MatAssayKrakowRnChamberTwoVolume}{\SI{50}{\liter}}
\newcommand{\MatAssayKrakowRnChamberThreeVolume}{\SI{250}{\liter}}
%--- Materials and Assay Temple
\newcommand{\MatAssayTempleAxisLength}{\SI{70}{\cm}}
\newcommand{\MatAssayTempleResolution}{\SI{2.5}{\keV}}
\newcommand{\MatAssayTempleEnergy}{\SI{1334}{\keV}}
\newcommand{\MatAssayTempleTempSensorU}{\SI{4000}{\ppb}}
\newcommand{\MatAssayTempleTempSensorTh}{\SI{2200}{\ppb}}
\newcommand{\MatAssayTempleAluminaU}{\SI{350}{\ppb}}
\newcommand{\MatAssayTempleEndCap}{\SI{13}{\milli\becquerel\per\kg}}
\newcommand{\MatAssayTempleFET}{\SI{600}{\ppb}}
\newcommand{\MatAssayTempleLeadThickness}{\SI{20}{\cm}}
\newcommand{\MatAssayTempleCuThickness}{\SI{5}{\cm}}
\newcommand{\MatAssayTempleCavityVolume}{\SI{30}{\cubic\cm}}
\newcommand{\MatAssayTempleYear}{\num{2012}}
\newcommand{\MatAssayTempleEff}{\SI{100}{\percent}}
%--- Materials and Assay BiPo
\newcommand{\MatAssayBiPoScreeningYearTwo}{\num{2017}}
\newcommand{\MatAssayBiPoScreeningPercentage}{\SI{70}{\percent}}
\newcommand{\MatAssayBiPoSensitivityCL}{\SI{90}{\percent}}
\newcommand{\MatAssayBiPoPMTsize}{\SI{5}{\inch}}
\newcommand{\MatAssayBiPoSurfaceArea}{\SI{3.6}{\square\m}}
\newcommand{\MatAssayBiPoBackground}{\SI{1.0(3)}{\micro\becquerel\per\square\m}}
\newcommand{\MatAssayBiPoTlSensitivity}{\SI{2}{\micro\becquerel\per\kg}}
\newcommand{\MatAssayBiPoBiSensitivity}{\SI{140}{\micro\becquerel\per\kg}}
\newcommand{\MatAssayBiPoStartYear}{\num{2013}}
\newcommand{\MatAssayBiPoSDSkcreeningStartYear}{\num{2016}}
%--- Materials and Assay PNNL
\newcommand{\MatAssayPNNLChamberOneVolume}{\SI{0.3}{\liter}}
\newcommand{\MatAssayPNNLChamberTwoVolume}{\SI{35}{\liter}}
%--- Materials and Assay SiPM
\newcommand{\MatAssaySiPMLNGSUTh}{\si{\ppb}}
\newcommand{\MatAssaySiPMBHSUU}{\SI{<19}{\ppt}}
\newcommand{\MatAssaySiPMBHSUTh}{\SI{<35}{\ppt}}
\newcommand{\MatAssaySiPMPNNLU}{\SI{<2}{\ppt}}
\newcommand{\MatAssaySiPMPNNLTh}{\SI{<0.8}{\ppt}}
%--- Materials and Assay SiPM
\newcommand{\MatAssayTiMSUU}{\SI{<3}{\ppt}}
\newcommand{\MatAssayTiMSUTh}{\SI{<50}{\ppt}}
\newcommand{\MatAssayTiPNNLK}{\SI{<1}{\milli\becquerel\per\kg}}
\newcommand{\MatAssayTiPNNLTh}{\SI{13}{\ppt}}
%--- General
\newcommand{\MatAssayThActivityPptEquiv}{\SI{4.1}{\micro\becquerel\per\kg}}
\newcommand{\MatAssayUActivityPptEquiv}{\SI{12.4}{\micro\becquerel\per\kg}}
\newcommand{\MatAssayCopperSurfaceActivitiyLimit}{\SI{3}{\milli\becquerel\per\square\m}}
\newcommand{\MatAssayPlasmaTemperature}{\SI{8000}{\kelvin}}
\newcommand{\MatAssayICPMSChargeState}{\num{+1}}
%--- DS-50 Global Run
\newcommand{\DSfGlobalNeutronsRadiogenicObserved}{\num{1}}								%2015-10-02 AFan: updated per email discussions
\newcommand{\DSfGlobalNeutronsRadiogenicExpected}{\SI{2(2)}{\ev}}						%DocDb#1011 v2      2015-10-02 AFan: updated per email discussions
\newcommand{\DSfGlobalNeutronsRadiogenicExpectedPassVetoCuts}{\num{<0.02}}	
\newcommand{\DSfGlobalLiveTime}{\SI{118}{\liveday}}                                 	%47.1 + 70.9 days
%--- DS-50
\newcommand{\DSfTotalMass}{\SI{153(1)}{\kg}}											%To be checked with Hanguo
\newcommand{\DSfActiveMass}{\SI{46.4(7)}{\kg}}
\newcommand{\DSfNominalActiveMass}{\SI{50}{\kg}}
\newcommand{\DSfActiveDiameter}{\SI{356}{\mm}}
\newcommand{\DSfActiveHeight}{\SI{363}{\mm}}
\newcommand{\DSfFiducialMass}{\SI{36.9(6)}{\kg}}
\newcommand{\DSfSpectraFitMass}{\SI{\sim34}{\kg}}
\newcommand{\DSfPlannedRunTime}{\SI{3}{\year}}
\newcommand{\DSfDMSArThreeNineBackgroundCondition}{\SI{0.01}{\ev\per\bin}}
\newcommand{\DSfDMSFNineNineZeroUpperLimit}{\SI{90}{\percent}}
\newcommand{\DSfDMSFNineNineNineUpperLimit}{\SI{99}{\percent}}
\newcommand{\DSfRnTwoTwoTwoSpecificActivityLimit}{\SI{2}{\micro\becquerel\per\kg}}
\newcommand{\DSfRnTwoTwoTwoActivityLimit}{\SI{40}{\milli\becquerel}}
\newcommand{\DSfKrEightFiveExtractionEfficiency}{$\sim$\SI{66}{\percent}}
\newcommand{\DSfSTwoOverSOne}{\num{40}}
\newcommand{\DSfSTwoOverSThree}{$\sim$\num{1000}}										%Alden Fan plot
\newcommand{\DSfSTwoSlowComponentMeanLife}{$\sim$\SI{3.4}{\us}}
\newcommand{\DSfSTwoIntegrationWindow}{\SI{30}{\us}}
\newcommand{\DSfPMTRadiogenicNeutronRate}{\SI{7}{\ev\per\pm\year}}
\newcommand{\DSfDetectorRadiogenicNeutronRate}{\SI{1}{\ev\per\week}}
\newcommand{\DSfHighMassThreshold}{\SI{20}{\GeV\per\square\c}}
\newcommand{\DSfLowMassThreshold}{\SI{8}{\GeV\per\square\c}}
\newcommand{\DSfLowMassBestRecordRange}{\SIrange{1.8}{6.0}{\GeV\per\square\c}}
\newcommand{\DSfLowMassElectronBestRecordRange}{\SIrange{30}{50}{\MeV\per\square\c}}
\newcommand{\DSfLowMassBackgroundRate}{\SI{1.5}{event\per\keVee\per\kg\per\day}}
\newcommand{\DSfLowMassThresholdEe}{\SI{100}{\eVee}}
\newcommand{\DSfLowMassThresholdNr}{\SI{600}{\eVr}}
\newcommand{\DSfLowMassThresholdE}{\SI{4}{\el}}
\newcommand{\DSfLowMassThresholdPE}{\SI{23}{\pe}}
\newcommand{\DSfLowMassKnownBckThresholdE}{\SI{7}{\el}}
\newcommand{\DSfPMTsNumber}{\num{38}}
\newcommand{\DSfPMTsNumberTop}{\num{19}}
\newcommand{\DSfPMTsNumberBottom}{\num{19}}
\newcommand{\DSfPMTsAliveNumber}{\DSfPMTsNumber}
\newcommand{\DSfPMTsNumberText}{thirty-eight}
\newcommand{\DSfPMT}{{Hamamatsu R11065}}
\newcommand{\DSfPMTSize}{\SI{3}{\inch}}
\newcommand{\DSfPMTQE}{\SI{34}{\percent}}												%PDM: average for actual PMTs in DS-50, see also DocDb#42
\newcommand{\DSfPMTCE}{\SI{92}{\percent}}
\newcommand{\DSfPMTWaveLength}{\SI{420}{\nano\meter}}
\newcommand{\DSfPMTGainEqualization}{\SI{10}{\percent}}
\newcommand{\DSfPMTBiasMax}{\SI{-1050}{\volt}}
\newcommand{\DSfPMTBiasMin}{\SI{-1288}{\volt}}
\newcommand{\DSfPMTGain}{\num{4.E5}}
\newcommand{\DSfDriftTimeMax}{\SI{376}{\us}}											% Value for UAr analysis See docdb 1255. Compare to old AAr value of 373.3. Change is due to change of power supply.  
\newcommand{\DSfElectronMeanLife}{\SI{\ge5}{ms}}
\newcommand{\DSfUArChemicalPurity}{\SI{0.01}{\ppb}}
\newcommand{\DSfElectronExtractionEfficiency}{\SI{>99.9}{\percent}}
\newcommand{\DSfDriftField}{\SI{200}{\volt\per\centi\meter}}
\newcommand{\DSfExtractionField}{\SI{2.8}{\kilo\volt\per\centi\meter}}
\newcommand{\DSfMultiplicationField}{\SI{4.2}{\kilo\volt\per\centi\meter}}
\newcommand{\DSfCathodePotential}{\SI{-12.7}{\kilo\volt}}
\newcommand{\DSfGridPotential}{\SI{-5.6}{\kilo\volt}}
\newcommand{\DSfAnodePotential}{\SI{0}{\kilo\volt}}
\newcommand{\DSfLArTotalHeight}{\SI{353.5}{\mm}}
\newcommand{\DSfGArHeight}{\SI{1}{\centi\meter}}
\newcommand{\DSfLArAboveMeshHeight}{\SI{4.7}{\mm}}
\newcommand{\DSfLArBelowMeshHeight}{\SI{348.8}{\mm}}
\newcommand{\DSfLArElectronSpeedStability}{\SI{0.04}{\percent}}
\newcommand{\DSfLArAboveMeshElectronSpeed}{\SI{3.510}{\mm\per\us}}
\newcommand{\DSfLArBelowMeshElectronSpeed}{\SI{0.93(1)}{\mm\per\us}}					%Guangyong Koh
\newcommand{\DSfTriggerDiscriminatorThreshold}{\SI{0.6}{\pe}}							%PDM: changed from 0.60
\newcommand{\DSfTriggerPMTsNumberThreshold}{\num{2}}
\newcommand{\DSfTriggerWindow}{\SI{100}{\nano\second}}
\newcommand{\DSfTriggerEfficiency}{\SI{100}{\percent}}
\newcommand{\DSfTriggerEfficiencyThreshold}{\SI{60}{\pe}}
\newcommand{\DSfTriggerSTwoEfficiency}{\SI{100}{\percent}}
\newcommand{\DSfTriggerSTwoEfficiencyThreshold}{\SI{30}{\pe}}
\newcommand{\DSfTriggerSTwoAnalysisThreshold}{\SI{100}{\eVr}}
\newcommand{\DSfTriggerAcquisitionPreWindow}{\SI{5}{\us}}
\newcommand{\DSfTriggerAcquisitionPostWindow}{\SI{40}{\us}}
\newcommand{\DSfTriggerAcquisitionTotalWindow}{\SI{440}{\us}}
\newcommand{\DSfTriggerInhibitWindow}{\SI{810}{\us}}
\newcommand{\DSfTriggerGOneGate}{\SI{10}{\us}}
\newcommand{\DSfTriggerGTwoGate}{\SI{13}{\us}}
\newcommand{\DSfPulseFindingEfficiency}{\SI{100}{\percent}}
\newcommand{\DSfPulseFindingEfficiencyThreshold}{\SI{30}{\pe}}
\newcommand{\DSfColdAmplifierGain}{\SI{3}{\volt/\volt}}
\newcommand{\DSfColdAmplifierBandWidth}{\SI{150}{\mega\hertz}}
\newcommand{\DSfColdAmplifierRiseAndFallTime}{\SI{2.4}{\nano\second}}
\newcommand{\DSfColdAmplifierLowFrequencyTimeConstant}{\SI{5.8}{\milli\second}}
\newcommand{\DSfColdAmplifierOutputRange}{\SI{3}{\volt}}
\newcommand{\DSfColdAmplifierTermination}{\SI{50}{\ohm}}                               	%George Korga
\newcommand{\DSfColdAmplifierNoise}{\SI{45}{\micro\volt}}
\newcommand{\DSfFrontEndGain}{\num{10}}
\newcommand{\DSfADCBitNumber}{\SI{12}{\bit}}
\newcommand{\DSfADCSamplingRate}{\SI{250}{\MHz}}
\newcommand{\DSfLaserWaveLength}{\SI{405}{nm}}											%Giuliana Fiorillo, Hamamatsu PLP10-040
\newcommand{\DSfLaserPMTOccupancy}{\SI{0.1}{\pe}}
\newcommand{\DSfLaserPulseWidth}{\SI{60}{\ps}}											%Giuliana Fiorillo, Hamamatsu PLP10-040
\newcommand{\DSfLaserPulseRate}{\SI{500}{\hertz}}
\newcommand{\DSfLaserAcquisitionWindow}{\SI{3}{\us}}
\newcommand{\DSfLaserIntegrationWindow}{\SI{108}{\nano\second}}
\newcommand{\DSfLaserSPEMeanStability}{\SI{2.5}{\percent}}
\newcommand{\DSfLaserSPESystematic}{$<$\SI{2.5}{\percent}}
\newcommand{\DSfCryogenicsExchangerCoolingPower}{\SI{300}{\watt}}
\newcommand{\DSfCryogenicsExchangerLINPower}{\SI{125}{\kg\per\day}}
\newcommand{\DSfCryogenicsGasFlowNormal}{\SI{30}{\standard\liter\per\minute}}
\newcommand{\DSfCryogenicsGasFlowLINBoost}{\SI{50}{\standard\liter\per\minute}}
\newcommand{\DSfCryogenicsCryostatPowerLeak}{\SI{25}{\watt}}
\newcommand{\DSfCryogenicsPMTsHeatLoad}{\SI{3}{\watt}}
\newcommand{\DSfCrogenicsHeaterPower}{\SI{40}{\watt}}
\newcommand{\DSfCryogenicsEmergencyCoolingDuration}{\SI{10}{\day}}
\newcommand{\DSfCryogenicsUllagePressure}{\SI{1080.0(1)}{\milli\bar}}
\newcommand{\DSfCryogenicsUllagePressureStability}{\SI{\pm0.1}{\milli\bar}}
\newcommand{\DSfCryogenicsPressureStability}{\SI{0.023}{\psi}}
\newcommand{\DSfCryogenicsRnTrapTemperature}{\SIrange[range-units=single]{185}{190}{\kelvin}}		%Yury Suvorov e-mail with graph 9/10/2014
\newcommand{\DSfCryogenicsInCryostatTemperature}{\SI{87.95(2)}{\kelvin}}
\newcommand{\DSfITOThickness}{\SI{15}{\nano\meter}}
\newcommand{\DSfITOTopWindowBottomBias}{\SI{-1183}{\volt}}
\newcommand{\DSfITOTopWindowTopBias}{\SI{-1157}{\volt}}
\newcommand{\DSfPTFEReflectorThickness}{\SI{2.54}{\centi\meter}}
\newcommand{\DSfTPBCenterThickness}{\SI{230(10)}{\micro\gram\per\square\centi\meter}}	%Evap elog# 96-100
\newcommand{\DSfTPBEdgeThickness}{\SI{190(15)}{\micro\gram\per\square\centi\meter}}		%Guangyong Koh (PDM changed from +20-10)
\newcommand{\DSfTPBPTFEReflectorCenterThickness}{\SI{165(20)}{\micro\gram\per\square\centi\meter}}  %Jason Brodsky
\newcommand{\DSfTPBPTFEReflectorEndThickness}{\SI{224(27)}{\micro\gram\per\square\centi\meter}} 	%Jason Brodsky
\newcommand{\DSfGridFoilThickness}{\SI{50}{\micro\meter}}
\newcommand{\DSfGridFoilTrasparency}{\SI{95}{\percent}}
\newcommand{\DSfCryostatExternalDiameter}{\SI{32}{\cm}}
\newcommand{\DSfCALISTransversePositioningRange}{\SIrange{0}{60}{\cm}}
\newcommand{\DSfCALISArmLength}{\SI{62}{\cm}}
\newcommand{\DSfCALISArmArticulationRange}{\SIrange{0}{90}{\degree}}
\newcommand{\DSfCALISOrganPipeAxisDistanceToCenter}{\SI{80}{\cm}}
\newcommand{\DSfCALISGateValvesNumber}{\num{4}}
\newcommand{\DSfCALISGateValveDiameter}{\SI{15}{\cm}}
\newcommand{\DSfCALISGateValveDistanceToLSV}{\SI{6}{\m}}
\newcommand{\DSfSpatialZResolution}{\chk{\SI{888}{\mm}}}
\newcommand{\DSfSpatialXYResolution}{\chk{\SI{888}{\mm}}}
\newcommand{\DSfDataTotalRate}{\SI{9E5}{\ev\per\day}}
\newcommand{\DSfDataLaserRate}{\SI{8E5}{\ev\per\day}}
\newcommand{\DSfDataLaserSize}{\SI{0.1}{\mega\byte}}
\newcommand{\DSfDataDMSRate}{\SI{1E5}{\ev\per\day}}
\newcommand{\DSfDataDMSSize}{\SI{2.6}{\mega\byte}}
\newcommand{\DSfDataStorageLNGSShortDisk}{\SI{7}{\tera\byte}}
\newcommand{\DSfDataStorageLNGSLongDisk}{\SI{710}{\tera\byte}}
\newcommand{\DSfDataStorageCNAFDisk}{\SI{1}{\peta	\byte}}
\newcommand{\DSfDataStorageCNAFTape}{\SI{300}{\tera\byte}}
\newcommand{\DSfDataStorageFNALDisk}{\SI{50}{\tera\byte}}
\newcommand{\DSfDataStorageFNALTape}{\SI{620}{\tera\byte}}
\newcommand{\DSfCPUsLNGS}{\mbox{400~cores}}
\newcommand{\DSfCPUsCNAF}{\mbox{400~job~queues}}
\newcommand{\DSfCPUsFNAL}{\mbox{25~guaranteed~batch~slots}}
\newcommand{\DSfCPUsFNALUpgrade}{\mbox{60~guaranteed~batch~slots}}
\newcommand{\OSGCPUEquivalent}{\mbox{6000~CPU}}
%--- LSV High Background TMB
\newcommand{\LSVOldTMBConcentration}{\SI{50}{\percent}}									%Augusto Goretti email to PDM 12/23/14
\newcommand{\LSVOldPPOConcentration}{\SI{2.5}{\gram\per\liter}}							%Augusto Goretti email to PDM 12/23/14
\newcommand{\LSVOldPhY}{\SI{12}{photons\per\keV}}
\newcommand{\LSVOldLY}{\SI{0.54(4)}{\pe\per\keV}}										%Maria Elena Monzani email, 10/1/2014
\newcommand{\LSVOldNeutronsRadiogenicRejectionEfficiencyMeasured}{\SI{97}{\percent}}
\newcommand{\LSVOldNeutronCaptureMeanLife}{\SI{2.2}{\us}}
\newcommand{\LSVOldCFourteenFitRange}{\SIrange[range-units=single]{30}{110}{\pe}}
\newcommand{\LSVOldCFourteenRate}{$\sim$\SI{150}{\kilo\becquerel}}						%DocDb#885, #738
\newcommand{\LSVOldAlphaQuenchedEnergy}{\SIrange[range-units=single]{50}{60}{\keV}}
\newcommand{\LSVOldBTenCaptureFraction}{$\sim$\SI{99.2}{\percent}}
%--- LSV Low Background TMB
\newcommand{\LSVNewTMBConcentration}{\SI{5}{\percent}}
\newcommand{\LSVNewPPOConcentration}{\SI{1.4}{\gram\per\liter}}							
\newcommand{\LSVNewPhY}{\SI{12}{photons\per\keV}}
\newcommand{\LSVNewLY}{\SI{0.53(3)}{\pe\per\keV}}
\newcommand{\LSVNewNeutronsRadiogenicRejectionEfficiencyMeasured}{\SI{>99.5}{\percent}}
\newcommand{\LSVNewNeutronsRadiogenicRejectionAcceptanceLoss}{\SI{<16}{\percent}}
\newcommand{\LSVNewNeutronCaptureMeanLife}{\SI{22}{\micro\s}}
\newcommand{\LSVNeutronThermalizationTimeScale}{\SI{< 100}{\nano\second}}
\newcommand{\LSVBackgroundRatioOldOverNew}{\SI{1}{\percent}}
\newcommand{\LSVNewCOneFourRate}{$\sim$\SI{0.3}{\kilo\becquerel}}
\newcommand{\LSVNewBTenCaptureGroundPE}{\SI{30}{\pe}}
\newcommand{\LSVNewBTenCaptureExcitedPE}{\SI{240}{\pe}}
\newcommand{\LSVNewBTenCaptureFraction}{$\sim$\SI{92}{\percent}}
\newcommand{\LSVNewHOneCaptureFraction}{$\sim$\SI{8}{\percent}}
\newcommand{\LSVNewNeutronsRadiogenicRejectionEfficiencySoleCapture}{\SI{>99.1}{\percent}}
\newcommand{\LSVNewRecordLengthShort}{\SI{140}{\micro\s}}
\newcommand{\LSVNewRecordLengthLong}{\SI{200}{\micro\s}}
\newcommand{\LSVShortRecordLengthLiveTime}{\SI{36.7}{\day}}
\newcommand{\LSVLongRecordLengthLiveTime}{\SI{34.9}{\day}}
\newcommand{\LSVNewRecordLengthStart}{\SI{-6.5}{\micro\s}}
\newcommand{\LSVNewRecordLengthEndShort}{\SI{133.5}{\micro\s}}
\newcommand{\LSVNewRecordLengthEndLong}{\SI{193.5}{\micro\s}}
%--- LSV
\newcommand{\LSVScintillatorMass}{\SI{30}{\tonne}}
\newcommand{\LSVStainlessSphereDiameter}{\SI{4.0}{\m}}
\newcommand{\LSVStainlessSteelTopFlangeDiameter}{\SI{2.0}{\m}}
\newcommand{\LSVStainlessSteelReducedFlangeDiameter}{\SI{91}{\cm}}
\newcommand{\LSVPMTsNumber}{\num{110}}
\newcommand{\LSVPMTsAliveNumber}{\num{106}}
\newcommand{\LSVPMTModel}{\mbox{Hamamatsu R5912 LRI}}
\newcommand{\LSVPMTSize}{\SI{8}{\inch}}
\newcommand{\LSVPMTQE}{\SI{37}{\percent}}
\newcommand{\LSVPMTModelwave}{\SI{408}{\nano\meter}}
\newcommand{\LSVPMTCE}{\SI{92}{\percent}}
\newcommand{\LSVProtonsQuenchingFactor}{\num{10}}
\newcommand{\LSVPMTsBiasRange}{\SI{+1500}{1800}{\volt}}
\newcommand{\LSVNeutronsRadiogenicRejectionEfficiencyDesign}{\SI{99.5}{\percent}}
\newcommand{\LSVNeutronsCosmogenicRejectionEfficiencyDesign}{\SI{95}{\percent}}
\newcommand{\LSVOrganPipesDiameter}{\SI{15}{\cm}}
%--- CTF
\newcommand{\CTFHeight}{\SI{10}{\meter}}
\newcommand{\CTFDiameter}{\SI{11}{\meter}}
\newcommand{\CTFWaterMass}{\SI{1}{\kilo\tonne}}
\newcommand{\CTFTopPortSize}{\SI[product-units=power]{3.2 x 3.2}{\square\m}}
\newcommand{\CTFTopFlangeDiameter}{\SI{2.3}{\m}}
\newcommand{\CTFCurrentManHoleSize}{\SI[product-units=power]{1.5 x 0.6}{\square\m}}
\newcommand{\CTFModifiedManHoleSize}{\SI[product-units=power]{4.0 x 4.0}{\square\m}}
\newcommand{\CTFPMTsNumber}{\num{80}}
\newcommand{\CTFPMTsAliveNumber}{\num{74}}
\newcommand{\CTFPMTsOnWallNumber}{\num{56}}
\newcommand{\CTFPMTsOnFloorNumber}{\num{24}}
\newcommand{\CTFPMTModel}{\mbox{ETL 9351}}
\newcommand{\CTFPMTSize}{\SI{8}{\inch}}
\newcommand{\CTFPMTQE}{\SI{27}{\percent}}
\newcommand{\CTFPMTCE}{\SI{60}{\percent}}
\newcommand{\CTFPMTWaveLength}{\SI{420}{\nano\meter}}
\newcommand{\CTFPMTBiasMax}{\SI{+1150}{\volt}}
\newcommand{\CTFPMTBiasMin}{\SI{+1600}{\volt}}
%--- OD High Background TMB
\newcommand{\ODOldNeutronRejectionMeasured}{\numrange{40}{60}}							%DocDb#982
%--- OD Low Background TMB
\newcommand{\ODNewNRAcceptance}{$>$\SI{81.3}{\percent}}
%--- OD
\newcommand{\ODPMTGain}{\num{1.E7}}
\newcommand{\ODPMTsNumber}{\num{190}}
\newcommand{\ODPMTsAliveNumber}{\num{180}}
\newcommand{\ODFrontEndGain}{\num{10}}
\newcommand{\ODADCBits}{\SI{10}{\bit}}													%Checked by SD
\newcommand{\ODADCSamplingRate}{\SI{1.25}{\GHz}}										%Checked by SD
\newcommand{\ODAcquisitionWindow}{\SI{200}{\us}}										%Analysis Memo v11 line 725
\newcommand{\ODBaselineWindow}{\SI{15}{\nano\second}}
\newcommand{\ODNeutronRejectionRequirement}{\num{200}}
\newcommand{\ODLaserPulseRate}{\SI{500}{\hertz}}
\newcommand{\ODLaserIntegrationWindow}{\SI{200}{\nano\second}}
\newcommand{\ODLaserAccidentalRate}{\SI{7.4}{\percent}}
\newcommand{\ODZeroSuppressionThreshold}{\SI{\sim0.25}{\pe}}
%--- 3Dpi
\newcommand{\LYSOTimeConstant}{\SI{45}{\nano\second}}
\newcommand{\ThreeDPiGammaEnergy}{\SI{511}{\kilo\eV}}
\newcommand{\ThreeDPiFOV}{\SI{200}{\centi\meter}}
\newcommand{\ThreeDPiID}{\SI{45}{\centi\meter}}
\newcommand{\ThreeDPiOD}{\SI{64}{\centi\meter}}
\newcommand{\ThreeDPiLArVolume}{\SI{1.3}{\cubic\meter}}
\newcommand{\ThreeDPiLArMass}{\SI{1800}{\kilo\gram}}
\newcommand{\ThreeDPiRingNumber}{\num{9}}
\newcommand{\ThreeDPiLArLayerThickness}{\SI{2.11}{\centi\meter}}
\newcommand{\ThreeDPiLArThickness}{\SI{19}{\centi\meter}}
\newcommand{\ThreeDPiTiThickness}{\SI{4}{\mm}}
\newcommand{\ThreeDPiSiPMSize}{\SI[product-units=power]{10 x 10}{\square\mm}}
\newcommand{\ThreeDPiNumSiPM}{\num{1E6}}
\newcommand{\ThreeDPiXenonPercentage}{\SI{10}{\percent}}
\newcommand{\ThreeDPiXenonConcentration}{\SI{1E5}{\ppm}}
\newcommand{\ThreeDPiXenonDopedDecayTime}{\SI{5}{\nano\second}}
\newcommand{\PETRadioTracerActivity}{\SI{10}{\milli\Curie}}
\newcommand{\ThreeDPiTimeResolution}{\SI{60}{\ps}}
\newcommand{\ThreeDPiEnergyResolution}{\SI{5}{\percent}}
\newcommand{\SigmaPar}{\mbox{$\sigma_\parallel$}}
\newcommand{\SigmaPerp}{\mbox{$\sigma_\perp$}}
\newcommand{\SigmaTau}{\mbox{$\sigma_\tau$}}
\newcommand{\ThreeDPiSensitivityGain}{\num{200}}
\newcommand{\ThreeDPiFOVSensitivityGain}{\num{40}}
\newcommand{\ThreeDPiFOVSNRGain}{\num{6.3}}
\newcommand{\ThreeDPiTimingSNRGain}{\num{3}}
\newcommand{\ThreeDPiTimingDoseGain}{\num{9}}
\newcommand{\CommercialPETBodyOutsideFOV}{\SI{85}{\percent}}
\newcommand{\ComemrcialPETGammaEfficiency}{\SI{5}{\percent}}
\newcommand{\CommercialPETTotalEfficiency}{\SI{1}{\percent}}
\newcommand{\CommercialPETFOV}{\SIrange{20}{30}{\centi\meter}}
\newcommand{\CommercialPETTimingRes}{\SI{400}{\pico\second}}
\newcommand{\CommercialPETBestTimingRes}{\SI{100}{\pico\second}}
%--- 3Dpi Simulations Results
\newcommand{\ThreeDPiTPBPointSourceSigmaX}{\SI{1.2}{\centi\meter}}
\newcommand{\ThreeDPiTPBPointSourceSigmaY}{\SI{1.2}{\centi\meter}}
\newcommand{\ThreeDPiTPBPointSourceSigmaZ}{\SI{0.9}{\centi\meter}}
\newcommand{\ThreeDPiTPBPointSourceSigmaPar}{\SI{2.1}{\centi\meter}}
\newcommand{\ThreeDPiTPBPointSourceSigmaPerp}{\SI{0.1}{\centi\meter}}
\newcommand{\ThreeDPiXePointSourceSigmaX}{\SI{4.4}{\milli\meter}}
\newcommand{\ThreeDPiXePointSourceSigmaY}{\SI{4.6}{\milli\meter}}
\newcommand{\ThreeDPiXePointSourceSigmaZ}{\SI{3.6}{\milli\meter}}
\newcommand{\ThreeDPiXePointSourceSigmaPar}{\SI{8.0}{\milli\meter}}
\newcommand{\ThreeDPiXePointSourceSigmaPerp}{\SI{1.1}{\milli\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterSigmaX}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterSigmaY}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterSigmaZ}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterSigmaPar}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterSigmaPerp}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterSigmaX}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterSigmaY}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterSigmaZ}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterSigmaPar}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterSigmaPerp}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndSigmaX}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndSigmaY}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndSigmaZ}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndSigmaPar}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndSigmaPerp}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndSigmaX}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndSigmaY}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndSigmaZ}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndSigmaPar}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndSigmaPerp}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTenSigmaX}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTenSigmaY}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTenSigmaZ}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTenSigmaPar}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTenSigmaPerp}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTenSigmaX}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTenSigmaY}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTenSigmaZ}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTenSigmaPar}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTenSigmaPerp}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTenSigmaX}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTenSigmaY}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTenSigmaZ}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTenSigmaPar}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTenSigmaPerp}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTenSigmaX}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTenSigmaY}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTenSigmaZ}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTenSigmaPar}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTenSigmaPerp}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTwentySigmaX}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTwentySigmaY}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTwentySigmaZ}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTwentySigmaPar}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatCenterTwentySigmaPerp}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTwentySigmaX}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTwentySigmaY}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTwentySigmaZ}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTwentySigmaPar}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatCenterTwentySigmaPerp}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTwentySigmaX}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTwentySigmaY}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTwentySigmaZ}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTwentySigmaPar}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiTPBNEMASpatEndTwentySigmaPerp}{\SI{}{\centi\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTwentySigmaX}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTwentySigmaY}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTwentySigmaZ}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTwentySigmaPar}{\SI{}{\milli\meter}}
\newcommand{\ThreeDPiXeNEMASpatEndTwentySigmaPerp}{\SI{}{\milli\meter}}
%--- GAP-TPC
\newcommand{\GAPTPC}{\mbox{GAP-TPC}}
\newcommand{\GAPTPCLightYield}{\SI{12}{\pe\per\keVee}}
\newcommand{\GAPTPCSPEResolution}{\SIrange{5}{10}{\percent}}
\newcommand{\GAPTPCSpatialResolution}{\SI{5}{\mm}}
\newcommand{\GAPTPCActiveDiameter}{\SI{50}{\mm}}
\newcommand{\GAPTPCActiveHeight}{\SI{50}{\cm}}
\newcommand{\GAPProtoActiveDiameter}{\SI{46}{\mm}}
\newcommand{\GAPProtoActiveHeight}{\SI{112}{\mm}}
%--- ReD
\newcommand{\ReDNeutronsEnergyRange}{\SIrange{1}{4}{\MeV}}
\newcommand{\ReDNeutronsEnergyAnalysisRange}{\SIrange{2}{3}{\MeV}}
\newcommand{\ReDArFortyThreshold}{\SI{1.497}{\MeV}}
\newcommand{\ReDRecoilsEnergyRange}{\SIrange{10}{200}{\keV}}
\newcommand{\ReDRecoilsEnergyMax}{\SI{200}{\keV}}
\newcommand{\ReDDirectionalityEnergyRange}{\SIrange{55}{206}{\keV}}
\newcommand{\ReDDirectionalityCrossSectionOneGeV}{\SI{E-46}{\square\cm}}
\newcommand{\RedNaplesVoltage}{\SI{15}{\mega\volt}}
\newcommand{\RedNaplesTransmission}{\SI{85}{\percent}}
\newcommand{\RedNaplesCurrent}{\SIrange{10}{200}{\nano\ampere}}
\newcommand{\RedNaplesLithiumSevenBindingEnergy}{\SI{-1.644}{\MeV}}
\newcommand{\RedNaplesLithiumSevenBeamEnergy}{\SIrange{20}{30}{\MeV}}
\newcommand{\RedNaplesCHTwoTargetDensity}{\SIrange{100}{200}{\micro\gram\per\centi\meter\squared}}
\newcommand{\RedNaplesTargetDensity}{\SI{0.2}{\milli\gram\per\centi\meter\squared}}
\newcommand{\RedNaplesSiTelescopeArea}{\SI[product-units=power]{0.5 x 0.5}{\square\cm}}
\newcommand{\RedNaplesSiTelescopeDistance}{\SI{60}{\centi\meter}}
\newcommand{\RedNaplesSiTelescopeAngle}{\SI{4.5}{\degree}}
\newcommand{\RedNaplesBeamIntensity}{\SI{0.5}{\rm p\nano\ampere}}
\newcommand{\RedNaplesCrossSection}{\SI{25}{\milli\barn\per\steradian}}
\newcommand{\RedNaplesCoincidenceNeutronRate}{\SI{10}{\hertz}}
\newcommand{\RedNaplesDEnergyRange}{\SIrange{6}{14}{\MeV}}
\newcommand{\RedNaplesHeliumThreeBindingEnergy}{\SI{3.27}{\MeV}}
\newcommand{\RedNaplesCDTwoTargetDensity}{\SIrange{100}{200}{\micro\gram\per\centi\meter\squared}}
\newcommand{\RedNaplesSiTelescopeCOuntingRate}{\SIrange{1}{2}{\kilo\hertz}}
\newcommand{\RedNaplesSiDetectorNumMicroStrips}{\num{16}}
\newcommand{\RedNaplesSiDetectorArea}{\SI[product-units=power]{4.8 x 4.8}{\square\cm}}
\newcommand{\RedNaplesSiDetectorDistance}{\SI{60}{\centi\meter}}
\newcommand{\RedNaplesSiDetectorAngle}{\SI{15}{\degree}}
\newcommand{\RedNaplesDBeamIntensity}{\SI{5}{\rm p\nano\ampere}}
\newcommand{\RedNaplesDCrossSection}{\SI{4}{\milli\barn\per\steradian}}
\newcommand{\RedNaplesDCoincidenceNeutronRate}{\SI{20}{\hertz}}
\newcommand{\RedNaplesSilverDBindingEnergy}{\SI{-2.22}{\MeV}}
\newcommand{\RedNaplesSilverCoulombBarrier}{\SI{13.5}{\MeV}}
\newcommand{\RedNaplesSilverDBreakupEnergy}{\SI{2.25}{\MeV}}
\newcommand{\RedNaplesSilverTargetDensity}{\SI{1}{\milli\gram\per\centi\meter\squared}}
\newcommand{\RedNaplesSiDetectorDistanceSilver}{\SI{15}{\centi\meter}}
\newcommand{\RedNaplesSiDetectorAbgleSilver}{\SI{70}{\degree}}
\newcommand{\RedNaplesDBeamEnergySilver}{\SI{10}{\MeV}}
\newcommand{\RedNaplesDBeamIntensitySilver}{\SI{10}{\rm p\nano\ampere}}
\newcommand{\RedNaplesDBeamNeutronRateSilver}{\SI{2}{\kilo\hertz}}
\newcommand{\RedNaplesDSilverCrossSection}{\SI{1}{\milli\barn\per\MeV\per\steradian}}
\newcommand{\RedNaplesDSilverNeutronRate}{\SI{0.2}{\ev\per\second\per\MeV}}
%--- ReD LNS
\newcommand{\RedLNSDistanceDedicatedLine}{\SI{80}{\deg}}
\newcommand{\RedLNSDistanceFromInteractionPoint}{\SI{1}{\m}}
%--- ReD Neutron Spectrometer
\newcommand{\RedLNSNeutronSpectrometerDetectorsManufacturer}{\mbox{Scionix}}
\newcommand{\RedLNSNeutronSpectrometerDetectorsNumber}{\numrange{8}{10}}
\newcommand{\RedLNSNeutronSpectrometerDetectorsPSD}{\SIrange{1.5}{2.0}{\sgm}}
\newcommand{\RedLNSNeutronSpectrometerDetectorsScintillatorType}{\mbox{EJ309}}
\newcommand{\RedLNSNeutronSpectrometerDetectorsPMTsDiameter}{\SI{3}{\inch}}
\newcommand{\RedLNSNeutronSpectrometerDetectorsPMTsType}{\mbox{ET 9821B}}
\newcommand{\RedLNSNeutronSpectrometerDetectorsPMTsTimeResolution}{\SI{1}{\nano\second}}
%--- Other Experiments
\newcommand{\DuNEHHVTest}{\SI{-115}{\kilo\volt}}
\newcommand{\pDUNELArMass}{\SI{700}{\tonne}}
%--- DS-50 Run Selection Criteria
\newcommand{\CriterionPSNumber}{CR\#1}
\newcommand{\CriterionPSString}{Period Selection}
\newcommand{\CriterionPSAArLiveTime}{\SI{56.4(2)}{\day}}										%Alessandro Razeto 9/26/14
%
\newcommand{\CriterionTTNumber}{CR\#2}
\newcommand{\CriterionTTString}{Run Type}
\newcommand{\CriterionTTAArLiveTime}{\SI{54.7(2)}{\day}}
%
\newcommand{\CriterionDGNumber}{CR\#3}
\newcommand{\CriterionDGString}{Digitizer Gate}
\newcommand{\CriterionDGTitle}{Usable runs}
\newcommand{\CriterionDGAArLiveTime}{\SI{53.8(2)}{\day}}
%
\newcommand{\CriterionNSNumber}{CR\#4}
\newcommand{\CriterionNSString}{No Small Runs}
\newcommand{\CriterionNSAArLiveTime}{\SI{53.5(2)}{\day}}
%
\newcommand{\CriterionDFNumber}{CR\#5}
\newcommand{\CriterionDFString}{DAQ Fever}
\newcommand{\CriterionDFAArLiveTime}{\SI{51.2(2)}{\day}}
%
\newcommand{\CriterionDCNumber}{CR\#6}
\newcommand{\CriterionDCString}{DAQ Cold}
\newcommand{\CriterionDCStringpaper}{Automated selection}
\newcommand{\CriterionDCAArLiveTime}{\SI{51.1(2)}{\day}}
%
\newcommand{\CriterionSRNumber}{CR\#7}
\newcommand{\CriterionSRString}{Single Run}
\newcommand{\CriterionSRAArLiveTime}{\SI{49.2(2)}{\day}}
%--- DS-50 Cuts
\newcommand{\CutNCNumber}{CX\#1}
\newcommand{\CutNCString}{Number of channels}
\newcommand{\CutNCValue}{\DSfPMTAliveNumber}
\newcommand{\CutNCSLADVariable}{nchannel}
\newcommand{\CutNCAArLiveTime}{\SI{48.8(2)}{\day}}
\newcommand{\CutNCUArLiveTime}{}
%
\newcommand{\CutBFNumber}{CX\#2}
\newcommand{\CutBFString}{Baseline found}
\newcommand{\CutBFValue}{\num{0}}
\newcommand{\CutBFSLADVariable}{SumChannelHasNoBaseline}
\newcommand{\CutBFAArLiveTime}{\SI{48.8(2)}{\day}}
\newcommand{\CutBFUArLiveTime}{}
%
\newcommand{\CutPTNumber}{CX\#3}
\newcommand{\CutPTString}{Time since previous trigger}
\newcommand{\CutPTSLADVariable}{(lifetime+inhibittime)}
\newcommand{\CutPTMin}{\SI{1.35}{\milli\second}}
\newcommand{\CutPTAArLiveTime}{\SI{48.7(2)}{\day}}
\newcommand{\CutPTUArLiveTime}{}
%
\newcommand{\CutLGNumber}{CX\#4}
\newcommand{\CutLGString}{Large gap}
\newcommand{\CutLGSLADVariable}{lifetime}
\newcommand{\CutLGAArMax}{\SI{1}{\second}}
\newcommand{\CutLGUArMax}{$\infinity$}
\newcommand{\CutLGAArLiveTime}{\SI{48.1(2)}{\day}}
\newcommand{\CutLGUArLiveTime}{}
%
\newcommand{\CutVPNumber}{CX\#5}
\newcommand{\CutVPString}{Veto data present}
\newcommand{\CutVPSLADVariable}{veto\_present}
\newcommand{\CutVPValue}{TRUE}
\newcommand{\CutVPAArLiveTime}{\SI{47.1(2)}{\day}}
\newcommand{\CutVPAArLiveDay}{\SI{47.1}{\liveday}}
\newcommand{\CutVPUArLiveTime}{}
%
\newcommand{\CutNPNumber}{CX\#6}
\newcommand{\CutNPString}{Number of pulses}
\newcommand{\CutNPSLADVariable}{n\_phys\_pulses}
\newcommand{\CutNPValue}{}
\newcommand{\CutNPAcceptance}{\mbox{$0.95^{+0.00}_{-0.01}$}}
%
\newcommand{\CutTTNumber}{CX\#7}
\newcommand{\CutTTString}{Coincident Trigger Time}
\newcommand{\CutTTSLADVariable}{s1\_start\_time}
\newcommand{\CutTTRange}{\SI{\pm50}{\nano\second}}
\newcommand{\CutTTAcceptance}{\mbox{$1.00^{+0.00}_{-0.01}$}}
%
\newcommand{\CutNSNumber}{CX\#8}
\newcommand{\CutNSString}{No \SOne\ Saturation}
\newcommand{\CutNSValue}{FALSE}
\newcommand{\CutNSSLADVariable}{is\_saturated\_pulse0}
\newcommand{\CutNSAcceptance}{\num{1.00}}												%Suppress 0 error
%
\newcommand{\CutWPNumber}{CX\#9}
\newcommand{\CutWPString}{\STwo\ pulse shape}
\newcommand{\CutWPSLADVariable}{total\_s2\_f90\_fixed}
\newcommand{\CutWPMax}{\num{0.20}}
\newcommand{\CutWPAcceptance}{\num{1.00}}												%Suppress 0 error
%
\newcommand{\CutMWNumber}{CX\#10}
\newcommand{\CutMWString}{Minimum \STwo}
\newcommand{\CutMWSLADVariable}{total\_s2\_true}
\newcommand{\CutMWMin}{\SI{100}{\pe}}
\newcommand{\CutMWAcceptance}{\mbox{$0.99^{+0.01}_{-0.04}$}}
%
\newcommand{\CutMFNumber}{CX\#11}
\newcommand{\CutMFString}{Max \SOne\ fraction per \PMT}
\newcommand{\CutMFSLADVariable}{s1\_max\_frac}
\newcommand{\CutMFAArAcceptance}{\SI{99}{\percent}}
\newcommand{\CutMFUArAcceptance}{\SI{95}{\percent}}
%
\newcommand{\CutCVNumber}{CX\#12}
\newcommand{\CutCVString}{Prompt \LSV\ Signal}
\newcommand{\CutCVSLADVariable}{roi\_total\_prompt\_charge}
\newcommand{\CutCVAArMax}{\SI{10}{\pe}}
\newcommand{\CutCVUArMax}{\SI{1}{\pe}}
\newcommand{\CutCVAArWindow}{\SIrange[range-units=single]{-10}{200}{\nano\second}}
\newcommand{\CutCVUArWindow}{\SIrange[range-units=single]{-50}{250}{\nano\second}}
\newcommand{\CutCVAArAcceptance}{\num{0.95}}												%Suppress 0 error
\newcommand{\CutCVUArAcceptance}{}															%Suppress 0 error
%
\newcommand{\CutHV}{CX\#13}
\newcommand{\CutHVstr}{Delayed \LSV\ and \WCV}
%\newcommand{\CutHVsliderwidth}{\SI{300}{\nano\second}}										%DocDb#972, Analysis Memo v11 line 1024
%\newcommand{\CutHVdelpemax}{\SI{80}{\pe}}
%\newcommand{\CutHVdelenemax}{\SI{150}{\keV}}
%\newcommand{\CutHVdelwin}{\SI{8.8}{\us}}													%DocDb#972, Analysis Memo v11 line 1024, confirmed by Shawn Westerdale: this is 8.8 us from PROMPT time, not TPC trig time.
%\newcommand{\CutHVlatewin}{\mbox{\TPC\ record length}}
%\newcommand{\CutHVlatepemax}{\SI{110}{\pe}}
%\newcommand{\CutHVlateenemax}{\SI{200}{\keV}}
%\newcommand{\CutHVlateenemaxmod}{\SI{280}{\keV}}
%\newcommand{\CutHVlateenemaxalt}{\SI{300}{\keV}}
%\newcommand{\CutHVlatectfpemax}{\SI{200}{\pe}}
%\newcommand{\CutHVdef}{(lsv\_max\_window\_charge<\CutHVdelpemax)\&\&(lsv\_late\_window\_charge<\CutHVlatepemax)\&\&(wt\_charge<\CutHVlatectfpemax)}
%\newcommand{\CutHVliv}{\SI{47.1(2)}{\day}}
%\newcommand{\CutHVacc}{\num{0.94}}															%Suppress 0 error
%\newcommand{\CutHVnewsliderwidth}{\SI{500}{\nano\second}}									%DocDb#972, Analysis Memo v11 line 1024
%\newcommand{\CutHVnewslidershortcapturetimes}{$\sim$6}
%\newcommand{\CutHVnewsliderlongcapturetimes}{$\sim$9}
%\newcommand{\CutHVnewdelshortpemax}{\SI{3}{\pe}}
%\newcommand{\CutHVnewdellongpemax}{\SI{6}{\pe}}
%\newcommand{\CutHVnewsliderwidth}{\SI{500}{\nano\second}}									%DocDb#972, Analysis Memo v11 line 1024
%\newcommand{\CutHVnewslidershortcapturetimes}{$\sim$6}
%\newcommand{\CutHVnewsliderlongcapturetimes}{$\sim$9}
\newcommand{\CutHVnewdelshortpemax}{\SI{3}{\pe}}                            				%DocDB 1345
\newcommand{\CutHVnewdellongpemax}{\SI{6}{\pe}}												%DocDB 1345
\newcommand{\CutHVnewsliderwidth}{\SI{500}{\nano\second}}									%DocDB 1345
%%
%\newcommand{\pvcutstr}{Pre-prompt \LSV\ Signal}
\newcommand{\pvcutpemax}{\SI{3}{\pe}}														%DocDB 1345
\newcommand{\pvcuttime}{$\sim$\SI{8}{\us}}													%DocDB 1345
%%
\newcommand{\mvcutstr}{Muon}																%DocDB 1345
\newcommand{\mvcutlsvpemax}{\SI{>2000}{\pe}}												%DocDB 1345
\newcommand{\mvcutwcvpemax}{\SI{>400}{\pe}}												%DocDB 1345
\newcommand{\mvcutdelay}{\SI{2}{\second}}													%DocDB 1345
%
\newcommand{\CutDF}{CX\#14}
\newcommand{\CutDFString}{Drift Time Fiducialization}
\newcommand{\CutDFSLADVariable}{tdrift}
\newcommand{\CutDFRange}{\SI{40.0}{334.5}{\us}}
\newcommand{\CutDFZRange}{\SI{36.3}{317.0}{\mm}}
\newcommand{\CutDFAcceptance}{\num{1.000(0)}}
%
\newcommand{\CutSONumber}{CX\#15}
\newcommand{\CutSOString}{\SOne\ range}
\newcommand{\CutSOSLADVariable}{total\_s1\_corr}
\newcommand{\CutSOMin}{\SI{20}{\pe}}														%Update 9/22/2014
\newcommand{\CutSOMax}{\SI{460}{\pe}}														%Update 9/22/2014
\newcommand{\CutSOAcceptance}{\num{1.000(0)}}
%
\newcommand{\CutRLNumber}{CX\#16}
\newcommand{\CutRLString}{Radial Fiducialization}
\newcommand{\CutRLMax}{\SI{16}{\cm}}
\newcommand{\CutRLSLADVariable}{radius<\CutRLMax}
%
\newcommand{\CutSRNumber}{CX\#17}
\newcommand{\CutSRString}{\STwo/\SOne}
\newcommand{\CutSRMax}{0.0}
\newcommand{\CutSRSLADVariable}{nr\_sigma\_s2}
\newcommand{\CutSRAcceptance}{\mbox{$0.53^{+0.01}_{-0.02}$}}
%
\newcommand{\CutRSNumber}{CX\#18}
\newcommand{\CutRSString}{\TPC\ Core}
\newcommand{\CutRSMax}{\SI{10}{\cm}}
\newcommand{\CutRSSLADVariable}{radius}
\newcommand{\CutRSFIducialMass}{\SI{11.7(5)}{\kg}}
%
\newcommand{\CutFNNumber}{CX\#19}
\newcommand{\CutFNString}{Fast \FNine}
\newcommand{\CutFNMin}{0.15}
\newcommand{\CutFNSLADVariablef}{total\_f90\_corr}
\newcommand{\CutFNAcceptance}{\num{1.00(0)}}
%
\newcommand{\DSfAArLiveTime}{\CutVPAArLiveTime}
\newcommand{\DSfAArLiveDay}{\CutVPAArLiveDay}
\newcommand{\DSfAArDFCumulariveAcceptance}{\mbox{$0.82^{+0.01}_{-0.04}$}}
\newcommand{\DSfAArSRCumulariveAcceptance}{\mbox{$0.429^{+0.010}_{-0.022}$}}
\newcommand{\DSfAArFNCumulariveAcceptance}{\mbox{$0.428^{+0.010}_{-0.022}$}}
\newcommand{\DSfUArLiveTime}{\SI{70.9}{\day}}
\newcommand{\DSfUArLiveDay}{\SI{70.9}{\liveday}}
\newcommand{\DSfUArDFCumulariveAcceptance}{}
\newcommand{\DSfUArSRCumulariveAcceptance}{}
\newcommand{\DSfUArFNCumulariveAcceptance}{}
%
\newcommand{\DSfDdNullFieldLightYield}{\SI{8.0(2)}{\pe\per\keV}}						% Doc 2508
\newcommand{\DSfDdNullFieldLYStability}{\SI{\sim0.4}{\percent}}							% Doc 2508
\newcommand{\DSfDdLTPostRVnum}{545.6}													% Total livetime after Run Validation before cuts.
\newcommand{\DSfDdLTPostRV}{\SI{\DSfDdLTPostRVnum}{\liveday}}							% Total livetime after Run Validation before cuts.
\newcommand{\DSfDdLTPostQualCutnum}{532.4}												% Total livetime after Run Validation and quality cuts.
\newcommand{\DSfDdLTPostQualCut}{\SI{\DSfDdLTPostQualCutnum}{\liveday}}					% Total livetime after Run Validation and quality cuts.
\newcommand{\DSfDdStartDate}{August 2, 2015}											% v3 runlist, Doc 1989
\newcommand{\DSfDdEndDate}{October 4, 2017}												% v3 runlist, Doc 1989
\newcommand{\DSfDdLaserrunDuration}{\SI{\sim5}{\minute}}								% Meyers -- typ value thru most of run -- from database
\newcommand{\DSfDdLSVOscLoss}{\SI{34.3}{\liveday}}										% Hao: Doc1625 Veto_Data_Validation_Hao_June12_2017.pdf, page 3
\newcommand{\DSfDdTPCPedRMSLoss}{\SI{16.2}{\liveday}}									% PDM XII-87
\newcommand{\DSfDdMinRunEvt}{1000~events}												% Xin's Livetime plotter
\newcommand{\DSfDdMinRunTime}{\SI{\sim10}{\minute}}
\newcommand{\DSfDdPoTwoTenSideRate}{\SI{2.51(1)}{\milli\becquerel\per\square\meter}}	% Corrected version of C. Stanford thesis table.  Email to P. Meyers 2/12/2018
\newcommand{\DSfSdFiftyPcAccPE}{\SI{75}{\pe}}											% 70-day paper Fig. 3
\newcommand{\DSfSdNinetyPcAccPE}{\SI{95}{\pe}}											% 70-day paper Fig. 3
\newcommand{\DSfDarkart}{{\tt darkart}}
\newcommand{\DSfDdRanBlindProb}{\num{2E-5}}
\newcommand{\DSfDdSTwoUncorrMin}{\SI{200}{\pe}}
\newcommand{\DSfDdSTwoFnMin}{0.20}
\newcommand{\DSfDdtdriftFid}{\SI{40}{\micro\s}}
\newcommand{\DSfDdtdriftFidcm}{\SI{4}{\centi\m}}
\newcommand{\DSfDdSurvBkgndSurfTypeOne}{$0.0006\pm 0.0001$}								% C. Stanford thesis, p. 119, scaled to 534 l.d.
\newcommand{\DSfDdSurvBkgndSurfTypeTwo}{$0.00092\pm 0.00004$}							% With full set of cuts, including R (on accidental S2's): Alissa Doc  2547, for 532.4 ld
\newcommand{\DSfDdSurvBkgndRadioNeutron}{$<\!0.005$}									% Was typo "<0.0005$ till 2/17 
\newcommand{\DSfDdSurvBkgndCosmoNeutron}{$<\!0.00035$}									% Doc 2505
\newcommand{\DSfDdSurvBkgndER}{0.08$\pm$0.04}											% By definition: target for box design.  Doc 2033 full_analysis_final_decisions.pdf
\newcommand{\DSfDdSurvBkgndTot}{$0.09\pm0.04$}											% Must be sum of previous!!

% 500-d cut info
\newcommand{\DSfDdLSVpromptInterval}{[-50,250]~ns}										% Shawn thesis, consistent with less info in Veto electronics paper
\newcommand{\DSfDdLSVprepromptInterval}{[$-10.5$,0]~$\mu$s}								% Veto electronics paper
\newcommand{\DSfDdLSVdelayedInterval}{[0,189.5]~$\mu$s}									% Veto electronics paper
\newcommand{\DSfDdWCVmuonActInterval}{0.6~s}
\newcommand{\DSfDdLSVpromptThreshold}{\SI{1}{\pe}}
\newcommand{\DSfDdRcutAcceptance}{\num{0.848(2)}}										% F. Granato, Doc 2376, acceptance-2018-03-23.pdf, updated to use "Method 1" via email 5/8/18.  Stat and sys errors directly added by P. Meyers.
\newcommand{\DSfDdSToverSOMinEffective}{\SI{150}{\pe}}									% Approx min S1 for which S2/S1 is effective particle ID cut.  From comparing Slides 9 and 10 of Doc 2033 "2018.02.09: Checks before box opening" (v3_4_1_check.pdf)
% 500-d misc
\newcommand{\DSfDdVPTdelayedStart}{\SI{200}{\nano\second}}								% Hao, Doc 2198, prompt_veto_tag_July_19_2017.pdf
\newcommand{\DSfDdBoxTop}{0.84}															% f90 of top of 540-d box.  Confirmed by G. Koh.
\newcommand{\DSfDdExposure}{{\SI{16660(270)}{\kg\day}}}									% P. Meyers XIII-6  (updated 5/25/18).  Includes radial cut acceptance. 
\newcommand{\DSfDdFiducialMass}{{\SI{31.3(5)}{\kg}}}									% P. Meyers XIII-6 (updated 5/25/18).  Includes radial cut acceptance.
\newcommand{\DSfUArAfterQualityCutsLiveTimeAdj}{70.9-live-day}
\newcommand{\DSfDdKrEightFiveActivityNum}{\num{1.9+-0.1}}								% G. Koh, checked by P. Meyers XIII-6.
\newcommand{\DSfDdKrEightFiveActivity}{{\DSfDdKrEightFiveActivityNum}~\si{\milli\becquerel\per\kg}}
\newcommand{\DSfDdSurvBkgndSurfTypeOneMod}{$<$0.0007}									% C. Stanford thesis, p. 119, scaled to 534 l.d., but with factor of ~100 tail-cut rejection (emailc 4/13/18).  Change didn't affect total background.
\newcommand{\DSfDdHundredGeVLim}{\SI{1.14E-44}{\square\cm}}								% G. Koh Email 5/21/2018
\newcommand{\DSfDdOneTeVLim}{\SI{3.78E-44}{\square\cm}}									% G. Koh Email 5/21/2018
\newcommand{\DSfDdTenTeVLim}{\SI{3.43E-43}{\square\cm}}									% G. Koh Email 5/21/2018
\newcommand{\DSfDdMinLim}{\SI{1.09E-44}{\square\cm}}									% G. Koh Email 5/28/2018
\newcommand{\DSfDdMinLimMass}{\SI{126}{\GeV\per\square\c}}								% G. Koh Email 5/28/2018
\newcommand{\DSfDdMinResSOneTwoTdrift}{\SI{3}{\us}}										% Minimum tdrift to resolve S1 and S2.  A. Monte, email to PDM 6/5/18.
\newcommand{\DSfDdMinSTwouncorrActual}{\SI{400}{\pe}}									% Minimum S2uncorr of interest in analysis, defined as lower edge of S2uncorr distribution for NR's near the edge of the detector with S1~100 PE.  (about the same for ER's)  PDM interpretation of Xin study, email 6/6/2018.
\newcommand{\DSfDdPulsefinderThr}{\SI{10}{\pe}}											% Approx thr.  Alden Fan thesis, Doc 2439, pp. 83-85
\newcommand{\DSfDdMinLivetimeCut}{\SI{400}{\micro\second}}								% A. Monte, Doc 2105, 2017-11-15.
\newcommand{\DSfDdRadCutTopBot}{\SI{23}{\mm}}											% PDM: approx -- read from 532-day Fig 4 with Rmax=17.8
\newcommand{\DSfDdRadCutCenter}{\SI{4}{\mm}}											% PDM: approx -- read from 532-day Fig 4 with Rmax=17.8
\newcommand{\DSfDdSurfBkgndPassSTwo}{$<$0.07}											% Number of surface events passing standard S2 cuts in 532 live-days.  C. Stanford.
\newcommand{\DSfDdLSVEffPrompt}{\num{0.9927+-0.0005}}									% Qian email to Meyers 12/28/2017 -- see Doc. 2884
\newcommand{\DSfDdLSVEffDelayed}{\num{0.9958\pm 0.0004}}								% Qian email to Meyers 12/28/2017 -- see Doc. 2884
\newcommand{\DSfDdLSVEffCombined}{\num{0.9964\pm 0.0004}}								% Qian email to Meyers 12/28/2017 -- see Doc. 2884
\newcommand{\DSfDdVPTCaptThr}{\SI{100}{\pe}}											% Final version used in n selection.  Code in G. Koh email to Meyers 2/13/18
\newcommand{\DSfDdVPTneutronEff}{0.79}													% PDM -- Doc. 2368 "2018-07-27: Final radiogenic neutron calculation for 532-d paper"
\newcommand{\DSfDdCosmoMuMaxE}{\SI{4}{\GeV}}											% PDM -- Doc 2505, 2027
\newcommand{\DSfDdCosmoMuMaxPath}{\SI{2}{\meter}}										% PDM -- Doc 2505, 2027
\newcommand{\DSfDdCosmoMCGen}{\SI{48.7}{\year}}											% PDM -- Doc 2505, 2027
\newcommand{\DSfDdCosmoMCreachTPC}{1388}												% PDM -- Doc 2505, 2027
\newcommand{\DSfDdSTwoMinSep}{\SI{4.65}{\mm}}											% Koh thesis, Doc 2745, p.51
\newcommand{\DSfDdRegionABBeforeRadCut}{30}												% Koh thesis, Doc 2745, p.73
\newcommand{\DSfDdRegionABAfterRadCut}{13}												% Koh thesis, Doc 2745, p.73
